Causally-guided Regularization of Graph Attention Improves Generalizability

Graph attention networks estimate the relational importance of node neighbors to aggregate relevant information over local neighborhoods for a prediction task. However, the inferred attentions are vulnerable to spurious correlations and connectivity in the training data, hampering the generalizability of the model. We introduce CAR, a general-purpose regularization framework for graph attention networks. Embodying a causal inference approach, CAR aligns the attention mechanism with the causal effects of active interventions on graph connectivity in a scalable manner. CAR is compatible with a variety of graph attention architectures, and we show that it systematically improves generalizability on various node classification tasks. Our ablation studies indicate that CAR hones in on the aspects of graph structure most pertinent to the prediction (e.g., homophily), and does so more effectively than alternative approaches. Finally, we also show that CAR enhances interpretability of attention weights by accentuating node-neighbor relations that point to causal hypotheses. For social media network-sized graphs, a CAR-guided graph rewiring approach could allow us to combine the scalability of graph convolutional methods with the higher performance of graph attention.

==> iclr2023/abstract.tex <==
Graph attention networks estimate the relational importance of node neighbors to aggregate relevant information over local neighborhoods for a prediction task.
%@AW: changing this to emphasize generalizability. I'd argue we should push for the causal view as a tool, rather than an end. 
However, the inferred attentions are vulnerable to spurious correlations and connectivity in the training data, hampering the generalizability of models. We introduce \methodname, a general-purpose regularization framework for graph attention networks. Embodying a causal inference approach based on invariance prediction, \methodname aligns the attention mechanism with the causal effects of active interventions on graph connectivity in a scalable manner.
\methodname is compatible with a variety of graph attention architectures, and we show that it systematically improves generalizability on various node classification tasks.
Our ablation studies indicate that \methodname hones in on the aspects of graph structure most pertinent to the prediction (e.g., homophily), and does so more effectively than alternative approaches.
Finally, we also show that \methodname enhances interpretability of attention coefficients by accentuating node-neighbor relations that point to causal hypotheses.
% For social media network-sized graphs, a \methodname-guided graph rewiring approach could allow us to combine the scalability of graph convolutional methods with the higher performance of graph attention. 


==> iclr2023/backup-20220925/abstract.tex <==
Graph attention networks estimate the relational importance of node neighbors to aggregate relevant information over local neighborhoods for a prediction task.
%@AW: changing this to emphasize generalizability. I'd argue we should push for the causal view as a tool, rather than an end. 
However, the inferred attentions are vulnerable to spurious correlations and connectivity in the training data, hampering the generalizability of the model. We introduce \methodname, a general-purpose regularization framework for graph attention networks. Embodying a causal inference approach, \methodname aligns the attention mechanism with the causal effects of active interventions on graph connectivity in a scalable manner.
% While causal methods can scale poorly, 
% Scalability is achieved by simultaneously performing multiple non-overlapping interventions.
\methodname is compatible with a variety of graph attention architectures and we show that it systematically improves generalizability on various node and graph classification tasks.
Our ablation studies indicate that \methodname hones in on the aspects of graph structure most pertinent to the prediction (e.g., task-relevant homophily), and does so more effectively than alternative approaches.
Finally, We also show that \methodname enables interpretability by identifying node-neighbor relations that point to causal hypotheses.
For social media network-sized graphs, a \methodname-guided graph rewiring approach could allow us to combine the scalability of graph convolutional methods with the higher performance of attention mechanisms. 


==> iclr2023/backup-20220925/intro.tex <==
Graphs encode rich relational information that can be leveraged in learning tasks across a wide variety of domains. Graph neural networks (GNNs) can learn powerful node, edge or graph-level representations by aggregating a node's representations with that of its neighbors. 
%Graph neural networks (GNNs) have demonstrated considerable promise in recent years by using these graph relations to supplement node representations with information from node neighbors.
%However, t
The specifics of a GNN's neighborhood aggregation scheme are critical to its effectiveness on a prediction task. For instance, many standard graph convolutional networks (GCNs) aggregate information over node neighborhoods via a simple averaging or max-pooling of neighbor features \citep{gcn_kipf_welling,graphsage}. While this scales well, it is also indiscriminate: GCNs are prone to suffer in many real-world scenarios where uninformative or noisy connections exist between nodes. GCNs may also over-smooth, with nodes in a graph taking on indistinguishable representations due to the indiscriminate aggregation operation \citep{gcn_oversmoothing,measuring_oversmoothing,topping2022understanding}. 

Graph-based attention mechanisms combat these issues by quantifying the relevance of node-neighbor relations and softly selecting neighbors in the aggregation step accordingly \citep{gat,gatv2,transformerconv}. This process of attending to select neighbors has contributed to significant performance gains for GNNs across a variety of tasks \citep{gnn_review, 2022message}. In addition, similar to the use of attention in natural language processing and computer vision \citep{attn_review}, attention in graph settings enables the interpretability of model predictions via the examination of attention weights \citep{attn_interpret,attn_generalization_gnn}. 

Paramount to the effectiveness of attention mechanisms in GNNs is their ability to discern the specific graph connectivity patterns that underlie accurate, generalizable predictions. As graph training data often contains noisy features and/or connections, attention mechanisms in GNNs can be sensitive to spurious correlations that mislead them in how they attend to node neighbors. The result of this miscalibrated attention manifests as a failure to generalize to unseen data \citep{attn_generalization_gnn}. One approach to improve the GNN's generalizability is to regularize the attention weights so that they become more robust to spurious correlations/connections in the training data. The limited previous work along this direction has focused on $L_0$ regularization of attention weights to enforce sparsity \citep{ye2021sparse} or has co-optimized a link prediction side-task using the attention mechanism\citep{kim2021how}. Since these regularization strategies are formulated independently of the actual prediction task, they align the attention mechanism with some intrinsic property of the input graph in always the same way, regardless of the training objective. 
%Some of the previous work is also specific to the kind of graph attention mechanism chosen. 
% the inability of attention mechanisms to select the appropriate node neighbors also suggests an inability to determine the graph connections that causally contribute to a particular prediction.

We instead approach the regularization task from the perspective of causal modeling. Intuitively, an edge in the input graph is important to a prediction task if removing it leads to substantial degradation in the prediction performance of the GNN. The key conceptual advance of this work is to leverage active interventions on node neighborhoods (i.e., deletion of specific edges) to align graph attention training with the causal impact of these interventions on task performance. We introduce \methodname, a causal attention regularization framework that is suitable for any graph attention network architecture. To our knowledge, this is the first work to take a causal, edge-intervention approach to learning graph attention weights. While some efforts have previously been made to infuse notions of causality into GNNs, these causal approaches have been largely limited to using causal effects from pre-trained models as features for a separate model \citep{trust_neigh,attn_generalization_gnn} or decoupling causal from non-causal effects \citep{causal_attn_graph}. 

We applied \methodname on three graph attention architectures across seven node classification and graph-property prediction tasks each, finding that it consistently and significantly improved test loss and accuracy. Our ablation studies suggest that \methodname derives its power by better capturing the aspects of graph homophily relevant to the prediction task. In comparison to our causal approach, a label-propagation approach (that captures homophily more generically) did not regularize the attention weights as effectively. 

Understanding how GNNs learn remains a major open problem and an active area of research. Towards this, our findings support previous evidence [CITE] that graph attention weights capture certain aspects of homophily. \methodname refines these weights by aligning them with the aspects of graph homophily that are causally relevant to the prediction task. \RS{need a line about interpretability}. Also, by applying it on sample sub-networks for a large social media-sized network, \methodname can enable us to learn the attention weights that would generalize to the broader network. These networks are too large for attention-based approaches and are instead typically processed using GCNs.  Using \methodname-learnt attention weights to guide graph rewiring could improve the results obtained with convolutional techniques while ensuring scalability.    

% performance gains
% intepretability
% issues: spurious correlations (training data size?, training data network connectivity), limitations of interpretability
% sensitivity to initialization

% themes:
% graph attention
% determining relevant neighbors
% causal modeling: interventions ("causal view of robustness...", "matching learned causal effects...")
% causal attention
% causal regularization: KDD paper + ICML paper (causal effects domain priors)
% 

==> iclr2023/backup-20220925/related_work.tex <==
The performance gains associated with graph attention networks have led to a number of efforts to enhance and better understand graph attention mechanisms \citep{gat_survey}. One category of methods aims to improve the expressive power of graph attention mechanisms by supplementing a given prediction objective with one or more tasks. \cite{attn_generalization_gnn} found that adding the supervised training of attention as an auxiliary task dramatically improved classification accuracy and that classification accuracy depended exponentially on attention correctness in their experiments. Such settings with ground truth attention are rare, though, so alternative tasks have been proposed to learn better attention weights. For example, SuperGAT adds an edge self-supervision task that uses the connectivity patterns of existing edges in a graph to inform the assignment of attention weights to edges \citep{kim2021how}. 
% still need to add some more here...

A related set of methods leverage signals from interventions on graphs to aid in training GNNs. \cite{attn_generalization_gnn} devised an auxiliary weakly-supervised attention learning task based on changes in a pre-trained GCN's predictions that stem from node-level interventions. Causal GCN Inference (CGI) uses the outcomes of node-level interventions on a pre-trained GCN as well but as features in a classifier rather than as a means of informing attention \citep{trust_neigh}. Meanwhile, the Causal Attention Learning (CAL) strategy \citep{causal_attn_graph} aims to decouple causal and non-causal effects by introducing an additional task that encourages robustness to abstract interventions on graph representations rather than specific nodes or edges. Unlike these approaches, \methodname employs active interventions on specific edges during training and leverages causal effects specific to both the model being trained and its prediction task to guide attention training.

Perhaps the method most comparable to ours is CFLP~\cite{2106.02172}, which treats an edge's existence as an individual treatment effect and constructs a causal model to predict the average treatment effect directly. However, it differs from \methodname substantially, both in application and approach. \methodname uses an estimate of the individual treatment effect to regularize the attention weights for arbitrary attention-based models, rather than alter the data distribution that is used for training. Additionally, CFLP is aimed at link-prediction which requires positional, rather than structural, representations\cite{Srinivasan2020On}, whereas our work is aimed at node and graph classification for which structural representations are sufficient.

% Graph data augmentation
Inspired by the success of data augmentation approaches in computer vision, graph perturbations have also found their use in graph data augmentation~\cite{2202.08871}. In DropEdge~\cite{DBLP:conf/iclr/RongHXH20}, edges are randomly deleted in subgraph samples to reduce overfitting. Dropping edges indiscriminately can result in pathological examples that limit generalization. TADropEdge~\cite{gao2021training} seeks to limit this effect by drawing edges according to topological invariants. MH-Aug~\cite{NEURIPS2021_9e7ba617} instead uses Metropolis-Hastings to generate new training examples through a set of graph mutation rules. AD-GCL~\cite{suresh2021adversarial} constructs a contrastive learning framework to drop edges by minimizing the information lost by dropping each edge. All of these approaches are designed either for self-supervised learning (e.g., AD-GCL) or in a task-agnostic fashion (e.g., DropEdge), distinguishing them from \methodname. % This is done to increase generalization by reducing the number of repeated structural features that are learned.

% Graph Rewiring

Many methods have explored graph rewiring as a way to improve inferential accuracy, predictive performance, or improve generalization. GDC~\cite{10.5555/3454287.3455484} seeks to improve information diffusion while reducing noise through densification and then sparsification steps. In an attempt to debias learned representations, FairAug~\cite{2201.08549} and FairDrop~\cite{9645324} remove edges according to a defined fairness metric. MeTa~\cite{NEURIPS2021_0b0b0994} generates new subgraphs through temporal edge-sampling, and then learns to pass messages between temporally distinct subgraphs. This method has clear causal intuition, but without the interventional semantic of \methodname. The AdaEdge method~\cite{Chen_Lin_Li_Li_Zhou_Sun_2020}, supervised edge-perturbation is performed through multiple full-training runs where the graph is rewired to optimize for predicted-homophily.

% Graph Geometry

Another related set of methods have observed that intrinsic properties of the graph, such as sparsity or curvature, can be leveraged to rewire the graph to increase task generalization. Pro-GNN\cite{10.1145/3394486.3403049} co-learns a GNN and a sparsified graph structure to build methods that are robust to external perturbation. Sparsification is learned through structural optimization of the adjacency matrix. Similar to \methodname, NeuralSparse~\cite{pmlr-v119-zheng20d} seeks to sparsify by removing task-irrelevant edges. NeuralSparse, however, chooses to do so by learning a generative distribution over graph perturbations. Moving beyond sparsification, work based on the balanced Forman curvature~\cite{topping2022understanding} rewires the graph to improve information flow through the graph, which yielded state of the art performance on a variety of benchmarks. This idea is pushed further in by Bober \textit{et al.}~\cite{2207.08026} where they view a graph as a discrete geometry and use tools for discrete differential geometry. Alternatively, DiffWire~\cite{2206.07369} presents two different GCN layers: CT and GAP that are fully differentiable and optimize graph connectivity according to commute times or the algebraic connectivity. While \methodname can be understood through the lens of graph sparsification, \methodname does not seek to explicitly alter the edge connectivity through structural perturbations that may be deleterious to generalization. Moreover, \methodname alters the underlying geometry in \textit{task specific} ways.


% edge-level interventions
% during training (accounts for ability of GAT to adjust weights of neighbors vs. indiscriminate pooling as in GCNs)

% \noindent \textbf{Attention in GNNs:}

% \noindent \textbf{Graph Attention Regularization:} 

% self-supervised learning: friendly neighbors
% weakly supervised learning: graph attention generalization (attention over nodes, intervention w/ weak supervision)
% causal: granger-causal attentive mixtures of experts, trust neighbors?
% l0 regularization: ye2021 - graph rewiring too

% \cite{attn_generalization_gnn} found that, in cases where ground-truth attention is available, supervised training of attention contributed to improved generalization performance of models to unseen and noisy graph inputs. 

% Hence, efforts have been made to design graph attention through supplementing learning tasks with self-supervision \cite{friendly_neigh} or by .

% using causal effects from pre-trained models as features for a separate model \citep{trust_neigh} or decoupling causal from non-causal effects \citep{causal_attn_graph}. To our knowledge, no efforts have . 

% graph attention
% graph causal modeling
% causal explanations
% causal regularization (graph domain priors, CAL) + supervised attention

==> iclr2023/backup-20220925/results.tex <==
\subsection{Experimental Setup}
We assessed the effectiveness of \methodname across a diverse set of prediction tasks, datasets, graph attention mechanisms, and hyperparameter choices. We evaluated \methodname on 6 node classification and Y graph property prediction datasets (Y1 regression tasks, Y2 classification tasks). We used a minimal network architecture for all datasets, which consisted of $L=1$ or $L=2$ graph attention layers positioned between single-layer feed-forward networks (Appendix \ref{appen:arch_hyper}). For each model, one of the GAT, GATv2, or Graph Transformer attention mechanisms was used as the graph attention operator \citep{gat,gatv2,transformerconv}. 

To establish \methodname's robustness to hyperparameter choices, we evaluated \methodname across a broad range of hyperparameter settings rather than employing a hyperparameter selection scheme for each model configuration. The number of attention heads was selected from $k=\{1,3,5\}$; the regularization strength was from $\lambda=\{0.1,0.5,1,5\}$; and the number of hidden features used across layers were from $F'=\{100,200\}$ or $F'=\{10,25\}$. See Appendix \ref{appen:arch_hyper} for more details on the network architecture, hyperparameter, and training configurations. 

We used binary cross-entropy loss for the causal regularization loss $\ell^c(\cdot,\cdot)$, and the link function $\sigmoid(\cdot)$ was chosen to be the sigmoid function with temperature $T=0.1$. Unless otherwise specified, we perform 5 rounds of edge interventions per mini-batch when training with \methodname. Runtimes for training models with \methodname ranged from roughly 2 seconds to 5 minutes on the evaluated datasets, with \methodname's runtime only 1.5-2 times that of standard training on average. We provide more details on scalability, runtime, and memory usage in Appendix \ref{appen:runtime_memory}.

\subsection{Node Classification}
\noindent \textbf{Datasets and evaluation:} We used a total of 8 real-world node classification datasets of varying sizes and degrees of homophily: Cora, CiteSeer, PubMed, ogbn-arxiv, Chameleon, and Squirrel. Each model was evaluated according to its accuracy with respect to a held-out test set. We also evaluated the test cross entropy loss, as it accounts for the full distribution of per-class predictions rather than just the highest-valued prediction as in the accuracy calculation. See Appendix \ref{appen:node_class_datasets} for details on dataset statistics, splits, and references. 

\noindent \textbf{Generalization performance:} We compared both the test accuracy and the test loss of each model when trained with and without \methodname. We found that across graph attention mechanisms and hyperparameter choices, training with \methodname resulted in significantly higher test accuracy in 7 of the 8 node classification datasets and a significant reduction in test loss in all 8 datasets (\textbf{Figure} \ref{fig:figure_2}, $p < 0.05$, paired Wilcoxon signed-rank test).  Furthermore, for 6 of the 8 datasets, when focusing on the \methodname-trained models that were trained with the higher $\lambda=1$ or $\lambda=5$ causal regularization strengths, \methodname-trained models demonstrated significantly larger reductions in test loss in these datasets compared to those that were trained with the lower $\lambda=0.1$ or $\lambda=0.5$ values ($p < 0.05$, one-tailed Welch's $t$-test, Appendix \ref{appen:compare_loss_lambda}). These results highlight the consistency of performance gains achieved with \methodname across the vast space of graph attention mechanisms and hyperparameters evaluated.

\noindent \textbf{Selecting $\lambda$ for \methodname in multi-layer GNNs:} (still include?)

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.995 \linewidth ]{fig2_causal_comparison_node.pdf}
    \caption{Test accuracy and negative loss on 8 node classification datasets}
    \label{fig:figure_2}
\end{figure}

% HERE: number of interventions per node?
\subsection{Model Investigation and Ablation Studies}
\RS{points to make: a) \methodname accentuates correlation with homophily, more so for heterophilic networks [label agreement result?]; b) effect of hyperparameter $\lambda$ (b.1: violin plot; b.2: dialed-up/down cora homophily)  c) an ablation where label propagation was directly used to regularize also helps but not as much as \methodname, esp for heterophilic networks; \sout{d) random edge ablation?}}


We also evaluated the degree to which aligning attention mechanisms with their causal effects contributed to this improved generalization performance. To do so, we employ a similar regularization scheme to that of \methodname (\textbf{Equation} \ref{eqn:causal_effect}) but decouple the causal effect calculation from the specific network being trained. Instead of using predictions from the network to determine the causal effect, we use predictions from a neighbor voting model, in which each node's classification prediction is a histogram of class labels from the node's neighbors. In this neighbor voting regularization scheme, the attention mechanism for the network being trained is thus guided during training by the effects of edge interventions to this neighbor voting model's predictions rather than by the effects of edge interventions to the network's own predictions. 

% Separately, we also we simply draw each causal effect $c_{i,j}^{(n)}$ from a uniform distribution on the interval $[0,1)$ 

We compared \methodname-trained models with those trained with neighbor voting regularization by evaluating the consistency of their test loss improvements with respect to the baseline models without regularization across the aforementioned set of model architecture and hyperparameter choices. Models trained when regularizing attention weights with the neighbor voting scheme underperformed those trained with \methodname in 7 of the 8 datasets (\textbf{Table} \ref{table:ablation}). The neighbor voting-based regularization did in most cases lead to a gain in performance relative to the baseline models trained without any regularization, though, which lends support to the utility of regularization in training attention, even if non-specific. Overall, these results demonstrate the effectiveness of using \methodname to improve generalization performance for many node classification tasks.

\begin{table}[h!]
\centering
\caption{Generalization performance of \methodname-trained models with ablations compared to baseline \\($-\log_{10}(p)$, one-tailed paired Wilcoxon signed-rank test)}
\label{table:ablation}
\renewcommand{\arraystretch}{1.8}
\resizebox{14cm}{!}{%

\begin{tabular}{ r  c  c  c  c  c  c  c  c } 
    % \multirow{3}{*}{\bf Method}  &\multicolumn{2}{c}{\bf Cora} &\multicolumn{2}{c}{\bf CiteSeer} &\multicolumn{2}{c}{\bf PubMed} &\multicolumn{2}{c}{\bf orgn-arxiv} &\multicolumn{2}{c}{\bf Chameleon} &\multicolumn{2}{c}{\bf Squirrel} \\ 
    & \textbf{Cora} & \textbf{CiteSeer} & \textbf{PubMed} & \textbf{ogbn-arxiv} & \textbf{Chameleon} & \textbf{Squirrel} & \textbf{Cornell} & \textbf{Wisconsin} \\
    % \cmidrule(lr){2-3}\cmidrule(lr){3-4}\cmidrule(lr){5-6}
    \hline
    \methodname & \textbf{8.99} & \textbf{4.34} & \textbf{7.81} & \textbf{0.655} & \textbf{10.84} & 9.56 & \textbf{3.84} & \textbf{6.24} \\
    \hline
    Neighbor Voting & 8.89 & 3.62 & 4.78 & 0.233 & 9.20 & 10.84 & 2.28 & 5.30 \\
    \hline
    Random & X & X & X & X & X & X \\
\end{tabular}}
\end{table}


% \begin{table}[h!]
% \centering
% \caption{\methodname-trained graph attention mechanisms attend to homophilous edges in node classification}
% \label{table:attn_homophily}
% \renewcommand{\arraystretch}{2.5}
% \begin{tabular}{ c  c  c  c  c  c  c } 
%     & Cora & CiteSeer & PubMed & ogbn-arxiv & Chameleon & Squirrel \\
%     % \cmidrule(lr){2-3}\cmidrule(lr){3-4}\cmidrule(lr){5-6}
%     \hline
%     Baseline & 0.81 \pm 0.01 & 0.76 \pm 0.01 & 0.81 \pm 0.01 & 0.70 \pm 0.01 &  \\
%     \hline
%     Baseline & 0.81 \pm 0.01 & 0.76 \pm 0.01 & 0.81 \pm 0.01 & 0.70 \pm 0.01 & 
% \end{tabular}
% \end{table}

\subsubsection{Label agreement} 
We also sought to determine if the graph attention mechanisms in models trained with \methodname more effectively prioritized relevant edges. For the node classification task, the relevant neighbors to a particular node are expected to be those that share the same label as that node. Therefore, we used the label agreement between nodes connected by an edge as a proxy for the ground-truth relevance of the edge. Specifically, we assign a reference attention weight to an edge based on the label agreement in the target node's neighborhood \citep{kim2021how}.
\begin{equation}
    \label{eqn:label_agreement}
    \ell_{ij} = \hat{\ell}_{ij}/\sum_{k\in N(j)} \hat{\ell}_{kj}
\end{equation}
Here, $\hat{\ell}_{ij} = 1$ if nodes $i$ and $j$ have the same label $\hat{\ell}_{ij} = 0$ otherwise. $N(j)$ denotes the in-neighbors of node $j$. We then calculate the KL divergence of an edge's attention weight $\alpha_{i,j}$ from its reference attention weight $\ell_{ij}$ and summarize a model's ability to identify relevant edges as the mean of these KL divergence values across the edges in the held-out test set. 

We compared these mean KL divergences between baseline models trained without \methodname and models trained with \methodname across the same broad range of model architecture and hyperparameter choices described above. We found that \methodname-trained models consistently yielded lower mean KL divergence values than models trained without \methodname  for 6 of 8 node classification datasets (\textbf{Figure }\ref{fig:figure_3},$p < 0.05$, paired Wilcoxon signed-rank test). 
% The improvement in AP for \methodname-trained models was particularly pronounced for the Chameleon and Squirrel datasets, which are characterized by lower homophily, while the higher homophily datasets (Cora, CiteSeer, PubMed) were not associated with such gains (Appendix \ref{appen:label_agreement_homophily}). 
Notably, this enhanced prioritization of relevant edges was achieved without explicitly optimizing label agreement during training and is an inherent manifestation of aligning attention with the node classification tasks' causal effects. 
% In addition, this result highlights the applicability of \methodname for low homophily graphs, as graph attention is essential in such settings due to the relative dissimilarity of neighboring nodes in these graphs. 
Thus, these results demonstrate that \methodname not only improves performance on node classification tasks but also more accurately prioritizes the edges that are most relevant to the task at hand. 

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.7 \linewidth ]{fig3_label_agreement.pdf}
    \caption{Coherence between attention weights and label agreement for \methodname-trained models compared to baseline}
    \label{fig:figure_3}
\end{figure}

% \subsubsection{Cheeger Constant}
% \TM{Do we have results here? Because the graphs are all disconnected, this might be difficult to interpret.}
% Next, we turn our attention to a series of experiments intended to understand the topological changes that our graph undergoes due to our causal regularization method. 

% Because our method prunes edges, we are specifically interested in understanding whether our method is introducing bottlenecks that would make us more susceptible to over-squashing. To answer this question, we compute Cheeger constant as a function of regularization strength for the Cora dataset.

% Furthermore, we computed the curvature of the original graph, pruned graph, and removed edges; and present the kernel density estimates below.

\subsubsection{Graph Diffusion Distance}
\TM{Do we have results here? It feels like a nice to have but probably a P1/P2 priority.}
Next, we are interested to understand whether our proposed method is simply removing edges that are ``topologically noisy''. To answer this question, we have computed the graph diffusion distance defined as

\begin{equation}
 d^{(u,v)}_{GDD}(A_1, A_2) = \sqrt{ \argmax_{t} \left | \left |  e^{-t L}  - e^{-t L\backslash ({u,v}) } \right | \right |^2_F},
\end{equation}

where $L$ is the graph Laplacian, and $L\backslash ({u,v})$ is the graph Laplacian with the edge from $u$ to $v$ deleted. We use this metric because it provides a global measure of graph diffusion, which is intimately connected to message passing.



\subsection{Graph Classification}
\noindent \textbf{Datasets and evaluation:} We used a total of Y real-world graph property prediction datasets, of which Y1 are regression tasks (ogbg-R1, ogbg-R2, ogbg-R3) and Y2 are classification tasks (ogbg-molbace, ogbg-B, ogbg-C, ogbg-molpcba). Regression tasks were evaluated using the Kendall's $\Tau$ correlation between model predictions and their corresponding ground-truth values, as has been done in previous graph ranking tasks \citep{graph_rank}. The ogbg-molbace, ogbg-B, and ogbg-C classification tasks were evaluated using the area under the receiver opereating characteristic curve (AUROC), while the ogbg-molpcba task was evaluated using the average precision (AP) due to its extreme class imbalance. See Appendix \ref{appen:graph_prop_datasets} for more detailed descriptions of dataset statistics, splits, and references. 

\noindent \textbf{Generalization performance:}
\TM{@RS, this is the section I was thinking of. Let's just comment out the heading?}

% \subsection{\methodname-Guided Pruning}
% While graph attention networks have demonstrated notable performance gains, its inclusion of graph attention layers currently limits its use in large-scale applications compares to GCNs, for which a number of advances in scalability have been made \citep{sign}. To leverage the advantages of \methodname in graph attention alongside the scalability of GCNs, we explored a graph rewiring approach based on \methodname-guided edge pruning. For a given dataset, we first use a trained graph attention network to assign an attention weight for each edge in the training and validation sets, after which edges with attention weights below a threshold $\alpha_{T}$ are pruned. A GCN is then trained on the rewired training set with early stopping imposed with respect to the validation loss on the rewired validation set. 


\subsection{Explainability}

In addition to providing a robust way to increase both model quality and generalization, \methodname learn attention weights that feel more explainable. We compute the edge-wise difference of the attention values to understand the differences between the base and causally attended models. In the case of the \textrm{ogbn-arxiv} dataset, we observe that the shifts in attention between the two models can largely be understood as fitting into one of three stories (i) down-weighting self-citations with a time gap of more than two years, (ii) down-weighting popular ``anchor'' papers, or (iii) upweighting topically-narrow papers with few citations.

In the first case, we find that \methodname down-weights edges associated with self-citations. The causal story here is quite clear as well -- machine learning is a fast moving field with authors moving into the field and changing specialties as those specialties are born. Because of this, the narrative arc that a set of authors constructs to present this idea can include citations to previous work from different subfields. While these citations do help situate the work within the broader research community, and can highlight unconventional connections that readers might find valuable, they are not relevant to the topic-prediction task. As an illustrative example, we present a few examples of title pairs which were significantly downweighted in table~\ref{tab:self-cites}.

\begin{table}[ht]
\caption{\label{tab:self-cites}Down-weighted Self Citations. }
\label{sample-table}
\begin{center}
\begin{tabular}{p{0.4\linewidth} p{0.4\linewidth} p{0.10\linewidth}}
Paper Title & Cited Title & $\Delta$ \\
 \hline
\textit{Viterbinet a Deep Learning Based Viterbi Algorithm for Symbol Detection} &
\textit{Frequency Shift Filtering for Ofdm Signal Recovery in Narrowband Power Line Communications} & -90.13 \% \\
\textit{Solving Underdetermined Systems with Error Correcting Codes} &
\textit{Systems of MDS Codes from Units and Idempotents} & -89.80 \% \\
\textit{adaptive cross packet harq} &
\textit{rate adaptation for secure harq protocols} & -81.96 \% \\
\end{tabular}
\end{center}
\end{table}

In the second case, we find that \methodname down-weights edges directed towards popular or otherwise seminal papers. The causal story for this is clear -- these papers tends to be included in introductions to provide references for industry standard concepts like the existence of a ResNet, Word2Vec, or ADAM. It's quite clear that these citations span communities, and as such, have little bearing on the prediction task at hand. We have collected an illustrative set of examples and present them in table~\ref{tab:anchor-cites}.

% Table of down-weighted papers
\begin{table}[th]
\caption{\label{tab:anchor-cites}Down-weighted self citations associated with the citation of ``anchor'' papers. Each of the cited works that is down-weighted is a well known ML paper.}
\label{sample-table}
\begin{center}
\begin{tabular}{p{0.42\linewidth} p{0.42\linewidth} p{0.10\linewidth}}
Paper Title & Cited Title & $\Delta$ \\
\hline
\textit{Quantization Networks} &
\textit{Deep Residual Learning for Image Recognition} &
-99.94\% \\
\textit{Hypergraph Convolution and Hypergraph Attention} &
\textit{ADAM: a Method for Stochastic Optimization} &
-99.88\% \\
% Submodular Hamming Metrics &
% Distributed Representations of Sords and Phrases and Their Compositionality &
% -99.92\% \\
\textit{Robust Learning from Untrusted Sources} &
\textit{Batch Normalization Accelerating Deep Network Training by Reducing Internal Covariate Shift} &
-99.86\% \\
\end{tabular}
\end{center}
\end{table}

The representation that is learned by \methodname does not simply learn to ignore high-degree nodes. In the example of the Word2Vec paper, we find that significant increases in attention weight for a multiple highly related papers, including Node2Vec which saw a 1.2e5 \% increase and \textit{Quantum Inspired Complex Word Embedding} realized a 9.5e4 \% increase.

In the final case, we observed that \methodname up-weighted edges directed towards deeply related but largely unnoticed papers. In our manual exploration of the data, we observed that these papers are those that are dangerously close to your proposed method, which you only find after a thorough literature review. Obviously, these are exactly the sorts of edges that we would like to up-weight for the task of predicting a paper's topic. We present a sampling of the up-weighted citations in table~\ref{tab:up-cites}.

\begin{table}[ht]
\caption{\label{tab:up-cites} Upweighted highly relevant citations.}
\label{sample-table}
\begin{center}
\begin{tabular}{p{0.35\linewidth} p{0.35\linewidth} p{0.10\linewidth}}
Paper Title & Cited Title & $\Delta$ \\
\\ \hline \\
\textit{Bundle Adjustment Revisited} &
\textit{Distributed Bundle Adjustment} &
5200 \% \\
\textit{Optimality and Approximate Optimality of Source Channel Separation in Networks} &
\textit{Multicasting Correlated Multi Source to Multi Sink Over a Network} &
4600 \% \\
\textit{Cyclic Orbit Codes} &
\textit{List Decoding of Lifted Gabidulin Codes via the Plucker Embedding} &
3960 \% \\
\end{tabular}
\end{center}
\end{table}

\subsection{Runtimes and Scalability}

\TM{ Number of interventions scales as $O(C * |V|)$. Each intervention scales as $O(b^2l)$ due to the BFS to ensure non-overlapping interventions, where b is the branching factor and l is the number of layers. In the long run, we're unconcerned about the identification of non-overlapping interventions can be done as a preprocessing step, similar to the generation of graph samples in graph sage.}
% AW: included a section in appendix (feel free to modify with content from here)
\TM{Table of runtimes}
% AW: included in appendix

==> iclr2023/backup-20220925/theory.tex <==
\subsection{Graph Attention Networks}

Attention mechanisms have been effectively used across many domains by enabling models to dynamically attend to the specific parts of an input that are most relevant to a prediction task \citep{attention_survey}. In graph settings, attention mechanisms compute the relevance of node-neighbor relations, as denoted by the edges of the graph. The neighbor aggregation operator in GNNs then uses this information to weight the contribution of each edge in the prediction task. 

Across the multitude of graph attention mechanisms that have been proposed \citep{gat_survey}, the procedures for computing attention share a general form \citep{gat}. A graph attention layer takes as input a set of node features $\mathbf{h} = \{\vec{h}_1,...,\vec{h}_N\}$, $\vec{h}_i \in \mathbb{R}^F$, where $N$ is the number of nodes and $F$ is the dimensionality of the node features. From these node features, the graph attention layer in a GAT computes unnormalized attention weights for each edge $(i,j)$
\begin{equation}
    \label{eqn:attn_edges}
    e_{ij} = a(\mathbf{W}\vec{h}_i,\mathbf{W}\vec{h}_j),
\end{equation}
where $\mathbf{W}\in \mathbb{R}^{F' \times F}$ linearly projects the input features into a new feature space and the attention mechanism function $a : \mathbb{R}^{F'} \times \mathbb{R}^{F'} \rightarrow \mathbb{R}$ uses these new node features to compute an attention weight for each edge. These attention weights are typically normalized with respect to the 1-hop neighborhood of each node using the softmax function, yielding normalized attention coefficients $\alpha_{ij}$ that indicate the importance of node $i$'s input features to node $j$. For a node $j$, these normalized attention weights are then used to compute a linear combination of the new features for node $j$'s neighbors, which serves as the output of the graph attention layer for node $j$.
\begin{equation}
    \label{eqn:attn_aggr}
    \vec{h}_j' =  \sum_{i\in N_j}\alpha_{ij}\mathbf{W}\vec{h}_i
\end{equation} 
% 
To employ multi-headed attention with $K$ heads, each of the $K$ attention mechanisms first independently calculates its respective normalized weights $\alpha_{i,j}^{(k)}$ using its own attention mechanism function $a^{(k)}( \cdot )$ and linear projection weights $\mathbf{W}^{(k)}$. These attention weights are used to compute attention-head specific node outputs $\vec{h}_j'^{(k)}$, which are then averaged across the $K$ attention heads.
% \begin{equation}
%     \label{eqn:attn_heads}
%     \vec{h}_j' = \frac{1}{K}\sum_{k=1}^{K}\vec{h}_j'^{(k)}
% \end{equation}

In this paper, we focus on three widely used graph attention architectures: the original graph attention network (GAT) \citep{gat}, a modified version of this original network (GATv2) \citep{gatv2}, and the Graph Transformer network \cite{transformerconv}. These graph attention architecture variants are distinguished by the manner in which they compute the unnormalized attention weights $e_{ij}$ (Table \ref{table:gat_variants}). Here, $||$ denotes concatenation. For GAT and GATv2, the concatenated node features are passed through a single-layer feedforward neural network featuring a weight vector $\mathbf{a} \in \mathbb{R}^{2F'}$ and the LeakyReLU nonlinearity. 

\begin{table}[h!]
\centering
\caption{Attention weight calculation across graph attention architecture variants}
\label{table:gat_variants}
\renewcommand{\arraystretch}{2.5}
\begin{tabular}{  c  c  } 
    \hline
    GAT \citep{gat} & \(\displaystyle e_{ij} = \text{LeakyReLU}\big(\vec{\mathbf{a}}^T [ \mathbf{W}\vec{h}_i || \mathbf{W}\vec{h}_j \big)]\big) \)  \\
    % \hline
    GATv2 \citep{gatv2} & \(\displaystyle e_{ij} = \vec{\mathbf{a}}^T\text{LeakyReLU}\big( \mathbf{W} \vec{h}_i || \mathbf{W} \vec{h}_j \big) \) \\ 
    % \hline
    Graph Transformer \citep{transformerconv} & \(\displaystyle e_{ij} = \frac{(\mathbf{W}\vec{h}_i)^T(\mathbf{W}\vec{h}_j)}{\sqrt{F'}} \) \\ 
    \hline
\end{tabular}
\end{table}

% In the original graph attention network (GAT) framework, the unnormalized attention weights are computed as follows \citep{gat}. Here, $||$ denotes concatenation and the concatenated node features are passed through a single-layer feedforward neural network featuring a weight vector $\mathbf{a} \in \mathbb{R}^{2F'}$ and the LeakyRELU nonlinearity. 
% \begin{equation}
%     \label{eqn:gat_attn}
%     e_{ij} = \text{LeakyReLU}\big(\vec{\mathbf{a}}^T [ \mathbf{W}\vec{h}_i || \mathbf{W}\vec{h}_j \big)]\big)
% \end{equation}
% GATv2 was proposed to improve upon the expressiveness of the original graph attention mechanism by applying the linear projection to concatenated input node features instead of individual node features \citep{gatv2}.
% \begin{equation}
%     \label{eqn:gatv2_attn}
%     e_{ij} = \vec{\mathbf{a}}^T\text{LeakyReLU}\big( \mathbf{W} \vec{h}_i || \mathbf{W} \vec{h}_j \big)
% \end{equation}
% Lastly, the Graph Transformer network extends the Transformer architecture used in natural language processing \citep{transformer} to graphs and computes the attention weights as follows, where as above $F'$ is the dimensionality of the new feature space \citep{transformerconv}. 
% \begin{equation}
%     \label{eqn:transformer_attn}
%     e_{ij} = \frac{(\mathbf{W}\vec{h}_i)^T(\mathbf{W}\vec{h}_j)}{\sqrt{F'}}
% \end{equation}

\begin{figure}
    \centering
    \includegraphics[width=0.995 \linewidth ]{causal_attn_fig1_rs-v2.pdf}
    \caption{Schematic of \methodname}
    \label{fig:figure_1}
\end{figure}

\subsection{Causal Attention Regularization Scheme}

\subsubsection{Causal Attention Objective}
We propose a general-purpose regularization framework for graph attention networks that enhances a given learning task by including an attention learning scheme based on active graph interventions. In this framework, we leverage the intuition that relevant node-neighbor relations for a particular task should not only be assigned high attention weights but also be important to the predictive accuracy of the model (\textbf{Figure} \ref{fig:figure_1}). When removed from the graph, these relevant edges should cause the predictions that rely on them to dramatically worsen. We formalize this intuition by devising a an auxiliary supervised prediction task that aims to align the attention weight for an edge with the causal effect of removing that edge. The objective function for this task is as follows. 
\\
\begin{equation}
    \label{eqn:causal_reg}
    \mathcal{L}^{c} = \frac{1}{R} \sum^{R}_{r=1} \bigg( \frac{1}{\left| S^{\left( r \right )} \right|}\sum_{\left(n, i, j \right) \in S^{\left( r \right ) }} \ell^{c} \left( \alpha_{ij}^{(n)}, c_{ij}^{(n)} \right) \bigg)
\end{equation}
% \begin{equation}
%     \label{eqn:causal_reg}
%     \mathcal{L}^{c} = \frac{1}{N} \sum^{N}_{n=1} \frac{1}{\left| S^{\left( n \right )} \right|} \sum_{\left( i, j \right) \in S^{\left( n \right ) }} \ell^{c} \left( \alpha_{ij}^{(n)}, c_{ij}^{(n)} \right)
% \end{equation}

% Here, $n$ represents a single entity for which we aim to make a prediction. For a node prediction task, $n$ corresponds to a node, while in a graph prediction task, $n$ corresponds to a graph. $N$ represents the number of such entities in the training set. $\alpha_{ij}^{(n)}$ is the attention weight associated with edge $(i,j)$ for entity $n$. For models with multiple attention heads, $\alpha_{ij}^{(n)}$ is the mean attention weight for edge $(i,j)$ for entity $n$ across the attention heads. 

% $S^{(n)}$ denotes a set of edges $(i,j)$ associated with entity $n$ that will be individually removed from the training data to compute the causal effect $c_{ij}^{(n)}$. Importantly, we select only one edge per entity to remove in computing $c_{ij}^{(n)}$, so that the direct causal effect of each intervention can be calculated independently of other interventions. $\ell^c(\cdot,\cdot)$ is the loss function used to compare the attention weights and the causal effects, which we refer to as the causal regularization loss. 

Here, $n$ represents a single entity for which we aim to make a prediction. For a node prediction task, the entity $n$ corresponds to a node, and in a graph prediction task, $n$ corresponds to a graph. In each batch, we perform $R$ separate rounds of causal effect calculations, each of which consist of a set of edge interventions $S^{(r)}$, $r=1,\ldots,R$. Throughout this paper, we assume that all edges are directed and, if necessary, decompose an undirected into two directed edges. Each edge intervention in $S^{(r)}$ is represented by a set of tuples $(n,i,j)$ which denote a selected edge $(i,j)$ for an entity $n$ in round $r$. In a node classification task, $n$ is the same as $j$ (i.e., the node with the incoming edge); in a graph property-prediction task, $n$ corresponds to the graph. The causal effect $c_{ij}^{(n)}$ (\S\ref{subsec:methods:causaleffect}) scores the impact on predictive performance of deleting the edge $(i,j)$. This is compared to the attention weight $\alpha_{ij}^{(n)}$ of the edge via the loss function $\ell^c(\cdot,\cdot)$. For models with multiple attention heads, $\alpha_{ij}^{(n)}$ is the mean attention weight for edge $(i,j)$ for entity $n$ across the attention heads.

We include the above learning task as an additional task to be optimized during training so as to regularize the attention mechanism in accordance with the learned causal effects from edge interventions. Thus, our full objective function $\mathcal{L}$ includes the loss associated with the prediction $\mathcal{L}^p$, the loss associated with causal attention task $\mathcal{L}^{c}$, and a causal regularization strength hyperparameter $\lambda$ that mediates the contribution of the causal attention task to the objective.
\begin{equation}
    \label{eqn:full_objective}
    \mathcal{L} = \mathcal{L}^{p} + \lambda \mathcal{L}^{c}
\end{equation}

\subsubsection{Edge Intervention Selection}
We sample a set of edges in each round such that the prediction for each entity will strictly be affected by at most one edge intervention in that round. For example, in a node classification task for a model with one GNN layer, one round of edge interventions entails removing only a single incoming edge for each node being classified. Because a model with one GNN layer only aggregates information over a 1-hop neighborhood, the removal of each edge will only affect the model's prediction for that edge's target node. To select a set of edges in the $L$-layer GNN case, edges are sampled from the 1-hop neighborhood of each node being classified, and sampled edges that lie in more than one target nodes' $L$-hop neighborhood are removed from consideration as intervention candidates. In the graph property prediction case, only one edge will be removed from each graph per round.

This edge intervention selection procedure is crucial, as it enables the causal effect of each selected intervention $c_{ij}^{(n)}$ on an entity $n$ to be calculated independently of other interventions. Furthermore, by selecting only one intervention per entity within each round, we can parallelize the computation of these causal effects across all entities per round, enabling the causal effect calculations to be highly scalable. 

\subsubsection{Calculating Task-Specific Causal Effects}
\label{subsec:methods:causaleffect}
We quantify the causal effect of an edge intervention $c_{ij}$ on entity $n$ by evaluating the relative change in the prediction loss for entity $n$ upon removal of that edge. 
\begin{equation}
    \label{eqn:causal_effect}
    c_{ij}^{(n)} = \sigma \bigg( \bigg( \frac{\ell^p \bigl( \hat{y}_{\backslash ij}^{(n)}, y^{(n)} \bigr)} {\ell^p \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)} \bigg)^{d(n)}  -1 \bigg)
\end{equation}
% \begin{equation}
%     \label{eqn:causal_effect}
%     c_{ij}^{(n)} = \sigma \bigg( \frac{\ell^p \bigl( \hat{y}_{\backslash ij}^{(n)}, y^{(n)} \bigr)-\ell^p \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)} {\ell^p \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)} \bigg)
% \end{equation}
Here, $\ell^p(\cdot,\cdot)$ corresponds to the loss function for the given prediction task, $\hat{y}^{(n)}$ is the prediction for entity $n$, $\hat{y}_{\backslash ij}^{(n)}$ is the prediction for entity $n$ upon removal of edge $(i,j)$, and $y^{(n)}$ is the ground truth value for entity $n$. $d(n)$ scales the relative intervention effect $\ell^p \bigl( \hat{y}_{\backslash ij}^{(n)}, y^{(n)} \bigr) / \ell^p \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)$ so as to account for the abundance of edges that may contribute to the prediction of entity $n$. For example, in node classification tasks, predictions for a high-degree node will involve aggregating information over many neighbors, so the effect of a single edge intervention is adjusted via this $d(n)$ term to account for this specific node's high-degree context. As such, $d(n)$ represents the node degree for node classification, while it represents the number of edges in a graph for graph classification.  We also include $\sigma(\cdot)$ as a link function that maps its input to the support of the distribution of attention weights. The predictions $\hat{y}^{(n)}$ and $\hat{y}_{\backslash ij}^{(n)}$ are generated from the graph attention network that is being trained with \methodname. Furthermore, by using the prediction loss in these calculations, \methodname guides attention learning in a manner that is aware of the causal effects on the specific prediction task at hand. 



==> iclr2023/backup-20221113/abstract.tex <==
Graph attention networks estimate the relational importance of node neighbors to aggregate relevant information over local neighborhoods for a prediction task.
%@AW: changing this to emphasize generalizability. I'd argue we should push for the causal view as a tool, rather than an end. 
However, the inferred attentions are vulnerable to spurious correlations and connectivity in the training data, hampering the generalizability of the model. We introduce \methodname, a general-purpose regularization framework for graph attention networks. Embodying a causal inference approach, \methodname aligns the attention mechanism with the causal effects of active interventions on graph connectivity in a scalable manner.
\methodname is compatible with a variety of graph attention architectures, and we show that it systematically improves generalizability on various node classification tasks.
Our ablation studies indicate that \methodname hones in on the aspects of graph structure most pertinent to the prediction (e.g., homophily), and does so more effectively than alternative approaches.
Finally, we also show that \methodname enhances interpretability of attention weights by accentuating node-neighbor relations that point to causal hypotheses.
For social media network-sized graphs, a \methodname-guided graph rewiring approach could allow us to combine the scalability of graph convolutional methods with the higher performance of graph attention. 


==> iclr2023/backup-20221113/conclusion.tex <==
We introduced \methodname, a causally-inspired regularization scheme that can be applied to any attention based graph architecture. Applying it to both homophilic and heterophilic node-classification tasks, we found accuracy improvements and loss reductions in almost all circumstances. We performed ablation studies for a deeper understanding, and found that \methodname aligns attention with per-task homophily and does so better than a neighbor voting-based regularizer. A qualitative review also suggested that the attention-weight changes produced by \methodname are intuitive and interpretable. 

Understanding how, and improving what, GNNs learn remains a major open problem and an active area of research. Towards this, our work bridges two families of techniques: attention regularization and causal interventions. We believe this synthesis could be a promising direction of future research. Also, while our work is causally inspired, we do not currently formalize the causal foundations of our method. Future work may benefit from utilizing the tools of causal inference theory, like do-calculus \citep{pearl2021do_calculus}, for selecting and analyzing edge interventions. Lastly, while our graph pruning results are preliminary, they also suggest a promising direction for future work on scaling \methodname-based insights to web-scale graphs.

% While \methodname is not be guaranteed to uncover rigorous causal mechanisms, future research will explore extending \methodname with rigorous causal inference.

% Causality is a frequently misused term, and \methodname may not uncover rigorously causal mechanisms. However, \methodname is strongly influenced by the invariant prediction~\citep{} framework for causal inference.

==> iclr2023/backup-20221113/iclr_directions.tex <==

ICLR requires electronic submissions, processed by
\url{https://openreview.net/}. See ICLR's website for more instructions.

If your paper is ultimately accepted, the statement {\tt
  {\textbackslash}iclrfinalcopy} should be inserted to adjust the
format to the camera ready requirements.

The format for the submissions is a variant of the NeurIPS format.
Please read carefully the instructions below, and follow them
faithfully.

\subsection{Style}

Papers to be submitted to ICLR 2023 must be prepared according to the
instructions presented here.

%% Please note that we have introduced automatic line number generation
%% into the style file for \LaTeXe. This is to help reviewers
%% refer to specific lines of the paper when they make their comments. Please do
%% NOT refer to these line numbers in your paper as they will be removed from the
%% style file for the final version of accepted papers.

Authors are required to use the ICLR \LaTeX{} style files obtainable at the
ICLR website. Please make sure you use the current files and
not previous versions. Tweaking the style files may be grounds for rejection.

\subsection{Retrieval of style files}

The style files for ICLR and other conference information are available online at:
\begin{center}
   \url{http://www.iclr.cc/}
\end{center}
The file \verb+iclr2023_conference.pdf+ contains these
instructions and illustrates the
various formatting requirements your ICLR paper must satisfy.
Submissions must be made using \LaTeX{} and the style files
\verb+iclr2023_conference.sty+ and \verb+iclr2023_conference.bst+ (to be used with \LaTeX{}2e). The file
\verb+iclr2023_conference.tex+ may be used as a ``shell'' for writing your paper. All you
have to do is replace the author, title, abstract, and text of the paper with
your own.

The formatting instructions contained in these style files are summarized in
sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.

\section{General formatting instructions}
\label{gen_inst}

The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).
Use 10~point type with a vertical spacing of 11~points. Times New Roman is the
preferred typeface throughout. Paragraphs are separated by 1/2~line space,
with no indentation.

Paper title is 17~point, in small caps and left-aligned.
All pages should start at 1~inch (6~picas) from the top of the page.

Authors' names are
set in boldface, and each name is placed above its corresponding
address. The lead author's name is to be listed first, and
the co-authors' names are set to follow. Authors sharing the
same address can be on the same line.

Please pay special attention to the instructions in section \ref{others}
regarding figures, tables, acknowledgments, and references.


There will be a strict upper limit of 9 pages for the main text of the initial submission, with unlimited additional pages for citations. 

\section{Headings: first level}
\label{headings}

First level headings are in small caps,
flush left and in point size 12. One line space before the first level
heading and 1/2~line space after the first level heading.

\subsection{Headings: second level}

Second level headings are in small caps,
flush left and in point size 10. One line space before the second level
heading and 1/2~line space after the second level heading.

\subsubsection{Headings: third level}

Third level headings are in small caps,
flush left and in point size 10. One line space before the third level
heading and 1/2~line space after the third level heading.

\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone, regardless of the formatter being used.

\subsection{Citations within the text}

Citations within the text should be based on the \texttt{natbib} package
and include the authors' last names and year (with the ``et~al.'' construct
for more than two authors). When the authors or the publication are
included in the sentence, the citation should not be in parenthesis using \verb|\citet{}| (as
in ``See \citet{Hinton06} for more information.''). Otherwise, the citation
should be in parenthesis using \verb|\citep{}| (as in ``Deep learning shows promise to make progress
towards AI~\citep{Bengio+chapter2007}.'').

The corresponding references are to be listed in alphabetical order of
authors, in the \textsc{References} section. As to the format of the
references themselves, any style is acceptable as long as it is used
consistently.

\subsection{Footnotes}

Indicate footnotes with a number\footnote{Sample of the first footnote} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches
(12~picas).\footnote{Sample of the second footnote}

\subsection{Figures}

All artwork must be neat, clean, and legible. Lines should be dark
enough for purposes of reproduction; art work should not be
hand-drawn. The figure number and caption always appear after the
figure. Place one line space before the figure caption, and one line
space after the figure. The figure caption is lower case (except for
first word and proper nouns); figures are numbered consecutively.

Make sure the figure caption does not get separated from the figure.
Leave sufficient space to avoid splitting the figure and figure caption.

You may use color figures.
However, it is best for the
figure captions and the paper body to make sense if the paper is printed
either in black/white or in color.
\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
\end{center}
\caption{Sample figure caption.}
\end{figure}

\subsection{Tables}

All tables must be centered, neat, clean and legible. Do not use hand-drawn
tables. The table number and title always appear before the table. See
Table~\ref{sample-table}.

Place one line space before the table title, one line space after the table
title, and one line space after the table. The table title must be lower case
(except for first word and proper nouns); tables are numbered consecutively.

\begin{table}[t]
\caption{Sample table title}
\label{sample-table}
\begin{center}
\begin{tabular}{ll}
\multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION}
\\ \hline \\
Dendrite         &Input terminal \\
Axon             &Output terminal \\
Soma             &Cell body (contains cell nucleus) \\
\end{tabular}
\end{center}
\end{table}

\section{Default Notation}

In an attempt to encourage standardized notation, we have included the
notation file from the textbook, \textit{Deep Learning}
\cite{goodfellow2016deep} available at
\url{https://github.com/goodfeli/dlbook_notation/}.  Use of this style
is not required and can be disabled by commenting out
\texttt{math\_commands.tex}.


\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}



\section{Final instructions}
Do not change any aspects of the formatting parameters in the style files.
In particular, do not modify the width or length of the rectangle the text
should fit into, and do not change font sizes (except perhaps in the
\textsc{References} section; see below). Please note that pages should be
numbered.

\section{Preparing PostScript or PDF files}

Please prepare PostScript or PDF files with paper size ``US Letter'', and
not, for example, ``A4''. The -t
letter option on dvips will produce US Letter files.

Consider directly generating PDF files using \verb+pdflatex+
(especially if you are a MiKTeX user).
PDF figures must be substituted for EPS figures, however.

Otherwise, please generate your PostScript and PDF files with the following commands:
\begin{verbatim}
dvips mypaper.dvi -t letter -Ppdf -G0 -o mypaper.ps
ps2pdf mypaper.ps mypaper.pdf
\end{verbatim}

\subsection{Margins in LaTeX}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+
from the graphicx package. Always specify the figure width as a multiple of
the line width as in the example below using .eps graphics
\begin{verbatim}
   \usepackage[dvips]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.eps}
\end{verbatim}
or % Apr 2009 addition
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
for .pdf graphics.
See section~4.4 in the graphics bundle documentation (\url{http://www.ctan.org/tex-archive/macros/latex/required/graphics/grfguide.ps})

A number of width problems arise when LaTeX cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command.

\subsubsection*{Author Contributions}
If you'd like to, you may include  a section for author contributions as is done
in many journals. This is optional and at the discretion of the authors.

\subsubsection*{Acknowledgments}
Use unnumbered third level headings for the acknowledgments. All
acknowledgments, including those to funding agencies, go at the end of the paper.

==> iclr2023/backup-20221113/intro.tex <==
Graphs encode rich relational information that can be leveraged in learning tasks across a wide variety of domains. Graph neural networks (GNNs) can learn powerful node, edge or graph-level representations by aggregating a node's representations with that of its neighbors. 
%Graph neural networks (GNNs) have demonstrated considerable promise in recent years by using these graph relations to supplement node representations with information from node neighbors.
%However, t
The specifics of a GNN's neighborhood aggregation scheme are critical to its effectiveness on a prediction task.
For instance, graph convolutional networks (GCNs) aggregate information via a simple averaging or max-pooling of neighbor features. 
%\citep{gcn_kipf_welling,graphsage}.
While GCNs scales well, they are also indiscriminate. GCNs are prone to suffer in many real-world scenarios where uninformative or noisy connections exist between nodes \citep{gcn_kipf_welling,graphsage}. GCNs may also over-smooth, with nodes in a graph taking on indistinguishable representations due to the indiscriminate aggregation operation \citep{gcn_oversmoothing,measuring_oversmoothing,topping2022understanding}. 

Graph-based attention mechanisms combat these issues by quantifying the relevance of node-neighbor relations and softly selecting neighbors in the aggregation step accordingly \citep{gat,gatv2,transformerconv}. This process of attending to select neighbors has contributed to significant performance gains for GNNs across a variety of tasks \citep{gnn_review, 2022message}. Similar to the use of attention in natural language processing and computer vision, attention in graph settings also enables the interpretability of model predictions via the examination of attention weights \citep{attn_interpret,attn_review}. 

Paramount to the effectiveness of attention mechanisms in GNNs is their ability to discern the specific graph connectivity patterns that underlie accurate, generalizable predictions. %As graph training data often contains noisy features and/or connections,
Attention mechanisms in GNNs can be sensitive to spurious edges and correlations that mislead them in how they attend to node neighbors, which manifests as a failure to generalize to unseen data \citep{attn_review}. One approach to improve the GNN's generalizability is to regularize the attention weights so they become more robust to spurious correlations/connections in the training data. Previous work along this direction has focused on $L_0$ regularization of attention weights to enforce sparsity \citep{ye2021sparse} or has co-optimized a link prediction side-task using the attention mechanism\citep{kim2021how}. Since these regularization strategies are formulated independently of the actual prediction task, they align the attention mechanism with some intrinsic property of the input graph without regard for the training objective. 
%Some of the previous work is also specific to the kind of graph attention mechanism chosen. 
% the inability of attention mechanisms to select the appropriate node neighbors also suggests an inability to determine the graph connections that causally contribute to a particular prediction.

We take a different approach. We begin our study with the question: ``What is the importance of a specific edge to the prediction task?'' Our answer comes from the perspective of regularization: we introduce \methodname, a causal attention regularization framework that is suitable for any graph attention network architecture (\textbf{Figure}~\ref{fig:figure_1}). Intuitively, an edge in the input graph is important to a prediction task if removing it leads to substantial degradation in the prediction performance of the GNN. The key conceptual advance of this work is to scalably leverage active interventions on node neighborhoods (i.e., deletion of specific edges) to align graph attention training with the causal impact of these interventions on task performance. While some efforts have previously been made to infuse notions of causality into GNNs, these causal approaches have been largely limited to using causal effects from pre-trained models as features for a separate model \citep{trust_neigh,attn_review} or decoupling causal from non-causal effects \citep{causal_attn_graph}. Causality is a frequently misused term, and \methodname may not uncover rigorously causal mechanisms. Nonetheless, \methodname is strongly influenced by the invariant prediction~\citep{RePEc:bla:jorssb:v:78:y:2016:i:5:p:947-1012} framework for causal inference.

Our work builds on previous findings \citep{attn_review} that an explicit focus on improving attention weights can pay rich dividends. We apply \methodname on three graph attention architectures across eight node classification
% and \RS{ X other graph property-prediction} 
tasks each, finding that it consistently improves test loss and accuracy. Our causal regularization fine-tunes attention weights by aligning them with task-specific homophily. In contrast, a non-causal label-propagation approach can also pick up on homophily but is task-agnostic and generalizes less well. On the ogbn-arxiv network, we investigate the citations up/down-weighted by \methodname and found them to broadly group into three intuitive themes. Our causal approach can thus enhance the interpretability of attention weights, and we provide a qualitative analysis of this improved interpretability. We also present preliminary results demonstrating the applicability of \methodname to graph property prediction and graph pruning tasks. 
%Lastly, by applying it on sample sub-networks for a large social media-sized network, \methodname can enable us to learn the attention weights that would generalize to the broader network. 
Due to the size of industrially relevant graphs, it is common to use GCNs or sampling-based approaches on them. There, using attention weights learned by \methodname on sampled subnetworks may guide graph rewiring of the full network to improve the results obtained with convolutional techniques. %while retaining scalability.

%Understanding how, and improving what, GNNs learn remains a major open problem and an active area of research. Towards this, our work bridges two families of techniques (attention regularization and causal interventions) which we believe could be a promising direction of future research. 

% performance gains
% intepretability
% issues: spurious correlations (training data size?, training data network connectivity), limitations of interpretability
% sensitivity to initialization

% themes:
% graph attention
% determining relevant neighbors
% causal modeling: interventions ("causal view of robustness...", "matching learned causal effects...")
% causal attention
% causal regularization: KDD paper + ICML paper (causal effects domain priors)
% 

==> iclr2023/backup-20221113/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> iclr2023/backup-20221113/related_work.tex <==
The performance gains associated with graph attention networks have led to a number of efforts to enhance and better understand graph attention mechanisms \citep{gat_survey}. One category of methods aims to improve the expressive power of graph attention mechanisms by supplementing a given prediction objective with a supervised attention mechanism~\citep{trust_neigh}, or a self-supervised connectivity prediction approach~\citep{kim2021how}. A related set of methods leverage signals from interventions on graphs from a causal perspective to aid in training GNNs. One class of techniques performs interventions on the nodes~\citep{attn_review, trust_neigh}. Meanwhile, other methods such as CAL~\citep{causal_attn_graph} or CFLP~\citep{2106.02172} augment the loss by adding additional tasks intended to separate causal and non-causal effects.

Our intervention-oriented framework can also be understood as a graph structure perturbation method. Perturbation methods can be broadly split into three different categories: graph data augmentation~\citep{2202.08871}, structural graph rewiring~\citep{DBLP:conf/iclr/RongHXH20}, and geometric graph rewiring~\citep{topping2022understanding}. Inspired by the success of data augmentation approaches in computer vision, graph data augmentation methods seek to generate new training samples through different augmentation techniques. One of the earliest methods is DropEdge~\citep{DBLP:conf/iclr/RongHXH20} reduces overfitting by randomly selecting edges from a uniform distribution to delete . Other methods build on DropEdge and select edges according to additional constraints including geometrical invariants~\citep{gao2021training}, target probability distributions~\citep{NEURIPS2021_9e7ba617}, and information criteria~\citep{suresh2021adversarial}. Structural graph rewiring instead seeks to enforce structural priors such as sparsity or homophily during the graph alteration phase. Examples of these rewiring priors include fairness~\citep{2201.08549, 9645324}, temporal structure~\citep{NEURIPS2021_0b0b0994}, predicted homophily~\citep{measuring_oversmoothing}, sparsity\citep{10.1145/3394486.3403049, pmlr-v119-zheng20d}, or information transfer efficiency~\citep{10.5555/3454287.3455484}. Geometric approaches, instead, choose to view the graph as a discrete geometry and alter the connectivity according to the balanced Forman curvature~\citep{topping2022understanding}, the stochastic discrete Ricci flows~\citep{2207.08026}, commute times~\citep{2206.07369}, or algebraic connectivity\citep{2206.07369}. All of these approaches are designed either for use either in self-supervised learning or in a task-agnostic fashion, and consider the input graph independently of the task at hand.

To summarize, \methodname introduces a combination of advances not previously reported: applicability to diverse attention architectures; task-based supervised regularization (rather than task-agnostic or self-supervised regularization) that leads to improved generalization; and a causal approach that directly relates an edge's importance to its attention weight, enhancing interpretability. % A key innovation of our design is an edge selection scheme for performing multiple interventions in parallel, ensuring scalability. 

% Unlike these approaches, \methodname takes a more direct and interpretable approach to graph perturbation, and applies this to node classification and graph property prediction. \methodname achieves this by supervising the attention weights through active interventions on sampled edges during training. The active intervention framework directly enables the measurement of the individual treatment effect, so that we can perform task-specific casual regularization of the attention weights for arbitrary attention-based models. While \methodname can be understood through the lens of graph sparsification, \methodname does not seek to explicitly alter the edge connectivity through structural perturbations that may be deleterious to generalization. Moreover, \methodname alters the underlying geometry in \textit{task specific} ways.

% Unlike these approaches, \methodname takes a more direct and interpretable approach to graph perturbation, and applies this to node classification and graph property prediction. \methodname achieves this by supervising the attention weights by active interventions on sampled edges during training. The active intervention framework directly enables the measurement of the individual treatment effect, so that we can perform task-specific casual regularization of the attention weights for arbitrary attention-based models.

% The performance gains associated with graph attention networks have led to a number of efforts to enhance and better understand graph attention mechanisms \citep{gat_survey}. One category of methods aims to improve the expressive power of graph attention mechanisms by supplementing a given prediction objective with one or more tasks. \cite{attn_review} found that adding the supervised training of attention as an auxiliary task dramatically improved classification accuracy and that classification accuracy depended exponentially on attention correctness in their experiments. Such settings with ground truth attention are rare, though, so alternative tasks have been proposed to learn better attention weights. For example, SuperGAT adds an edge self-supervision task that is task-agnostic, using the connectivity patterns of existing edges in a graph to inform the assignment of attention weights to edges \citep{kim2021how}.

% A related set of methods leverage signals from interventions on graphs to aid in training GNNs. \cite{attn_review} devised an auxiliary weakly-supervised attention learning task based on changes in a pre-trained GCN's predictions that stem from node-level interventions. Causal GCN Inference (CGI) uses the outcomes of node-level interventions on a pre-trained GCN as well but as features in a classifier rather than as a means of informing attention \citep{trust_neigh}. Meanwhile, the Causal Attention Learning (CAL) strategy \citep{causal_attn_graph} aims to decouple causal and non-causal effects by introducing an additional task that encourages robustness to abstract interventions on graph representations rather than specific nodes or edges. Unlike these approaches, \methodname takes a more direct and interpretable approach, supervising the attention weights by active interventions on sampled edges during training and measuring the causal effect on the prediction task.

% Perhaps the method most comparable to ours is CFLP~\citep{2106.02172}, which treats an edge's existence as an individual treatment effect and constructs a causal model to predict the average treatment effect directly. However, it differs from \methodname substantially, both in application and approach. \methodname uses an estimate of the individual treatment effect to regularize the attention weights for arbitrary attention-based models, rather than alter the data distribution that is used for training. Additionally, CFLP is aimed at link-prediction which requires positional, rather than structural, representations~\citep{Srinivasan2020On}, whereas our work is aimed at node and graph classification for which structural representations are sufficient.

% % Graph data augmentation
% Inspired by the success of data augmentation approaches in computer vision, graph perturbations have also found their use in graph data augmentation~\cite{2202.08871}. In DropEdge~\citep{DBLP:conf/iclr/RongHXH20}, edges are randomly deleted in subgraph samples to reduce overfitting. Dropping edges indiscriminately can result in pathological examples that limit generalization. 
% TADropEdge~\citep{gao2021training} seeks to limit this effect by drawing edges according to topological invariants. MH-Aug~\cite{NEURIPS2021_9e7ba617} instead uses Metropolis-Hastings to generate new training examples through a set of graph mutation rules. 
% AD-GCL~\cite{suresh2021adversarial} constructs a contrastive learning framework to drop edges by minimizing the information lost by dropping each edge. All of these approaches are designed either for self-supervised learning (e.g., AD-GCL) or in a task-agnostic fashion (e.g., DropEdge), distinguishing them from \methodname. % This is done to increase generalization by reducing the number of repeated structural features that are learned.

% % Graph Rewiring

% Many methods have explored graph rewiring as a way to improve inferential accuracy, predictive performance, or improve generalization. GDC~\cite{10.5555/3454287.3455484} seeks to improve information diffusion while reducing noise through densification and then sparsification steps. In an attempt to debias learned representations, FairAug~\cite{2201.08549} and FairDrop~\cite{9645324} remove edges according to a defined fairness metric. MeTa~\cite{NEURIPS2021_0b0b0994} generates new subgraphs through temporal edge-sampling, and then learns to pass messages between temporally distinct subgraphs. This method has clear causal intuition, but without the interventional semantic of \methodname. The AdaEdge method~\cite{measuring_oversmoothing}, supervised edge-perturbation is performed through multiple full-training runs where the graph is rewired to optimize for predicted-homophily.

% % Graph Geometry
% \RS{@TM: ok if we kill/shrink this paragraph if we are still running short on space?}
% Another related set of methods have observed that intrinsic properties of the graph, such as sparsity or curvature, can be leveraged to rewire the graph to increase task generalization. Pro-GNN\cite{10.1145/3394486.3403049} co-learns a GNN and a sparsified graph structure to build methods that are robust to external perturbation. Sparsification is learned through structural optimization of the adjacency matrix. Similar to \methodname, NeuralSparse~\cite{pmlr-v119-zheng20d} seeks to sparsify by removing task-irrelevant edges. NeuralSparse, however, chooses to do so by learning a generative distribution over graph perturbations. Moving beyond sparsification, work based on the balanced Forman curvature~\cite{topping2022understanding} rewires the graph to improve information flow through the graph, which yielded state of the art performance on a variety of benchmarks. This idea is pushed further in by Bober \textit{et al.}~\cite{2207.08026} where they view a graph as a discrete geometry and use tools for discrete differential geometry. Alternatively, DiffWire~\cite{2206.07369} presents two different GCN layers: CT and GAP that are fully differentiable and optimize graph connectivity according to commute times or the algebraic connectivity. While \methodname can be understood through the lens of graph sparsification, \methodname does not seek to explicitly alter the edge connectivity through structural perturbations that may be deleterious to generalization. Moreover, \methodname alters the underlying geometry in \textit{task specific} ways.


% \RS{@TM/AW: new paragraph, pls check} To summarize, \methodname introduces a combination of advances not previously reported: applicability to diverse attention architectures; task-based supervised regularization (rather than task-agnostic or self-supervised regularization) leading to improved generalization; and a causal approach that directly relates an edge's importance to its attention weight, enhancing interpretability. A key innovation of our design is an edge selection scheme for performing multiple interventions in parallel, ensuring scalability. 


% edge-level interventions
% during training (accounts for ability of GAT to adjust weights of neighbors vs. indiscriminate pooling as in GCNs)

% \noindent \textbf{Attention in GNNs:}

% \noindent \textbf{Graph Attention Regularization:} 

% self-supervised learning: friendly neighbors
% weakly supervised learning: graph attention generalization (attention over nodes, intervention w/ weak supervision)
% causal: granger-causal attentive mixtures of experts, trust neighbors?
% l0 regularization: ye2021 - graph rewiring too

% \cite{attn_review} found that, in cases where ground-truth attention is available, supervised training of attention contributed to improved generalization performance of models to unseen and noisy graph inputs. 

% Hence, efforts have been made to design graph attention through supplementing learning tasks with self-supervision \cite{friendly_neigh} or by .

% using causal effects from pre-trained models as features for a separate model \citep{trust_neigh} or decoupling causal from non-causal effects \citep{causal_attn_graph}. To our knowledge, no efforts have . 

% graph attention
% graph causal modeling
% causal explanations
% causal regularization (graph domain priors, CAL) + supervised attention

==> iclr2023/backup-20221113/reproducibility.tex <==
To ensure the reproducibility of the results in this paper, we have included the source code for our method as supplementary materials. The datasets used in this paper are all publicly available, and we also use the publicly available train/validation/test splits for these datasets. We provide details on these datasets in the Appendix and have provided references to them in both the main text and the Appendix. In addition, we have provided detailed descriptions of the experimental setup, model training schemes, model architecture design choices, and hyperparameter choices in the ``Experimental Setup'' section as well as in Appendix \ref{appen:arch_hyper}.


==> iclr2023/backup-20221113/results.tex <==
\subsection{Experimental Setup}
We assessed the effectiveness of \methodname across a diverse set of prediction tasks, datasets, graph attention mechanisms, and hyperparameter choices. We evaluated \methodname on 8 node classification tasks (also see additional applications in \S \ref{subsec:methods:investigation}).
%and \RS{Y graph property prediction datasets (Y1 regression tasks, Y2 classification tasks)}. 
We used a simple network architecture, choosing  $L=1$ or $L=2$ graph attention layers positioned between single-layer feed-forward networks (\textbf{Appendix} \ref{appen:arch_hyper}). For each model, the PyTorch Geometric \citep{pyg} implementation of one of GAT, GATv2, or Graph Transformer was used as the graph attention mechanism \citep{gat,gatv2,transformerconv}. 

To establish \methodname's robustness to hyperparameter choices, we evaluated \methodname across a broad range of hyperparameter settings, rather than selecting specific hyperparameters for each model configuration.
%employing a hyperparameter selection scheme for each model configuration. 
The number of attention heads was selected from $k=\{1,3,5\}$; the regularization strength was from $\lambda=\{0.1,0.5,1,5\}$; and the number of hidden features used across layers were from $F'=\{10,25,100,200\}$. See \textbf{Appendix} \ref{appen:arch_hyper} for details on the network architecture, hyperparameters, and training configurations. 

We used cross-entropy loss for the prediction loss $\ell^p(\cdot,\cdot)$ and binary cross-entropy loss for the causal regularization loss $\ell^c(\cdot,\cdot)$. The link function $\sigmoid(\cdot)$ was chosen to be the sigmoid function with temperature $T=0.1$. Unless otherwise specified, we performed $R=5$ rounds of edge interventions per mini-batch when training with \methodname. 

\subsection{Node Classification}
\noindent \textbf{Datasets and evaluation:} We used a total of 8 real-world node classification datasets of varying sizes and degrees of homophily: Cora, CiteSeer, PubMed, ogbn-arxiv, Chameleon, Squirrel, Cornell and Wisconsin. Each model was evaluated according to its accuracy on a held-out test set. We also evaluated the test cross-entropy loss, as it accounts for the full distribution of per-class predictions rather than just the highest-valued prediction considered in accuracy calculations. See \textbf{Appendix} \ref{appen:node_class_datasets} for details on dataset statistics, splits, and references. Runtimes for training models with \methodname ranged from roughly 2 seconds to 5 minutes on the evaluated datasets, with \methodname's runtime only 1.5-2 times that of standard training on average (see \textbf{Appendix} \ref{appen:runtime_memory} for details). 

\noindent \textbf{Generalization performance:} We compared both the test accuracy and the test loss of each model when trained with and without \methodname. Across all model architecture and hyperparameter choices for a dataset, we applied the one-tailed paired Wilcoxon signed-rank test to quantify the overall outperformance of models trained with \methodname against models trained without it. \methodname resulted in higher test accuracy in 7 of the 8 node classification datasets and a lower test loss in all 8 datasets (\textbf{Figure} \ref{fig:figure_2}, $p < 0.05$). We also report the relative performance when averaging over all hyperparameter choices in \textbf{Table}~\ref{table:loss_results} (test loss) and \textbf{Table}~\ref{table:acc_results} (test accuracy, in Appendix \ref{appen:node_class_acc}). These results highlight the consistency of performance gains achieved with \methodname across the space of graph attention mechanisms and hyperparameters evaluated. 
% HERE: number of interventions per node?

% \AW{do we want to condense the accuracy and loss tables into one table with just the mean values of each? we can then show the full tables with the standard deviations in the appendix.}

\begin{table}[ht]
\caption{Test loss on 8 node classification datasets}
\label{table:loss_results}
\centering
\small
\renewcommand{\arraystretch}{1.5}
\begin{center}
\resizebox{14cm}{!}{%
\begin{tabular}{l c c c c c c c c }
    & \textbf{Cora} & \textbf{CiteSeer} & \textbf{PubMed} & \textbf{ogbn-arxiv} & \textbf{Chameleon} & \textbf{Squirrel} & \textbf{Cornell} & \textbf{Wisconsin} \\
    \hline
    GAT &  2.33 $\pm$ 0.75 & 3.68 $\pm$ 2.64 & 1.05 $\pm$ 0.24 & 1.49 $\pm$ 0.02 & 1.29 $\pm$ 0.03 & 1.48 $\pm$ 0.02 & 1.19 $\pm$ 0.23 & 0.88 $\pm$ 0.11  \\
    % \hline
    GAT + \methodname & \textbf{1.82 $\pm$ 0.77} & \textbf{3.06 $\pm$ 2.34} & \textbf{0.89 $\pm$ 0.18} & 1.49 $\pm$ 0.02 & \textbf{1.26 $\pm$ 0.03} & \textbf{1.47 $\pm$ 0.02} & \textbf{1.14 $\pm$ 0.17} & \textbf{0.84 $\pm$ 0.13} \\
    \hline
    GATv2 &  2.26 $\pm$ 0.54 & 3.08 $\pm$ 1.06 & 1.07 $\pm$ 0.29 & 1.48 $\pm$ 0.02 & 1.28 $\pm$ 0.03 & 1.48 $\pm$ 0.02 & 1.09 $\pm$ 0.11 & 0.88 $\pm$ 0.15 \\
    GATv2 + \methodname & \textbf{1.63 $\pm$ 0.59} & \textbf{3.04 $\pm$ 2.07} & \textbf{0.90 $\pm$ 0.17} & \textbf{1.47 $\pm$ 0.03} & \textbf{1.24 $\pm$ 0.03} & \textbf{1.46 $\pm$ 0.02} & \textbf{1.04 $\pm$ 0.10} & \textbf{0.81 $\pm$ 0.09} \\
    \hline
    Transformer & 3.43 $\pm$ 1.61 & 9.78 $\pm$ 8.27 & 1.79 $\pm$ 0.88 & 1.50 $\pm$ 0.03 & 1.38 $\pm$ 0.06 & 1.50 $\pm$ 0.02 & 1.22 $\pm$ 0.25 & 1.03 $\pm$ 0.28 \\
    Transf.\ + \methodname & \textbf{1.71 $\pm$ 0.50} & \textbf{3.92 $\pm$ 2.25} & \textbf{1.60 $\pm$ 0.59} & 1.50 $\pm$ 0.03 & \textbf{1.33 $\pm$ 0.04} & \textbf{1.48 $\pm$ 0.03} & \textbf{1.07 $\pm$ 0.12} & \textbf{0.86 $\pm$ 0.13} \\ 
    \hline
\end{tabular}}
\end{center}
\end{table}


\subsection{Model Investigation and Ablation Studies}
\label{subsec:methods:investigation}
%%\RS{points to make: a) \methodname accentuates correlation with homophily, more so for heterophilic networks [label agreement result?]; b) effect of hyperparameter $\lambda$ (b.1: violin plot; b.2: dialed-up/down cora homophily)  c) an ablation where label propagation was directly used to regularize also helps but not as much as \methodname, esp for heterophilic networks; \sout{d) random edge ablation?}}

\paragraph{Impact of regularization strength} 
We explored 4 settings of $\lambda$: $\{0.1, 0.5, 1, 5\}$. For 6 of the 8 node classification datasets, \methodname models trained with the higher causal regularization strengths ($\lambda=1,\,5$) demonstrated significantly larger reductions in test loss ($p < 0.05$, one-tailed Welch's $t$-test) compared to those trained with weaker regularization ($\lambda=0.1,\,0.5$). Notably, all four of the datasets with lower homophily (Chamelon, Squirrel, Cornell and Wisconsin) displayed significantly larger reductions with the higher regularization strengths, suggesting that stronger regularization may contribute to improved generalization in such settings (\textbf{Appendix} \ref{appen:compare_loss_lambda}).

%\noindent \textbf{Selecting $\lambda$ for \methodname in multi-layer GNNs:} (still include?)

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.995 \linewidth ]{fig2_causal_comparison_node.pdf}
    \caption{Test accuracy and negative loss on 8 node classification datasets. Each point corresponds to a comparison between a baseline model trained without \methodname and an identical model trained with \methodname. The point size represents the magnitude of the $\lambda$ value chosen for the \methodname-trained model. $p$-values are computed from one-tailed paired Wilcoxon signed-rank tests evaluating the improvement of \methodname-trained models over the baseline models.}
    \label{fig:figure_2}
\end{figure}



\paragraph{Connection to homophily} %{Label agreement} 
For the node classification task, the relevant neighbors to a particular node are expected to be those that share the same label as that node. We assessed if the graph attention mechanisms in models trained with \methodname more effectively prioritized such relevant edges. For each edge, we used the label agreement between nodes connected by it as a proxy for the edge's ground-truth relevance: specifically, we assigned a reference attention weight $\ell_{ij}$ to an edge based on the label agreement in the target node's neighborhood \citep{kim2021how}.
\begin{equation}
    \label{eqn:label_agreement}
    \ell_{ij} = \hat{\ell}_{ij}/\sum_{k\in N_j} \hat{\ell}_{kj}
\end{equation}
Here, $\hat{\ell}_{ij} = 1$ if nodes $i$ and $j$ have the same label $\hat{\ell}_{ij} = 0$ otherwise. $N_j$ denotes the in-neighbors of node $j$. We then calculate the KL divergence of an edge's attention weight $\alpha_{i,j}$ from its reference attention weight $\ell_{ij}$ and summarize a model's ability to identify relevant edges as the mean of these KL divergence values across the edges in the held-out test set. 

We compared these mean KL divergences between baseline models trained without \methodname and models trained with \methodname across the same broad range of model architecture and hyperparameter choices described above. We found that \methodname-trained models consistently yielded lower mean KL divergence values than models trained without \methodname  for 6 of 8 node classification datasets (\textbf{Figure }\ref{fig:figure_3},$p < 0.05$, one-tailed paired Wilcoxon signed-rank test). 

% The improvement in AP for \methodname-trained models was particularly pronounced for the Chameleon and Squirrel datasets, which are characterized by lower homophily, while the higher homophily datasets (Cora, CiteSeer, PubMed) were not associated with such gains (Appendix \ref{appen:label_agreement_homophily}). 
Notably, this enhanced prioritization of relevant edges was achieved without explicitly optimizing label agreement during training and is an inherent manifestation of aligning attention with the node classification tasks' causal effects. 
% In addition, this result highlights the applicability of \methodname for low homophily graphs, as graph attention is essential in such settings due to the relative dissimilarity of neighboring nodes in these graphs. 
Thus, these results demonstrate that \methodname not only improves performance on node classification tasks but also more accurately prioritizes the edges that are most relevant to the task at hand. 

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.8 \linewidth ]{fig3_label_agreement.pdf}
    \caption{Coherence between attention weights and label agreement for \methodname-trained models, compared to baseline. Lower KL divergence implies greater coherence. Point colors and sizes have the same meaning as in Figure \ref{fig:figure_2}. $p$-values are computed from one-tailed paired Wilcoxon signed-rank tests evaluating the improvement of \methodname-trained models over the baseline models.}
    \label{fig:figure_3}
\end{figure}

\paragraph{Comparison to neighbor voting-based regularization} 
%We also evaluated the degree to which aligning attention mechanisms with their causal effects contributed to this improved generalization performance. 
We wondered if the performance gains by our causal approach could be achieved by a non-causal approach that simply aligns the attention weights with a generic measure of homophily. To evaluate this, we employed a similar regularization scheme to that of \methodname (\textbf{Equation} \ref{eqn:causal_effect}) but decoupled the causal effect calculation from the specific network being trained. Instead of using predictions from the network to determine the causal effect, we used predictions from a neighbor voting model, in which each node's classification prediction is a histogram of class labels from the node's neighbors. In this neighbor voting regularization scheme, the attention mechanism for the network being trained is thus guided during training by the effects of edge interventions to this neighbor voting model's predictions rather than by the effects of edge interventions to the network's own predictions. 

% Separately, we also we simply draw each causal effect $c_{i,j}^{(n)}$ from a uniform distribution on the interval $[0,1)$ 

We compared \methodname-trained models with those trained with neighbor voting regularization by evaluating the consistency of their test loss improvements relative to the baseline models without regularization. We used the one-tailed paired Wilcoxon signed-rank test to evaluate the significance of the regularized models' test loss improvements across the set of model architecture and hyperparameter choices, focusing on models trained with the higher $\lambda=1$ or $\lambda=5$ regularization strengths. Models trained when regularizing attention weights with the neighbor voting scheme underperformed those trained with \methodname in 7 of the 8 datasets (\textbf{Table} \ref{table:ablation}). Interestingly, the neighbor voting-based regularization showed an overall gain in performance relative to the baseline models (i.e., those trained without any regularization), suggesting that even non-specific regularization can be somewhat useful for training attention. Overall, these results demonstrate the effectiveness of using \methodname to improve generalization performance for many node classification tasks.

\begin{table}[h!]
\smallskip
\centering
\caption{Generalization performance of \methodname-trained models with ablations compared to baseline \\($-\log_{10}(p)$, one-tailed paired Wilcoxon signed-rank test)}
\label{table:ablation}
\renewcommand{\arraystretch}{1.8}
\resizebox{14cm}{!}{%

\begin{tabular}{ r  c  c  c  c  c  c  c  c } 
    % \multirow{3}{*}{\bf Method}  &\multicolumn{2}{c}{\bf Cora} &\multicolumn{2}{c}{\bf CiteSeer} &\multicolumn{2}{c}{\bf PubMed} &\multicolumn{2}{c}{\bf orgn-arxiv} &\multicolumn{2}{c}{\bf Chameleon} &\multicolumn{2}{c}{\bf Squirrel} \\ 
    & \textbf{Cora} & \textbf{CiteSeer} & \textbf{PubMed} & \textbf{ogbn-arxiv} & \textbf{Chameleon} & \textbf{Squirrel} & \textbf{Cornell} & \textbf{Wisconsin} \\
    % \cmidrule(lr){2-3}\cmidrule(lr){3-4}\cmidrule(lr){5-6}
    \hline
    \methodname & \textbf{12.36} & \textbf{5.92} & \textbf{10.51} & \textbf{1.81} & \textbf{12.77} & 9.72 & \textbf{6.72} & \textbf{9.34} \\
    % \hline
    Neighbor Voting &  10.04 & 5.59 & 7.30 & 0.53 & 12.34 & \textbf{10.97} & 4.15 & 8.20 \\
    \hline
    % \methodname & \textbf{8.99} & \textbf{4.34} & \textbf{7.81} & \textbf{0.655} & \textbf{10.84} & 9.56 & \textbf{3.84} & \textbf{6.24} \\
    % % \hline
    % Neighbor Voting & 8.89 & 3.62 & 4.78 & 0.233 & 9.20 & 10.84 & 2.28 & 5.30 \\
    % \hline
    % Random & X & X & X & X & X & X \\
\end{tabular}}
\end{table}


% \begin{table}[h!]
% \centering
% \caption{\methodname-trained graph attention mechanisms attend to homophilous edges in node classification}
% \label{table:attn_homophily}
% \renewcommand{\arraystretch}{2.5}
% \begin{tabular}{ c  c  c  c  c  c  c } 
%     & Cora & CiteSeer & PubMed & ogbn-arxiv & Chameleon & Squirrel \\
%     % \cmidrule(lr){2-3}\cmidrule(lr){3-4}\cmidrule(lr){5-6}
%     \hline
%     Baseline & 0.81 \pm 0.01 & 0.76 \pm 0.01 & 0.81 \pm 0.01 & 0.70 \pm 0.01 &  \\
%     \hline
%     Baseline & 0.81 \pm 0.01 & 0.76 \pm 0.01 & 0.81 \pm 0.01 & 0.70 \pm 0.01 & 
% \end{tabular}
% \end{table}


% \subsubsection{Cheeger Constant}
% \TM{Do we have results here? Because the graphs are all disconnected, this might be difficult to interpret.}
% Next, we turn our attention to a series of experiments intended to understand the topological changes that our graph undergoes due to our causal regularization method. 

% Because our method prunes edges, we are specifically interested in understanding whether our method is introducing bottlenecks that would make us more susceptible to over-squashing. To answer this question, we compute Cheeger constant as a function of regularization strength for the Cora dataset.

% Furthermore, we computed the curvature of the original graph, pruned graph, and removed edges; and present the kernel density estimates below.

% \subsubsection{Graph Diffusion Distance}
% \TM{Do we have results here? It feels like a nice to have but probably a P1/P2 priority.}
% Next, we are interested to understand whether our proposed method is simply removing edges that are ``topologically noisy''. To answer this question, we have computed the graph diffusion distance defined as

% \begin{equation}
%  d^{(u,v)}_{GDD}(A_1, A_2) = \sqrt{ \argmax_{t} \left | \left |  e^{-t L}  - e^{-t L\backslash ({u,v}) } \right | \right |^2_F},
% \end{equation}

% where $L$ is the graph Laplacian, and $L\backslash ({u,v})$ is the graph Laplacian with the edge from $u$ to $v$ deleted. We use this metric because it provides a global measure of graph diffusion, which is intimately connected to message passing.

\paragraph{Additional applications}
To explore the utility of \methodname as a general-purpose framework, we employed \methodname in two additional tasks: graph property prediction and graph pruning. For graph property prediction, we evaluated \methodname on ogbg-molbace, a dataset for binary classification, and ogbg-molfreesolv, which features a regression task \citep{ogb}. We trained models with \methodname across a broad range of graph attention mechanisms and hyperparameter choices. For both datasets, we found that \methodname-trained models consistently outperformed those that were trained without \methodname ($p < 0.05$, one-tailed paired Wilcoxon signed-rank test, see \textbf{Appendix} \ref{appen:graph_property_pred} for details).

We also explored a graph pruning approach that uses attention weights from \methodname-trained models to remove task-irrelevant edges. In particular, we used this edge pruning procedure as a pre-processing step for training and inference with GCNs, which are more scalable than graph attention networks \citep{sign} but indiscriminate in how they aggregate information over node neighborhoods. We found that using \methodname-guided pruning was able to improve the test accuracy of GCNs not only relative to GCNs trained and evaluated over the full graph but also outperformed GCNs trained and evaluated with non-regularized (i.e. baseline) graph attention mechanisms (\textbf{Appendix} \ref{appen:graph_rewiring}). These preliminary results open the door for further exploration of \methodname's applicability on these tasks.


\subsection{Interpreting Attention Weights: Qualitative Analysis}
\label{subsec:results:qa}
%Previous perturbative approaches to guide GNN training did not directly intervene on edges in a task-specific way, making their interpretability less clear.
In addition to providing a robust way to increase both model quality and generalization, \methodname learns attention weights that are more interpretable in a \textit{post hoc} analysis. Here, we explored the edge-wise difference of the attention values between our method and a baseline GAT applied to the \textrm{ogbn-arxiv} dataset. In this dataset, nodes represent computer science arXiv papers, edges are citation links between these papers, and the prediction task is to classify papers into their subject areas. We manually reviewed citations that were up/down-weighted by \methodname-trained models and observed that these citations broadly fit into one of three categories:  (i) down-weighting self-citations, (ii) down-weighting popular ``anchor'' papers, or (iii) upweighting topically-narrow papers with few citations.

In the first case, we found that \methodname down-weights edges associated with self-citations (see \textbf{Table}~\ref{tab:self-cites} for examples). The causal story here is quite clear--- machine learning is a fast-moving field with authors moving into the field and changing specialties as those specialties are born. Because of this, the narrative arc that a set of authors constructs to present this idea can include citations to their own previous work from different subfields. While these citations do help situate the work within the broader literature and can provide background that readers might find valuable, they are not relevant to the subject area prediction task. 

\begin{table}[ht]
\small
\caption{\label{tab:self-cites}Down-weighted self-citations. }
\renewcommand{\arraystretch}{1.5}
\begin{center}
\begin{tabular}{p{0.42\linewidth} p{0.42\linewidth} p{0.10\linewidth}}
Paper Title & Cited Title (from a different subject area) & $\Delta$ \\
 \hline 
\textit{Viterbinet a Deep Learning Based Viterbi Algorithm for Symbol Detection} &
\textit{Frequency Shift Filtering for Ofdm Signal Recovery in Narrowband Power Line Communications} & -89.91 \% \\
% \smallskip \\
\textit{Solving Underdetermined Systems with Error Correcting Codes} &
\textit{Systems of MDS Codes from Units and Idempotents} & -89.80 \% \\
% \smallskip \\
\textit{Performance Analysis for Multichannel Reception of OOFSK Signaling} &
\textit{On-Off Frequency-Shift Keying for Wideband Fading Channels} & -81.03 \% \\
\end{tabular}
\end{center}
\end{table}

In the second case, we found that \methodname down-weights edges directed towards popular or otherwise seminal ``anchor'' papers (\textbf{Table}~\ref{tab:anchor-cites}). These papers tends to be included in introductions to provide references for common concepts or methods, such as Adam, ResNet, and ImageNet. They are also widely cited across subject areas and hence have little bearing on the subject area prediction task.

Notably, \methodname does not simply learn to ignore edges from high-degree nodes. In the example of the Word2Vec paper, we observed notable increases in attention weights for edges connecting it to multiple highly related papers, including a $2.5\times 10^6$ \% increase for \textit{Efficient Graph Computation for Node2Vec} and a $2.0\times 10^6$ \% increase for \textit{Multi-Dimensional Explanation of Reviews	}.


% Table of down-weighted papers
\begin{table}[th]
\small
\caption{\label{tab:anchor-cites}Down-weighted citations of ``anchor'' papers. Each of the cited works that is down-weighted is a well known ML paper.}
\renewcommand{\arraystretch}{1.5}
\begin{center}
\begin{tabular}{p{0.42\linewidth} p{0.42\linewidth} p{0.10\linewidth}}
Paper Title & Cited Title & $\Delta$ \\
\hline
\textit{Reservoir Computing Hardware with Cellular Automata} &
\textit{Adam: A Method for Stochastic Optimization} &
-99.87\% \\
\textit{Quantization Networks} &
\textit{Deep Residual Learning for Image Recognition} &
-99.86\% \\
%\smallskip \\
%\smallskip \\
% Submodular Hamming Metrics &
% Distributed Representations of Sords and Phrases and Their Compositionality &
% -99.92\% \\
\textit{Compressive Hyperspherical Energy Minimization} &
\textit{ImageNet Large Scale Visual Recognition Challenge} &
-99.75\% \\
\end{tabular}
\end{center}
\end{table}


In the final case, we observed that \methodname up-weighted edges directed towards deeply related but largely unnoticed papers (\textbf{Table}~\ref{tab:up-cites}). In our manual exploration of the data, we observed that these papers are those that are close to the proposed method. These papers are the type that are often found only after a thorough literature review. Clearly, such edges should play a key role in predicting a paper's topic and should be up-weighted.


==> iclr2023/backup-20221113/theory.tex <==
\subsection{Graph Attention Networks}

Attention mechanisms have been effectively used across many domains by enabling models to dynamically attend to the specific parts of an input that are most relevant to a prediction task \citep{attention_survey}. In graph settings, attention mechanisms compute the relevance of node-neighbor relations, as denoted by the edges of the graph. The neighbor aggregation operator in GNNs then uses this information to weight the contribution of each edge in the prediction task. 

Across the multitude of graph attention mechanisms that have been proposed \citep{gat_survey}, the procedures for computing attention share a general form \citep{gat}. A graph attention layer takes as input a set of node features $\mathbf{h} = \{\vec{h}_1,...,\vec{h}_N\}$, $\vec{h}_i \in \mathbb{R}^F$, where $N$ is the number of nodes and $F$ is the dimensionality of the node features. From these node features, the graph attention layer in a GAT computes unnormalized attention weights for each edge $(i,j)$
\begin{equation}
    \label{eqn:attn_edges}
    e_{ij} = a(\mathbf{W}\vec{h}_i,\mathbf{W}\vec{h}_j),
\end{equation}
where $\mathbf{W}\in \mathbb{R}^{F' \times F}$ linearly projects the input features into a new feature space and the attention mechanism function $a : \mathbb{R}^{F'} \times \mathbb{R}^{F'} \rightarrow \mathbb{R}$ uses these new node features to compute an attention weight for each edge. These attention weights are typically normalized with respect to the 1-hop neighborhood of each node using the softmax function, yielding normalized attention coefficients $\alpha_{ij}$ that indicate the importance of node $i$'s input features to node $j$. For a node $j$, these normalized attention weights are then used to compute a linear combination of its neighbors' features.

\begin{equation}
    \label{eqn:attn_aggr}
    \vec{h}_j' =  \sum_{i\in N_j}\alpha_{ij}\mathbf{W}\vec{h}_i,
    ~ ~ \mathit{s.t.} ~ 
    \sum_{i\in N_j} \alpha_{ij} = 1
\end{equation} 
% 
To employ multi-headed attention with $K$ heads, each of the $K$ attention mechanisms first independently calculates its respective normalized weights $\alpha_{i,j}^{(k)}$ using its own attention mechanism function $a^{(k)}( \cdot )$ and linear projection weights $\mathbf{W}^{(k)}$. The head-specific node outputs are then averaged. 
%RS: commenting out to save some space and make room for causal in the intro
%
%se attention weights are used to compute attention-head specific node outputs $\vec{h}_j'^{(k)}$, which are then averaged across the $K$ attention heads.
%
% \begin{equation}
%     \label{eqn:attn_heads}
%     \vec{h}_j' = \frac{1}{K}\sum_{k=1}^{K}\vec{h}_j'^{(k)}
% \end{equation}

In this paper, we focus on three widely used graph attention architectures: the original graph attention network (GAT) \citep{gat}, a modified version of this original network (GATv2) \citep{gatv2}, and the Graph Transformer network \citep{transformerconv}. %These graph attention architecture variants are distinguished by the manner in which they compute the unnormalized attention weights $e_{ij}$ (Table \ref{table:gat_variants}). 
The three architectures and their equations for computing attention  are presented in \textbf{Table} \ref{table:gat_variants}. Here, $||$ denotes concatenation. 

\begin{table}[h!]
\centering
\caption{Attention weight calculation across graph attention architecture variants}
\label{table:gat_variants}
\renewcommand{\arraystretch}{2}
\begin{tabular}{  c  c  } 
    \hline
    GAT \citep{gat} & \(\displaystyle e_{ij} = \text{LeakyReLU}\big(\vec{\mathbf{a}}^T [ \mathbf{W}\vec{h}_i || \mathbf{W}\vec{h}_j \big)]\big) \)  \\
    % \hline
    GATv2 \citep{gatv2} & \(\displaystyle e_{ij} = \vec{\mathbf{a}}^T\text{LeakyReLU}\big( \mathbf{W} \vec{h}_i || \mathbf{W} \vec{h}_j \big) \) \\ 
    % \hline
    Graph Transformer \citep{transformerconv} & \(\displaystyle e_{ij} = \frac{(\mathbf{W}\vec{h}_i)^T(\mathbf{W}\vec{h}_j)}{\sqrt{F'}} \) \\ 
    \hline
\end{tabular}
\end{table}

% In the original graph attention network (GAT) framework, the unnormalized attention weights are computed as follows \citep{gat}. Here, $||$ denotes concatenation and the concatenated node features are passed through a single-layer feedforward neural network featuring a weight vector $\mathbf{a} \in \mathbb{R}^{2F'}$ and the LeakyRELU nonlinearity. 
% \begin{equation}
%     \label{eqn:gat_attn}
%     e_{ij} = \text{LeakyReLU}\big(\vec{\mathbf{a}}^T [ \mathbf{W}\vec{h}_i || \mathbf{W}\vec{h}_j \big)]\big)
% \end{equation}
% GATv2 was proposed to improve upon the expressiveness of the original graph attention mechanism by applying the linear projection to concatenated input node features instead of individual node features \citep{gatv2}.
% \begin{equation}
%     \label{eqn:gatv2_attn}
%     e_{ij} = \vec{\mathbf{a}}^T\text{LeakyReLU}\big( \mathbf{W} \vec{h}_i || \mathbf{W} \vec{h}_j \big)
% \end{equation}
% Lastly, the Graph Transformer network extends the Transformer architecture used in natural language processing \citep{transformer} to graphs and computes the attention weights as follows, where as above $F'$ is the dimensionality of the new feature space \citep{transformerconv}. 
% \begin{equation}
%     \label{eqn:transformer_attn}
%     e_{ij} = \frac{(\mathbf{W}\vec{h}_i)^T(\mathbf{W}\vec{h}_j)}{\sqrt{F'}}
% \end{equation}

\begin{figure}
    \centering
    %\includegraphics[width=0.95 \linewidth ]{iclr2023/causal_attn_fig1_rs-v4.pdf}
    \includegraphics[width=0.95 \linewidth ]{car_regularization_overview.pdf}
    \caption{Schematic of \methodname: Graph attention networks learn the relative importance of each node-neighbor for a given prediction task. However, their inferred attention weights can be miscalibrated due to noise, spurious correlations, or confounders (e.g., node size here). Our causal approach directly intervenes on a sampled subset of edges and supervises an auxiliary task that aligns an edge's causal importance to the task with its attention weight.}
    \label{fig:figure_1}
\end{figure}

\subsection{Causal Attention Regularization Scheme}

\paragraph{Causal attention objective}
We leverage the intuition that relevant node-neighbor relations for a particular task should not only be assigned high attention weights but also be important to the predictive accuracy of the model (\textbf{Figure} \ref{fig:figure_1}). When removed from the graph, these relevant edges should cause the predictions that rely on them to substantially worsen. We formalize this intuition by devising an auxiliary supervised prediction task that aims to align the attention weight for an edge with the causal effect of removing that edge as per the following loss function:
\begin{equation}
    \label{eqn:causal_reg}
    \mathcal{L}^{c} = \frac{1}{R} \sum^{R}_{r=1} \bigg( \frac{1}{\left| S^{\left( r \right )} \right|}\sum_{\left(n, i, j \right) \in S^{\left( r \right ) }} \ell^{c} \left( \alpha_{ij}^{(n)}, c_{ij}^{(n)} \right) \bigg)
\end{equation}
% \begin{equation}
%     \label{eqn:causal_reg}
%     \mathcal{L}^{c} = \frac{1}{N} \sum^{N}_{n=1} \frac{1}{\left| S^{\left( n \right )} \right|} \sum_{\left( i, j \right) \in S^{\left( n \right ) }} \ell^{c} \left( \alpha_{ij}^{(n)}, c_{ij}^{(n)} \right)
% \end{equation}

% Here, $n$ represents a single entity for which we aim to make a prediction. For a node prediction task, $n$ corresponds to a node, while in a graph prediction task, $n$ corresponds to a graph. $N$ represents the number of such entities in the training set. $\alpha_{ij}^{(n)}$ is the attention weight associated with edge $(i,j)$ for entity $n$. For models with multiple attention heads, $\alpha_{ij}^{(n)}$ is the mean attention weight for edge $(i,j)$ for entity $n$ across the attention heads. 

% $S^{(n)}$ denotes a set of edges $(i,j)$ associated with entity $n$ that will be individually removed from the training data to compute the causal effect $c_{ij}^{(n)}$. Importantly, we select only one edge per entity to remove in computing $c_{ij}^{(n)}$, so that the direct causal effect of each intervention can be calculated independently of other interventions. $\ell^c(\cdot,\cdot)$ is the loss function used to compare the attention weights and the causal effects, which we refer to as the causal regularization loss. 

Here, $n$ represents a single entity for which we aim to make a prediction. For a node prediction task, the entity $n$ corresponds to a node, and in a graph prediction task, $n$ corresponds to a graph. In each batch, we perform $R$ separate rounds of causal effect calculations, each of which consists of a set of edge interventions $S^{(r)}$, $r=1,\ldots,R$. Throughout this paper, we assume that all edges are directed and, if necessary, decompose an undirected edge into two directed edges. Each edge intervention in $S^{(r)}$ is represented by a set of tuples $(n,i,j)$ which denote a selected edge $(i,j)$ for an entity $n$ in round $r$. Note that in a node classification task, $n$ is the same as $j$ (i.e., the node with the incoming edge). The causal effect $c_{ij}^{(n)}$ (see below) scores the impact on predictive performance of deleting the edge $(i,j)$. This is compared to the edge's attention weight $\alpha_{ij}^{(n)}$ via the loss function $\ell^c(\cdot,\cdot)$. For models with multiple attention heads, $\alpha_{ij}^{(n)}$ is the mean attention weight across the heads.

We regularize the attention mechanism in accordance with the learned causal effects from edge interventions. Thus, our full objective function $\mathcal{L}$ includes the loss associated with the prediction $\mathcal{L}^p$, the loss associated with causal attention task $\mathcal{L}^{c}$, and a causal regularization strength hyperparameter $\lambda$ that mediates the contribution of the causal attention task to the objective.
\begin{equation}
    \label{eqn:full_objective}
    \mathcal{L} = \mathcal{L}^{p} + \lambda \mathcal{L}^{c}
\end{equation}

\paragraph{Edge intervention procedure} %Selection}
We sample a set of edges in each round such that the prediction for each entity will strictly be affected by at most one edge intervention in that round. For example, in a node classification task for a model with one GNN layer, a round of edge interventions entails removing only a single incoming edge for each node being classified. In the graph property prediction case, only one edge will be removed from each graph per round. Because a model with one GNN layer only aggregates information over a 1-hop neighborhood, the removal of each edge will only affect the model's prediction for that edge's target node. To select a set of edges in the $L$-layer GNN case, edges are sampled from the 1-hop neighborhood of each node being classified, and sampled edges that lie in more than one target nodes' $L$-hop neighborhood are removed from consideration as intervention candidates. We note that in practice GNNs usually have $L \leq 2$ layers since greater depth increases the computational cost and the risk of oversmoothing~\citep{gcn_oversmoothing,measuring_oversmoothing,topping2022understanding}. %; this limits the computational expense of interventions. 

This edge intervention selection procedure is crucial, as it enables the causal effect of each selected intervention $c_{ij}^{(n)}$ on an entity $n$ to be calculated independently of other interventions. By selecting only one intervention per entity within each round, we can parallelize the computation of these causal effects across all entities per round, aiding scalability. 
 
\paragraph{Calculating task-specific causal effects}
\label{subsec:methods:causaleffect}
We quantify the causal effect of an intervention at edge $(i,j)$ on entity $n$ as the relative change in the prediction loss for entity $n$ upon removal of that edge.
% \begin{equation}
%     \label{eqn:causal_effect}
%     c_{ij}^{(n)} = \sigma \bigg( \bigg( \frac{\ell^p \bigl( \hat{y}_{\backslash ij}^{(n)}, y^{(n)} \bigr)} {\ell^p \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)} \bigg)^{d(n)}  -1 \bigg)
% \end{equation}

\begin{equation}
    \label{eqn:causal_effect}
    c_{ij}^{(n)} = \sigma \bigg( \bigg( \rho^{(n)}_{ij} \bigg)^{d(n)} - 1 \bigg)\;\;\;\text{where}\;\; \rho^{(n)}_{ij} = \frac{\ell^p \bigl( \hat{y}_{\backslash ij}^{(n)}, y^{(n)} \bigr)} {\ell^p \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)}
\end{equation}

% \begin{equation}
%     \label{eqn:causal_effect}
%     c_{ij}^{(n)} = \sigma \bigg( \frac{\ell^p \bigl( \hat{y}_{\backslash ij}^{(n)}, y^{(n)} \bigr)-\ell^p \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)} {\ell^p \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)} \bigg)
% \end{equation}
Here, $\ell^p(\cdot,\cdot)$ corresponds to the loss function for the given prediction task, $\hat{y}^{(n)}$ is the prediction for entity $n$, $\hat{y}_{\backslash ij}^{(n)}$ is the prediction for entity $n$ upon removal of edge $(i,j)$, and $y^{(n)}$ is the ground truth value for entity $n$. Here, $d(n)$ represents the node degree for node classification, while it represents the number of edges in a graph for graph classification. Since attention weights for each node sum to 1, per-edge attention weights are expected to be smaller for higher-degree nodes. Exponentiating the relative intervention effect $\rho^{(n)}_{ij}$ by $d(n)$ is intended to adjust for this.
% $\ell^p \bigl( \hat{y}_{\backslash ij}^{(n)}, y^{(n)} \bigr) / \ell^p \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)$ so as to account for the number of edges contributing to the prediction for entity $n$. For example, in node classification tasks, predictions for a high-degree node will involve aggregating information over many neighbors, so the effect of a single edge intervention is adjusted via this $d(n)$ term to account for this specific node's high-degree context. 
The link function $\sigma(\cdot)$ maps its input to the support of the distribution of attention weights. The predictions $\hat{y}^{(n)}$ and $\hat{y}_{\backslash ij}^{(n)}$ are generated from the graph attention network being trained with \methodname. We emphasize that they are both computed during the same training run, rather than in two separate runs. 

% \RS{@AW: the two y's are computed in a single run, right? pls clarify that as a line here?}
% \AW{added another sentence. is this what you mean?}
% %Furthermore, by using the prediction loss in these calculations, \methodname guides attention learning in a manner that is aware of the causal effects on the specific prediction task at hand. 

\paragraph{Scalability}
\methodname increases the computational cost of training in two ways: (i) additional evaluations of the loss function, and (ii) searches to ensure independent interventions. \methodname performs $\mathcal{O}(R |V| )$ interventions, where $R$ is the number of interventions per vertex, and $|V|$ is the cardinality of the vertex set. Each intervention requires a $L$-layer deep BFS, with complexity $\mathcal{O}(b^L)$, where $L$ is the depth of the GNN, and $b$ is the mean in-degree. While this carries a worst case time-complexity of $\mathcal{O}(R |V| b^L)$, in practice, we are able to mitigate much of the computational cost by parallelizing the intervention-overlap checks using the edge selection procedure above. Furthermore, the identification of non-overlapping interventions can also be done as a preprocessing step. 
%We have found \methodname to be highly scalable, with training runtimes that are only 1.5-2x of non-regularized attention training (Appendix \ref{appen:runtime_memory}).
In summary, we have found \methodname to have a modest effect on the scalability of graph attention methods, with training runtimes that are only increased by 1.5-2 fold (\textbf{Appendix} \ref{appen:runtime_memory}).

% \TM{ Number of interventions scales as $O(C * |V|)$. Each intervention scales as $O(b^2l)$ due to the BFS to ensure non-overlapping interventions, where b is the branching factor and l is the number of layers. In the long run, we're unconcerned about the identification of non-overlapping interventions can be done as a preprocessing step, similar to the generation of graph samples in graph sage.}


==> iclr2023/backup-20221113/todos.tex <==
\todo[inline]{
Todos: \\
1. P0 Results: \\
 \;\; - \sout{Abstract: need a summary stat or two} \\
 \;\; - Ablations: a) in appendix: need table of correlations between attn wts and homophily scores. b) put in line markers for what random baseline will be \\ 
 \;\; - \sout{Ablations: need label-propagation results} \\
 \;\; - Scalability: need runtimes and machine details \\
2. P0 Writing: \\
 \;\; - \sout{Interpretability: which dataset? \TM{ogbn-arxiv}} \\
3. P1 Results: \\
 \;\; - Fig 3: needs other 3 datasets (in appendix). Also needs p-values \\
 \;\; - Extra: graph property-prediction + graph rewiring. Ok to have limited examples \\
 \;\; - random/uniform regularization 
 \;\; - Should we worry about graph diffusion distance and cheeger constant stuff? Could be a solid appendix section

}


==> iclr2023/backup-20221113/v1_theory.tex <==
\subsection{Graph Attention Networks}

Attention mechanisms have been effectively used across many domains by enabling models to dynamically attend to the specific parts of an input that are most relevant to a prediction task \citep{attention_survey}. In graph settings, attention mechanisms compute the relevance of node-neighbor relations. The neighbor aggregation operator in GNNs then uses this information to weight the contribution of each node-neighbor relation in the prediction task. 

Across the multitude of graph attention mechanisms that have been proposed \citep{gat_survey}, the procedures for computing attention take on a general form \citep{gat}. A graph attention layer takes as input a set of node features $\mathbf{h} = \{\vec{h}_1,...,\vec{h}_N\}$, $\vec{h}_i \in \mathbb{R}^F$, where $N$ is the number of nodes and $F$ is the dimensionality of the node features. From these node features, the graph attention layer in a GAT computes unnormalized attention weights for each edge $(i,j)$
\begin{equation}
    \label{eqn:attn_edges}
    e_{ij} = a(\mathbf{W}\vec{h}_i,\mathbf{W}\vec{h}_j),
\end{equation}
where $\mathbf{W}\in \mathbb{R}^{F' \times F}$ linearly projects the input features into a new feature space and the attention mechanism function $a : \mathbb{R}^{F'} \times \mathbb{R}^{F'} \rightarrow \mathbb{R}$ uses these new node features to compute an attention weight for each edge. These attention weights are typically normalized with respect to the 1-hop neighborhood of each node using the softmax function, yielding normalized attention coefficients $\alpha_{ij}$ that indicate the importance of node $i$'s input features to node $j$. For a node $j$, these normalized attention weights are then used to compute a linear combination of the new features for node $j$'s neighbors, which serves as the output of the graph attention layer for node $j$.
\begin{equation}
    \label{eqn:attn_aggr}
    \vec{h}_j' =  \sum_{i\in N_j}\alpha_{ij}\mathbf{W}\vec{h}_i
\end{equation} 
% 
To employ multi-headed attention with $K$ heads, each of the $K$ attention mechanisms first independently calculates its respective normalized attention weights $\alpha_{i,j}^{(k)}$ using its own attention mechanism function $a^{(k)}( \cdot )$ and linear projection weights $\mathbf{W}^{(k)}$. These attention weights are used to compute attention head-specific node outputs $\vec{h}_j'^{(k)}$, which are then averaged across the $K$ attention heads.
\begin{equation}
    \label{eqn:attn_heads}
    \vec{h}_j' = \frac{1}{K}\sum_{k=1}^{K}\vec{h}_j'^{(k)}
\end{equation}

In this paper, we focus on three widely used graph attention architectures: the original graph attention network (GAT) \citep{gat}, a modified version of this original network (GATv2) \citep{gatv2}, and the Graph Transformer network \cite{transformerconv}. These graph attention architecture variants are distinguished by the manner in which they compute the unnormalized attention weights $e_{ij}$ (Table \ref{table:gat_variants}). Here, $||$ denotes concatenation. For GAT and GATv2, the concatenated node features are passed through a single-layer feedforward neural network featuring a weight vector $\mathbf{a} \in \mathbb{R}^{2F'}$ and the LeakyReLU nonlinearity. 

\begin{table}[h!]
\centering
\caption{Attention weight calculation across graph attention architecture variants}
\label{table:gat_variants}
\renewcommand{\arraystretch}{2.5}
\begin{tabular}{ | c | c |} 
    \hline
    GAT \citep{gat} & \(\displaystyle e_{ij} = \text{LeakyReLU}\big(\vec{\mathbf{a}}^T [ \mathbf{W}\vec{h}_i || \mathbf{W}\vec{h}_j \big)]\big) \)  \\
    \hline
    GATv2 \citep{gatv2} & \(\displaystyle e_{ij} = \vec{\mathbf{a}}^T\text{LeakyReLU}\big( \mathbf{W} \vec{h}_i || \mathbf{W} \vec{h}_j \big) \) \\ 
    \hline
    Graph Transformer \citep{transformerconv} & \(\displaystyle e_{ij} = \frac{(\mathbf{W}\vec{h}_i)^T(\mathbf{W}\vec{h}_j)}{\sqrt{F'}} \) \\ 
    \hline
\end{tabular}
\end{table}

% In the original graph attention network (GAT) framework, the unnormalized attention weights are computed as follows \citep{gat}. Here, $||$ denotes concatenation and the concatenated node features are passed through a single-layer feedforward neural network featuring a weight vector $\mathbf{a} \in \mathbb{R}^{2F'}$ and the LeakyRELU nonlinearity. 
% \begin{equation}
%     \label{eqn:gat_attn}
%     e_{ij} = \text{LeakyReLU}\big(\vec{\mathbf{a}}^T [ \mathbf{W}\vec{h}_i || \mathbf{W}\vec{h}_j \big)]\big)
% \end{equation}
% GATv2 was proposed to improve upon the expressiveness of the original graph attention mechanism by applying the linear projection to concatenated input node features instead of individual node features \citep{gatv2}.
% \begin{equation}
%     \label{eqn:gatv2_attn}
%     e_{ij} = \vec{\mathbf{a}}^T\text{LeakyReLU}\big( \mathbf{W} \vec{h}_i || \mathbf{W} \vec{h}_j \big)
% \end{equation}
% Lastly, the Graph Transformer network extends the Transformer architecture used in natural language processing \citep{transformer} to graphs and computes the attention weights as follows, where as above $F'$ is the dimensionality of the new feature space \citep{transformerconv}. 
% \begin{equation}
%     \label{eqn:transformer_attn}
%     e_{ij} = \frac{(\mathbf{W}\vec{h}_i)^T(\mathbf{W}\vec{h}_j)}{\sqrt{F'}}
% \end{equation}

\subsection{Causal Attention Regularization Scheme}

We propose a general-purpose regularization framework for graph attention networks that enhances a given learning task by including an attention learning scheme based on active graph interventions. In this framework, we leverage the intuition that relevant node-neighbor relations for a particular task should not only be assigned high attention weights but also be important to the predictive accuracy of the model. When removed from the graph, these relevant edges should cause the predictions that rely on them to dramatically worsen. 

\subsubsection{Causal Attention Objective}
We formalize this intuition by devising a weakly supervised prediction task that aims to align the attention weight for an edge with the causal effect of removing that edge. The objective function for this task is as follows. 
\\
\begin{equation}
    \label{eqn:causal_reg}
    \mathcal{L}^{c} = \frac{1}{R} \sum^{R}_{r=1} \frac{1}{\left| S^{\left( r \right )} \right|}\sum_{\left(n, i, j \right) \in S^{\left( r \right ) }} \ell^{c} \left( \alpha_{ij}^{(n)}, c_{ij}^{(n)} \right)
\end{equation}
% \begin{equation}
%     \label{eqn:causal_reg}
%     \mathcal{L}^{c} = \frac{1}{N} \sum^{N}_{n=1} \frac{1}{\left| S^{\left( n \right )} \right|} \sum_{\left( i, j \right) \in S^{\left( n \right ) }} \ell^{c} \left( \alpha_{ij}^{(n)}, c_{ij}^{(n)} \right)
% \end{equation}

% Here, $n$ represents a single entity for which we aim to make a prediction. For a node prediction task, $n$ corresponds to a node, while in a graph prediction task, $n$ corresponds to a graph. $N$ represents the number of such entities in the training set. $\alpha_{ij}^{(n)}$ is the attention weight associated with edge $(i,j)$ for entity $n$. For models with multiple attention heads, $\alpha_{ij}^{(n)}$ is the mean attention weight for edge $(i,j)$ for entity $n$ across the attention heads. 

% $S^{(n)}$ denotes a set of edges $(i,j)$ associated with entity $n$ that will be individually removed from the training data to compute the causal effect $c_{ij}^{(n)}$. Importantly, we select only one edge per entity to remove in computing $c_{ij}^{(n)}$, so that the direct causal effect of each intervention can be calculated independently of other interventions. $\ell^c(\cdot,\cdot)$ is the loss function used to compare the attention weights and the causal effects, which we refer to as the causal regularization loss. 

Here, $n$ represents a single entity for which we aim to make a prediction. For a node prediction task, $n$ corresponds to a node, while in a graph prediction task, $n$ corresponds to a graph. We perform $R$ rounds of edge interventions per mini-batch, sampling a set of edges in each round such that the prediction for each entity in the mini-batch will strictly be affected by at most one edge intervention in that round. For example, in a node classification task for a model with one GNN layer, one round of edge interventions for a mini-batch entails removing only a single incoming edge for each node being classified in the mini-batch. Because a model with one GNN layer only aggregates information over a 1-hop neighborhood, the removal of each edge will only affect the model's prediction for that edge's target node. Similarly, in the graph property prediction case, only one edge will be removed from each graph per round. $S^{(r)}$ denotes a set of tuples $(n,i,j)$, each of which corresponds to a selected edge $(i,j)$ for an entity $n$ in round $r$. 

This edge intervention selection procedure is crucial, as it enables the direct causal effect of each selected intervention $c_{ij}^{(n)}$ on an entity $n$ to be calculated independently of other interventions. Furthermore, by selecting only one intervention per entity within each round, we can parallelize the computation of these direct causal effects across all entities per round, enabling the causal effect calculations to be highly scalable. Each causal effect $c_{ij}^{(n)}$ is compared to the attention weight $\alpha_{ij}^{(n)}$ of its corresponding edge via the loss function $\ell^c(\cdot,\cdot)$. For models with multiple attention heads, $\alpha_{ij}^{(n)}$ is the mean attention weight for edge $(i,j)$ for entity $n$ across the attention heads.

We quantify the causal effect $c_{ij}$ of removing edge $(i,j)$ on the prediction for entity $n$ as follows. 
\begin{equation}
    \label{eqn:causal_effect}
    c_{ij}^{(n)} = \sigma \bigg( \frac{\ell \bigl( \hat{y}_{\backslash ij}^{(n)}, y^{(n)} \bigr)-\ell \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)} {\ell \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)} \bigg)
\end{equation}
% talk about importance of using prediction loss to compute causal effect instead of just change in predictions???
$\ell^p(\cdot,\cdot)$ corresponds to the loss function for the given prediction task, $\hat{y}^{(n)}$ is the prediction for entity $n$, $\hat{y}_{\backslash ij}^{(n)}$ is the prediction for entity $n$ upon removal of edge $(i,j)$, and $y^{(n)}$ is the ground truth value for entity $n$. We also include $\sigma(\cdot)$ as a link function that maps its input to the support of the distribution of attention weights. 

We include the above learning task as an additional task to be optimized during training so as to regularize the attention mechanism in accordance with the learned causal effects from edge interventions. Thus, our full objective function $\mathcal{L}$ includes the loss associated with the prediction $\mathcal{L}^p$, the loss associated with causal attention task $\mathcal{L}^{c}$, and a causal regularization strength hyperparameter $\lambda$ that mediates the contribution of the causal attention task to the objective.
\begin{equation}
    \label{eqn:full_objective}
    \mathcal{L} = \mathcal{L}^{p} + \lambda \mathcal{L}^{c}
\end{equation}

==> iclr2023/backup-20230214/abstract.tex <==
Graph attention networks estimate the relational importance of node neighbors to aggregate relevant information over local neighborhoods for a prediction task.
%@AW: changing this to emphasize generalizability. I'd argue we should push for the causal view as a tool, rather than an end. 
However, the inferred attentions are vulnerable to spurious correlations and connectivity in the training data, hampering the generalizability of models. We introduce \methodname, a general-purpose regularization framework for graph attention networks. Embodying a causal inference approach based on invariance prediction, \methodname aligns the attention mechanism with the causal effects of active interventions on graph connectivity in a scalable manner.
\methodname is compatible with a variety of graph attention architectures, and we show that it systematically improves generalizability on various node classification tasks.
Our ablation studies indicate that \methodname hones in on the aspects of graph structure most pertinent to the prediction (e.g., homophily), and does so more effectively than alternative approaches.
Finally, we also show that \methodname enhances interpretability of attention coefficients by accentuating node-neighbor relations that point to causal hypotheses.
% For social media network-sized graphs, a \methodname-guided graph rewiring approach could allow us to combine the scalability of graph convolutional methods with the higher performance of graph attention. 


==> iclr2023/backup-20230214/conclusion.tex <==
We introduced \methodname, an invariance principle-based causal regularization scheme that can be applied to graph attention architectures. Unlike other invariance-based approaches \citep{graph_ood}, our focus is on scalably improving overall generalization rather than handling distribution shifts. Towards that, we introduce an efficient scheme to directly intervene on multiple edges in parallel. Applying it to both homophilic and heterophilic node-classification tasks, we found accuracy improvements and loss reductions in almost all circumstances. We performed ablation studies for a deeper understanding, and found that \methodname aligns attention with task-specific homophily and does so better than a homophily-based regularizer. A qualitative review also suggested that the attention-weight changes produced by \methodname are intuitive and interpretable. 

Understanding how, and improving what, GNNs learn remains a major open problem and is an active area of research. For instance, \cite{heterophily} have discussed the challenges that GNNs face when handling low-homophily graphs or when different tasks could be specified on the same underlying graph (e.g., predicting citation year vs. topic in obgn-arxiv). Towards this, our method provides a principled and scalable approach to align attention coefficients with the relevant task. Our work bridges two families of techniques: attention regularization and causal interventions. The synthesis of these techniques is not only a promising direction for enhancing the performance and interpretability of graph attention but also opens the door for leveraging similar techniques for general GNNs without attention as well.
%In addition, while our work is causally inspired, we do not currently formalize the causal foundations of our method. Future work may benefit from utilizing the tools of causal inference theory, like do-calculus \citep{pearl2021do_calculus}, for selecting and analyzing edge interventions. 
Lastly, while our graph pruning results are preliminary, they also suggest a promising direction for future work on scaling \methodname-based insights to web-scale graphs.

% While \methodname is not be guaranteed to uncover rigorous causal mechanisms, future research will explore extending \methodname with rigorous causal inference.

% Causality is a frequently misused term, and \methodname may not uncover rigorously causal mechanisms. However, \methodname is strongly influenced by the invariant prediction~\citep{} framework for causal inference.

==> iclr2023/backup-20230214/iclr_directions.tex <==

ICLR requires electronic submissions, processed by
\url{https://openreview.net/}. See ICLR's website for more instructions.

If your paper is ultimately accepted, the statement {\tt
  {\textbackslash}iclrfinalcopy} should be inserted to adjust the
format to the camera ready requirements.

The format for the submissions is a variant of the NeurIPS format.
Please read carefully the instructions below, and follow them
faithfully.

\subsection{Style}

Papers to be submitted to ICLR 2023 must be prepared according to the
instructions presented here.

%% Please note that we have introduced automatic line number generation
%% into the style file for \LaTeXe. This is to help reviewers
%% refer to specific lines of the paper when they make their comments. Please do
%% NOT refer to these line numbers in your paper as they will be removed from the
%% style file for the final version of accepted papers.

Authors are required to use the ICLR \LaTeX{} style files obtainable at the
ICLR website. Please make sure you use the current files and
not previous versions. Tweaking the style files may be grounds for rejection.

\subsection{Retrieval of style files}

The style files for ICLR and other conference information are available online at:
\begin{center}
   \url{http://www.iclr.cc/}
\end{center}
The file \verb+iclr2023_conference.pdf+ contains these
instructions and illustrates the
various formatting requirements your ICLR paper must satisfy.
Submissions must be made using \LaTeX{} and the style files
\verb+iclr2023_conference.sty+ and \verb+iclr2023_conference.bst+ (to be used with \LaTeX{}2e). The file
\verb+iclr2023_conference.tex+ may be used as a ``shell'' for writing your paper. All you
have to do is replace the author, title, abstract, and text of the paper with
your own.

The formatting instructions contained in these style files are summarized in
sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.

\section{General formatting instructions}
\label{gen_inst}

The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).
Use 10~point type with a vertical spacing of 11~points. Times New Roman is the
preferred typeface throughout. Paragraphs are separated by 1/2~line space,
with no indentation.

Paper title is 17~point, in small caps and left-aligned.
All pages should start at 1~inch (6~picas) from the top of the page.

Authors' names are
set in boldface, and each name is placed above its corresponding
address. The lead author's name is to be listed first, and
the co-authors' names are set to follow. Authors sharing the
same address can be on the same line.

Please pay special attention to the instructions in section \ref{others}
regarding figures, tables, acknowledgments, and references.


There will be a strict upper limit of 9 pages for the main text of the initial submission, with unlimited additional pages for citations. 

\section{Headings: first level}
\label{headings}

First level headings are in small caps,
flush left and in point size 12. One line space before the first level
heading and 1/2~line space after the first level heading.

\subsection{Headings: second level}

Second level headings are in small caps,
flush left and in point size 10. One line space before the second level
heading and 1/2~line space after the second level heading.

\subsubsection{Headings: third level}

Third level headings are in small caps,
flush left and in point size 10. One line space before the third level
heading and 1/2~line space after the third level heading.

\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone, regardless of the formatter being used.

\subsection{Citations within the text}

Citations within the text should be based on the \texttt{natbib} package
and include the authors' last names and year (with the ``et~al.'' construct
for more than two authors). When the authors or the publication are
included in the sentence, the citation should not be in parenthesis using \verb|\citet{}| (as
in ``See \citet{Hinton06} for more information.''). Otherwise, the citation
should be in parenthesis using \verb|\citep{}| (as in ``Deep learning shows promise to make progress
towards AI~\citep{Bengio+chapter2007}.'').

The corresponding references are to be listed in alphabetical order of
authors, in the \textsc{References} section. As to the format of the
references themselves, any style is acceptable as long as it is used
consistently.

\subsection{Footnotes}

Indicate footnotes with a number\footnote{Sample of the first footnote} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches
(12~picas).\footnote{Sample of the second footnote}

\subsection{Figures}

All artwork must be neat, clean, and legible. Lines should be dark
enough for purposes of reproduction; art work should not be
hand-drawn. The figure number and caption always appear after the
figure. Place one line space before the figure caption, and one line
space after the figure. The figure caption is lower case (except for
first word and proper nouns); figures are numbered consecutively.

Make sure the figure caption does not get separated from the figure.
Leave sufficient space to avoid splitting the figure and figure caption.

You may use color figures.
However, it is best for the
figure captions and the paper body to make sense if the paper is printed
either in black/white or in color.
\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
\end{center}
\caption{Sample figure caption.}
\end{figure}

\subsection{Tables}

All tables must be centered, neat, clean and legible. Do not use hand-drawn
tables. The table number and title always appear before the table. See
Table~\ref{sample-table}.

Place one line space before the table title, one line space after the table
title, and one line space after the table. The table title must be lower case
(except for first word and proper nouns); tables are numbered consecutively.

\begin{table}[t]
\caption{Sample table title}
\label{sample-table}
\begin{center}
\begin{tabular}{ll}
\multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION}
\\ \hline \\
Dendrite         &Input terminal \\
Axon             &Output terminal \\
Soma             &Cell body (contains cell nucleus) \\
\end{tabular}
\end{center}
\end{table}

\section{Default Notation}

In an attempt to encourage standardized notation, we have included the
notation file from the textbook, \textit{Deep Learning}
\cite{goodfellow2016deep} available at
\url{https://github.com/goodfeli/dlbook_notation/}.  Use of this style
is not required and can be disabled by commenting out
\texttt{math\_commands.tex}.


\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}



\section{Final instructions}
Do not change any aspects of the formatting parameters in the style files.
In particular, do not modify the width or length of the rectangle the text
should fit into, and do not change font sizes (except perhaps in the
\textsc{References} section; see below). Please note that pages should be
numbered.

\section{Preparing PostScript or PDF files}

Please prepare PostScript or PDF files with paper size ``US Letter'', and
not, for example, ``A4''. The -t
letter option on dvips will produce US Letter files.

Consider directly generating PDF files using \verb+pdflatex+
(especially if you are a MiKTeX user).
PDF figures must be substituted for EPS figures, however.

Otherwise, please generate your PostScript and PDF files with the following commands:
\begin{verbatim}
dvips mypaper.dvi -t letter -Ppdf -G0 -o mypaper.ps
ps2pdf mypaper.ps mypaper.pdf
\end{verbatim}

\subsection{Margins in LaTeX}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+
from the graphicx package. Always specify the figure width as a multiple of
the line width as in the example below using .eps graphics
\begin{verbatim}
   \usepackage[dvips]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.eps}
\end{verbatim}
or % Apr 2009 addition
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
for .pdf graphics.
See section~4.4 in the graphics bundle documentation (\url{http://www.ctan.org/tex-archive/macros/latex/required/graphics/grfguide.ps})

A number of width problems arise when LaTeX cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command.

\subsubsection*{Author Contributions}
If you'd like to, you may include  a section for author contributions as is done
in many journals. This is optional and at the discretion of the authors.

\subsubsection*{Acknowledgments}
Use unnumbered third level headings for the acknowledgments. All
acknowledgments, including those to funding agencies, go at the end of the paper.

==> iclr2023/backup-20230214/intro.tex <==
Graphs encode rich relational information that can be leveraged in learning tasks across a wide variety of domains. Graph neural networks (GNNs) can learn powerful node, edge or graph-level representations by aggregating a node's representations with that of its neighbors. 
%Graph neural networks (GNNs) have demonstrated considerable promise in recent years by using these graph relations to supplement node representations with information from node neighbors.
%However, t
The specifics of a GNN's neighborhood aggregation scheme are critical to its effectiveness on a prediction task.
For instance, graph convolutional networks (GCNs) aggregate information via a simple averaging or max-pooling of neighbor features. 
%\citep{gcn_kipf_welling,graphsage}.
% While GCNs scales well, they are also indiscriminate. 
GCNs are prone to suffer in many real-world scenarios where uninformative or noisy connections exist between nodes \citep{gcn_kipf_welling,graphsage}. 
% GCNs may also over-smooth, with nodes in a graph taking on indistinguishable representations due to the indiscriminate aggregation operation \citep{gcn_oversmoothing,measuring_oversmoothing,topping2022understanding}. 
Graph-based attention mechanisms combat these issues by quantifying the relevance of node-neighbor relations and softly selecting neighbors in the aggregation step accordingly \citep{gat,gatv2,transformerconv}. This process of attending to select neighbors has contributed to significant performance gains for GNNs across a variety of tasks \citep{gnn_review, 2022message}. Similar to the use of attention in natural language processing and computer vision, attention in graph settings also enables the interpretability of model predictions via the examination of attention coefficients \citep{attn_interpret}. 

% Paramount to the effectiveness of attention mechanisms in GNNs is their ability to discern the specific graph connectivity patterns that underlie accurate, generalizable predictions. %As graph training data often contains noisy features and/or connections,
However, graph attention mechanisms can be prone to spurious edges and correlations that mislead them in how they attend to node neighbors, which manifests as a failure to generalize to unseen data \citep{attn_generalization}. One approach to improve GNNs' generalizability is to regularize attention coefficients in order to make them more robust to spurious correlations/connections in the training data. Previous work has focused on $L_0$ regularization of attention coefficients to enforce sparsity \citep{ye2021sparse} or has co-optimized a link prediction task using attention \citep{kim2021how}. Since these regularization strategies are formulated independently of the primary prediction task, they align the attention mechanism with some intrinsic property of the input graph without regard for the training objective. 
%Some of the previous work is also specific to the kind of graph attention mechanism chosen. 
% the inability of attention mechanisms to select the appropriate node neighbors also suggests an inability to determine the graph connections that causally contribute to a particular prediction.

% We take a different approach. We begin our study with the question: ``What is the importance of a specific edge to the prediction task?''
We take a different approach and consider the question: ``What is the importance of a specific edge to the prediction task?'' Our answer comes from the perspective of regularization: we introduce \methodname, a causal attention regularization framework that is broadly suitable for graph attention network architectures (\textbf{Figure}~\ref{fig:figure_1}). Intuitively, an edge in the input graph is important to a prediction task if removing it leads to substantial degradation in the prediction performance of the GNN. The key conceptual advance of this work is to scalably leverage active interventions on node neighborhoods (i.e., deletion of specific edges) to align graph attention training with the causal impact of these interventions on task performance. Theoretically, our approach is motivated by the invariant prediction framework for causal inference ~\citep{RePEc:bla:jorssb:v:78:y:2016:i:5:p:947-1012,graph_ood}. While some efforts have previously been made to infuse notions of causality into GNNs, these causal approaches have been largely limited to using causal effects from pre-trained models as features for a separate model \citep{trust_neigh,attn_generalization} or decoupling causal from non-causal effects \citep{causal_attn_graph}. 
% Causality is a frequently misused term, and \methodname may not uncover rigorously causal mechanisms. Nonetheless, 
%\methodname is motivated by the invariant prediction framework for causal inference ~\citep{RePEc:bla:jorssb:v:78:y:2016:i:5:p:947-1012,graph_ood}.

% Our work builds on previous findings \citep{attn_generalization} that an explicit focus on improving attention coefficients can pay rich dividends.
We apply \methodname on three graph attention architectures across eight node classification tasks, finding that it consistently improves test loss and accuracy. \methodname is able to fine-tune graph attention by improving its alignment with task-specific homophily. Correspondingly, we found that as graph heterophily increases, the margin of \methodname's outperformance widens. In contrast, a non-causal approach that directly regularizes with respect to label similarity generalizes less well. On the ogbn-arxiv network, we investigate the citations up/down-weighted by \methodname and found them to broadly group into three intuitive themes. Our causal approach can thus enhance the interpretability of attention coefficients, and we provide a qualitative analysis of this improved interpretability. We also present preliminary results demonstrating the applicability of \methodname to graph pruning tasks. 
%Lastly, by applying it on sample sub-networks for a large social media-sized network, \methodname can enable us to learn the attention coefficients that would generalize to the broader network. 
Due to the size of industrially relevant graphs, it is common to use GCNs or sampling-based approaches on them. There, using attention coefficients learned by \methodname on sampled subnetworks may guide graph rewiring of the full network to improve the results obtained with convolutional techniques. %while retaining scalability.

%Understanding how, and improving what, GNNs learn remains a major open problem and an active area of research. Towards this, our work bridges two families of techniques (attention regularization and causal interventions) which we believe could be a promising direction of future research. 

% performance gains
% intepretability
% issues: spurious correlations (training data size?, training data network connectivity), limitations of interpretability
% sensitivity to initialization

% themes:
% graph attention
% determining relevant neighbors
% causal modeling: interventions ("causal view of robustness...", "matching learned causal effects...")
% causal attention
% causal regularization: KDD paper + ICML paper (causal effects domain priors)
% 

==> iclr2023/backup-20230214/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> iclr2023/backup-20230214/related_work.tex <==
The performance gains associated with graph attention networks have led to a number of efforts to enhance and better understand graph attention mechanisms \citep{gat_survey}. One category of methods aims to improve the expressive power of graph attention mechanisms by supplementing a given prediction objective with a supervised attention mechanism~\citep{trust_neigh}, or a self-supervised connectivity prediction approach~\citep{kim2021how}. A related set of methods leverage signals from interventions on graphs from a causal perspective to aid in training GNNs. One class of techniques performs interventions on nodes~\citep{attn_generalization, trust_neigh}. CAL ~\citep{causal_attn_graph}, a method designed for graph property prediction tasks, performs abstract interventions on representations of entire graphs instead of specific nodes or edges to identify the causally attended subgraph for a given task. Specifically, it uses these interventions to achieve robustness rather than directly leveraging information about the effect of these interventions on model predictions. 
% Meanwhile, other methods such as CAL~\citep{causal_attn_graph}  or CFLP~\citep{2106.02172} aim to separate causal and non-causal effects with auxiliary tasks, with CAL and CFLP designed specifically for graph property prediction and link prediction tasks, respectively.

Our intervention-oriented framework can also be understood as a graph structure perturbation method. Perturbation methods can be broadly split into three different categories: graph data augmentation~\citep{2202.08871}, structural graph rewiring~\citep{DBLP:conf/iclr/RongHXH20}, and geometric graph rewiring~\citep{topping2022understanding}. Inspired by the success of data augmentation approaches in computer vision, graph data augmentation methods seek to generate new training samples through different augmentation techniques. One of the earliest methods is DropEdge~\citep{DBLP:conf/iclr/RongHXH20} reduces overfitting by randomly selecting edges from a uniform distribution to delete. Other methods build on DropEdge and select edges according to additional constraints including geometrical invariants~\citep{gao2021training}, target probability distributions~\citep{NEURIPS2021_9e7ba617}, and information criteria~\citep{suresh2021adversarial}. EERM, a powerful invariance-based approach by \cite{graph_ood} takes a graph-editing approach to learn GNNs that are robust to distribution shifts in the data. % In contrast to \methodname, EERM requires learning a graph generation policy for sampling subgraphs.
Structural graph rewiring instead seeks to enforce structural priors such as sparsity or homophily during the graph alteration phase. Examples of these rewiring priors include fairness~\citep{2201.08549, 9645324}, temporal structure~\citep{NEURIPS2021_0b0b0994}, predicted homophily~\citep{measuring_oversmoothing}, sparsity\citep{10.1145/3394486.3403049, pmlr-v119-zheng20d}, or information transfer efficiency~\citep{10.5555/3454287.3455484}. Geometric approaches, instead, choose to view the graph as a discrete geometry and alter the connectivity according to the balanced Forman curvature~\citep{topping2022understanding}, the stochastic discrete Ricci flows~\citep{2207.08026}, commute times~\citep{2206.07369}, or algebraic connectivity\citep{2206.07369}. All of these approaches are designed either for use either in self-supervised learning or in a task-agnostic fashion, and consider the input graph independently of the task at hand.

To summarize, \methodname introduces a combination of advances not previously reported: applicability to diverse attention architectures; task-based supervised regularization (rather than task-agnostic or self-supervised regularization) that leads to improved generalization; and a causal approach that scalably and directly relates an edge's importance to its attention coefficient, enhancing interpretability. 

% A key innovation of our design is an edge selection scheme for performing multiple interventions in parallel, ensuring scalability. 

% Unlike these approaches, \methodname takes a more direct and interpretable approach to graph perturbation, and applies this to node classification and graph property prediction. \methodname achieves this by supervising the attention coefficients through active interventions on sampled edges during training. The active intervention framework directly enables the measurement of the individual treatment effect, so that we can perform task-specific casual regularization of the attention coefficients for arbitrary attention-based models. While \methodname can be understood through the lens of graph sparsification, \methodname does not seek to explicitly alter the edge connectivity through structural perturbations that may be deleterious to generalization. Moreover, \methodname alters the underlying geometry in \textit{task specific} ways.

% Unlike these approaches, \methodname takes a more direct and interpretable approach to graph perturbation, and applies this to node classification and graph property prediction. \methodname achieves this by supervising the attention coefficients by active interventions on sampled edges during training. The active intervention framework directly enables the measurement of the individual treatment effect, so that we can perform task-specific casual regularization of the attention coefficients for arbitrary attention-based models.

% The performance gains associated with graph attention networks have led to a number of efforts to enhance and better understand graph attention mechanisms \citep{gat_survey}. One category of methods aims to improve the expressive power of graph attention mechanisms by supplementing a given prediction objective with one or more tasks. \cite{attn_review} found that adding the supervised training of attention as an auxiliary task dramatically improved classification accuracy and that classification accuracy depended exponentially on attention correctness in their experiments. Such settings with ground truth attention are rare, though, so alternative tasks have been proposed to learn better attention coefficients. For example, SuperGAT adds an edge self-supervision task that is task-agnostic, using the connectivity patterns of existing edges in a graph to inform the assignment of attention coefficients to edges \citep{kim2021how}.

% A related set of methods leverage signals from interventions on graphs to aid in training GNNs. \cite{attn_review} devised an auxiliary weakly-supervised attention learning task based on changes in a pre-trained GCN's predictions that stem from node-level interventions. Causal GCN Inference (CGI) uses the outcomes of node-level interventions on a pre-trained GCN as well but as features in a classifier rather than as a means of informing attention \citep{trust_neigh}. Meanwhile, the Causal Attention Learning (CAL) strategy \citep{causal_attn_graph} aims to decouple causal and non-causal effects by introducing an additional task that encourages robustness to abstract interventions on graph representations rather than specific nodes or edges. Unlike these approaches, \methodname takes a more direct and interpretable approach, supervising the attention coefficients by active interventions on sampled edges during training and measuring the causal effect on the prediction task.

% Perhaps the method most comparable to ours is CFLP~\citep{2106.02172}, which treats an edge's existence as an individual treatment effect and constructs a causal model to predict the average treatment effect directly. However, it differs from \methodname substantially, both in application and approach. \methodname uses an estimate of the individual treatment effect to regularize the attention coefficients for arbitrary attention-based models, rather than alter the data distribution that is used for training. Additionally, CFLP is aimed at link-prediction which requires positional, rather than structural, representations~\citep{Srinivasan2020On}, whereas our work is aimed at node and graph classification for which structural representations are sufficient.

% % Graph data augmentation
% Inspired by the success of data augmentation approaches in computer vision, graph perturbations have also found their use in graph data augmentation~\cite{2202.08871}. In DropEdge~\citep{DBLP:conf/iclr/RongHXH20}, edges are randomly deleted in subgraph samples to reduce overfitting. Dropping edges indiscriminately can result in pathological examples that limit generalization. 
% TADropEdge~\citep{gao2021training} seeks to limit this effect by drawing edges according to topological invariants. MH-Aug~\cite{NEURIPS2021_9e7ba617} instead uses Metropolis-Hastings to generate new training examples through a set of graph mutation rules. 
% AD-GCL~\cite{suresh2021adversarial} constructs a contrastive learning framework to drop edges by minimizing the information lost by dropping each edge. All of these approaches are designed either for self-supervised learning (e.g., AD-GCL) or in a task-agnostic fashion (e.g., DropEdge), distinguishing them from \methodname. % This is done to increase generalization by reducing the number of repeated structural features that are learned.

% % Graph Rewiring

% Many methods have explored graph rewiring as a way to improve inferential accuracy, predictive performance, or improve generalization. GDC~\cite{10.5555/3454287.3455484} seeks to improve information diffusion while reducing noise through densification and then sparsification steps. In an attempt to debias learned representations, FairAug~\cite{2201.08549} and FairDrop~\cite{9645324} remove edges according to a defined fairness metric. MeTa~\cite{NEURIPS2021_0b0b0994} generates new subgraphs through temporal edge-sampling, and then learns to pass messages between temporally distinct subgraphs. This method has clear causal intuition, but without the interventional semantic of \methodname. The AdaEdge method~\cite{measuring_oversmoothing}, supervised edge-perturbation is performed through multiple full-training runs where the graph is rewired to optimize for predicted-homophily.

% % Graph Geometry
% \RS{@TM: ok if we kill/shrink this paragraph if we are still running short on space?}
% Another related set of methods have observed that intrinsic properties of the graph, such as sparsity or curvature, can be leveraged to rewire the graph to increase task generalization. Pro-GNN\cite{10.1145/3394486.3403049} co-learns a GNN and a sparsified graph structure to build methods that are robust to external perturbation. Sparsification is learned through structural optimization of the adjacency matrix. Similar to \methodname, NeuralSparse~\cite{pmlr-v119-zheng20d} seeks to sparsify by removing task-irrelevant edges. NeuralSparse, however, chooses to do so by learning a generative distribution over graph perturbations. Moving beyond sparsification, work based on the balanced Forman curvature~\cite{topping2022understanding} rewires the graph to improve information flow through the graph, which yielded state of the art performance on a variety of benchmarks. This idea is pushed further in by Bober \textit{et al.}~\cite{2207.08026} where they view a graph as a discrete geometry and use tools for discrete differential geometry. Alternatively, DiffWire~\cite{2206.07369} presents two different GCN layers: CT and GAP that are fully differentiable and optimize graph connectivity according to commute times or the algebraic connectivity. While \methodname can be understood through the lens of graph sparsification, \methodname does not seek to explicitly alter the edge connectivity through structural perturbations that may be deleterious to generalization. Moreover, \methodname alters the underlying geometry in \textit{task specific} ways.


% \RS{@TM/AW: new paragraph, pls check} To summarize, \methodname introduces a combination of advances not previously reported: applicability to diverse attention architectures; task-based supervised regularization (rather than task-agnostic or self-supervised regularization) leading to improved generalization; and a causal approach that directly relates an edge's importance to its attention coefficient, enhancing interpretability. A key innovation of our design is an edge selection scheme for performing multiple interventions in parallel, ensuring scalability. 


% edge-level interventions
% during training (accounts for ability of GAT to adjust weights of neighbors vs. indiscriminate pooling as in GCNs)

% \noindent \textbf{Attention in GNNs:}

% \noindent \textbf{Graph Attention Regularization:} 

% self-supervised learning: friendly neighbors
% weakly supervised learning: graph attention generalization (attention over nodes, intervention w/ weak supervision)
% causal: granger-causal attentive mixtures of experts, trust neighbors?
% l0 regularization: ye2021 - graph rewiring too

% \cite{attn_review} found that, in cases where ground-truth attention is available, supervised training of attention contributed to improved generalization performance of models to unseen and noisy graph inputs. 

% Hence, efforts have been made to design graph attention through supplementing learning tasks with self-supervision \cite{friendly_neigh} or by .

% using causal effects from pre-trained models as features for a separate model \citep{trust_neigh} or decoupling causal from non-causal effects \citep{causal_attn_graph}. To our knowledge, no efforts have . 

% graph attention
% graph causal modeling
% causal explanations
% causal regularization (graph domain priors, CAL) + supervised attention

==> iclr2023/backup-20230214/reproducibility.tex <==
To ensure the reproducibility of the results in this paper, we have included the source code for our method as supplementary materials. The datasets used in this paper are all publicly available, and we also use the publicly available train/validation/test splits for these datasets. We provide details on these datasets in the Appendix and have provided references to them in both the main text and the Appendix. In addition, we have provided detailed descriptions of the experimental setup, model training schemes, model architecture design choices, and hyperparameter choices in the ``Experimental Setup'' section as well as in Appendix \ref{appen:arch_hyper}.


==> iclr2023/backup-20230214/results.tex <==
\subsection{Experimental Setup}
We assessed the effectiveness of \methodname by comparing the performance of a diverse range of models trained with and without \methodname on 8 node classification datasets.
% (see additional applications in \S \ref{subsec:methods:investigation}). 
Specifically, we aimed to assess the consistency of \methodname's outperformance 
over matching baseline models across various graph attention mechanism and hyperparameter choices. Accordingly, we evaluated numerous combinations of such configurations (48 settings for each dataset and graph attention mechanism), rather than testing only a limited set of optimized hyperparameter configurations. 
% to assess the effect of using \methodname on each configuration. 
The configurable model design and hyperparameter choices that we evaluated include the graph attention mechanism (GAT, GATv2, or Graph Transformer), the number of graph attention layers $L=\{1,2\}$, the number of attention heads $K=\{1,3,5\}$, the number of hidden dimensions $F'=\{10,25,100,200\}$, and the regularization strength $\lambda=\{0.1,0.5,1,5\}$. See \textbf{Appendix} \ref{appen:arch_hyper} for details on the network architecture, hyperparameters, and training configurations. 

\subsection{Node Classification}
\noindent \textbf{Datasets and evaluation:} We used a total of 8 real-world node classification datasets of varying sizes and degrees of homophily: Cora, CiteSeer, PubMed, ogbn-arxiv, Chameleon, Squirrel, Cornell and Wisconsin. Each model was evaluated according to its accuracy on a held-out test set. We also evaluated the test cross-entropy loss, as it accounts for the full distribution of per-class predictions rather than just the highest-valued prediction considered in accuracy calculations. See \textbf{Appendix} \ref{appen:node_class_datasets} for details on dataset statistics, splits, and references. % Runtimes for training models with \methodname ranged from roughly 2 seconds to 5 minutes on the evaluated datasets, with \methodname's runtime only 1.5-2 times that of standard training on average (see \textbf{Appendix} \ref{appen:runtime_memory} for details). 

\noindent \textbf{Generalization performance:} We compared both the test accuracy and the test loss of each model when trained with and without \methodname. Across all model architecture and hyperparameter choices for a dataset, we applied the one-tailed paired Wilcoxon signed-rank test to quantify the overall outperformance of models trained with \methodname against models trained without it. \methodname resulted in higher test accuracy in 7 of the 8 node classification datasets and a lower test loss in all 8 datasets (\textbf{Figure} \ref{fig:figure_2}, $p < 0.05$). We report the relative performance when averaging over all hyperparameter choices in \textbf{Table}~\ref{table:loss_results} (test loss), \textbf{Table}~\ref{table:acc_results} (test accuracy, in \textbf{Appendix} \ref{appen:node_class_acc}), and \textbf{Appendix} \ref{appen:percent_change_acc_loss}. We also observed that even small values of $R$ were effective (\textbf{Appendix} \ref{appen:num_interventions}). We believe that this is due to there being an adequate number of causal-effect examples for regularization, as even in the minimum $R=1$ case, we have roughly one causal-effect example per training example. 

We also compared \methodname with \cite{causal_attn_graph}'s CAL, a method for graph property prediction that relies on an alternative formulation of causal attention with interventions on implicit representations. We adapted CAL for node classification by removing its final pooling layer. \methodname-trained models substantially outperformed CAL (\textbf{Appendix} \ref{appen:compare_cal}), suggesting that \methodname's direct edge-intervention approach results in better generalization. Taken together, these results highlight the consistency of performance gains achieved with \methodname and its broad applicability across across graph attention architectures and hyperparameters. 
% Furthermore, in comparing \methodname with a modified version of CAL, a method that relies on an alternative formulation of causal attention for graph property predictions ~\citep{2106.02172}, we observed that \methodname-trained models drastically outperformed CAL as well (\textbf{Appendix} \ref{appen:compare_cal}).

% \AW{do we want to condense the accuracy and loss tables into one table with just the mean values of each? we can then show the full tables with the standard deviations in the appendix.}

\begin{table}[ht]
\caption{Test loss on 8 node classification datasets}
\label{table:loss_results}
\centering
\small
\renewcommand{\arraystretch}{1.5}
\begin{center}
\resizebox{14cm}{!}{%
\begin{tabular}{l c c c c c c c c }
    & \textbf{Cora} & \textbf{CiteSeer} & \textbf{PubMed} & \textbf{ogbn-arxiv} & \textbf{Chameleon} & \textbf{Squirrel} & \textbf{Cornell} & \textbf{Wisconsin} \\
    \hline
    GAT &  2.33 $\pm$ 0.75 & 3.68 $\pm$ 2.64 & 1.05 $\pm$ 0.24 & 1.49 $\pm$ 0.02 & 1.29 $\pm$ 0.03 & 1.48 $\pm$ 0.02 & 1.19 $\pm$ 0.23 & 0.88 $\pm$ 0.11  \\
    % \hline
    GAT + \methodname & \textbf{1.82 $\pm$ 0.77} & \textbf{3.06 $\pm$ 2.34} & \textbf{0.89 $\pm$ 0.18} & 1.49 $\pm$ 0.02 & \textbf{1.26 $\pm$ 0.03} & \textbf{1.47 $\pm$ 0.02} & \textbf{1.14 $\pm$ 0.17} & \textbf{0.84 $\pm$ 0.13} \\
    \hline
    GATv2 &  2.26 $\pm$ 0.54 & 3.08 $\pm$ 1.06 & 1.07 $\pm$ 0.29 & 1.48 $\pm$ 0.02 & 1.28 $\pm$ 0.03 & 1.48 $\pm$ 0.02 & 1.09 $\pm$ 0.11 & 0.88 $\pm$ 0.15 \\
    GATv2 + \methodname & \textbf{1.63 $\pm$ 0.59} & \textbf{3.04 $\pm$ 2.07} & \textbf{0.90 $\pm$ 0.17} & \textbf{1.47 $\pm$ 0.03} & \textbf{1.24 $\pm$ 0.03} & \textbf{1.46 $\pm$ 0.02} & \textbf{1.04 $\pm$ 0.10} & \textbf{0.81 $\pm$ 0.09} \\
    \hline
    Transformer & 3.43 $\pm$ 1.61 & 9.78 $\pm$ 8.27 & 1.79 $\pm$ 0.88 & 1.50 $\pm$ 0.03 & 1.38 $\pm$ 0.06 & 1.50 $\pm$ 0.02 & 1.22 $\pm$ 0.25 & 1.03 $\pm$ 0.28 \\
    Transf.\ + \methodname & \textbf{1.71 $\pm$ 0.50} & \textbf{3.92 $\pm$ 2.25} & \textbf{1.60 $\pm$ 0.59} & 1.50 $\pm$ 0.03 & \textbf{1.33 $\pm$ 0.04} & \textbf{1.48 $\pm$ 0.03} & \textbf{1.07 $\pm$ 0.12} & \textbf{0.86 $\pm$ 0.13} \\ 
    \hline
\end{tabular}}
\end{center}
\end{table}
\vspace*{-0.5cm}

\subsection{Model Investigation and Ablation Studies}
\label{subsec:methods:investigation}
%%\RS{points to make: a) \methodname accentuates correlation with homophily, more so for heterophilic networks [label agreement result?]; b) effect of hyperparameter $\lambda$ (b.1: violin plot; b.2: dialed-up/down cora homophily)  c) an ablation where label propagation was directly used to regularize also helps but not as much as \methodname, esp for heterophilic networks; \sout{d) random edge ablation?}}

\paragraph{Impact of regularization strength} 
We explored 4 settings of $\lambda$: $\{0.1, 0.5, 1, 5\}$. For 6 of the 8 node classification datasets, \methodname models trained with the higher causal regularization strengths ($\lambda=\{1,\,5\}$) demonstrated significantly larger reductions in test loss ($p < 0.05$, one-tailed Welch's $t$-test) compared to those trained with weaker regularization ($\lambda=\{0.1,\,0.5\}$). Notably, all four of the datasets with lower homophily (Chamelon, Squirrel, Cornell and Wisconsin) displayed significantly larger reductions in test loss with the higher regularization strengths, suggesting that stronger regularization may contribute to improved generalization in such settings (\textbf{Appendix} \ref{appen:compare_loss_lambda}).

%\noindent \textbf{Selecting $\lambda$ for \methodname in multi-layer GNNs:} (still include?)

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.995 \linewidth ]{fig2_causal_comparison_node.pdf}
    \caption{Test accuracy and negative loss on 8 node classification datasets. Each point corresponds to a comparison between a baseline model trained without \methodname and an identical model trained with \methodname. The point size represents the magnitude of the $\lambda$ value chosen for the \methodname-trained model. $p$-values are computed from one-tailed paired Wilcoxon signed-rank tests evaluating the improvement of \methodname-trained models over the baseline models.}
    \label{fig:figure_2}
\end{figure}



\paragraph{Connection to spurious correlations and homophily}

Graph attention networks that are prone to spurious correlations mistakenly attend to parts of the graph that are irrelevant to their prediction task. To evaluate if \methodname reduces the impact of such spurious correlations, we assessed if models trained with \methodname more effectively prioritized relevant edges. For node classification tasks, the relevant neighbors to a given node are expected to be those that share the same label as that node. We, therefore, used the label agreement between nodes connected by an edge as a proxy for the edge's ground-truth relevance. We assigned a reference attention coefficient $e_{ij}$ to an edge based on label agreement in the target node's neighborhood: $e_{ij} = \hat{e}_{ij}/\sum_{k\in N_j} \hat{e}_{kj}$ \citep{kim2021how}. Here, $\hat{e}_{ij} = 1$ if nodes $i$ and $j$ have the same label and $\hat{e}_{ij} = 0$ otherwise. $N_j$ denotes the in-neighbors of node $j$. We then calculated the KL divergence of an edge's attention coefficient $\alpha_{i,j}$ from its reference attention coefficient $e_{ij}$ and summarize a model's ability to identify relevant edges as the mean of these KL divergence values across the edges in the held-out test set. 

We compared these mean KL divergences between baseline models trained without \methodname and models trained with \methodname across the same broad range of model architecture and hyperparameter choices described above. We found that \methodname-trained models consistently yielded lower mean KL divergence values than models trained without \methodname  for 6 of 8 node classification datasets (\textbf{Figure }\ref{fig:figure_3},$p < 0.05$, one-tailed paired Wilcoxon signed-rank test). Notably, this enhanced prioritization of relevant edges was achieved without explicitly optimizing label agreement during training and is an inherent manifestation of aligning attention with the node classification tasks' causal effects.

% The improvement in AP for \methodname-trained models was particularly pronounced for the Chameleon and Squirrel datasets, which are characterized by lower homophily, while the higher homophily datasets (Cora, CiteSeer, PubMed) were not associated with such gains (Appendix \ref{appen:label_agreement_homophily}). 

Low homophily graphs are associated with greater proportions of task-irrelevant edges and thus may introduce more spurious correlations~\citep{heterophily}. We reasoned that \methodname's relative effectiveness should be greater in such settings. We assessed this by evaluating \methodname on 33 synthetic Cora datasets with varying levels of homophily \citep{homophily_syn_cora}. We observed that \methodname-trained models outperformed baseline models most substantially in low homophily settings, with performance gains generally increasing with decreasing homophily (\textbf{Appendix} \ref{appen:syn_cora}). Altogether, these results demonstrate that \methodname not only more accurately prioritizes the edges that are most relevant to the desired task but also highlights its utility in low homophily settings most prone to spurious correlations. 
%more effective greater sensitivity to spurious correlations, \methodname's effectiveness in such settings provides further evidence for its ability to enhance graph attention
% In addition, this result highlights the applicability of \methodname for low homophily graphs, as graph attention is essential in such settings due to the relative dissimilarity of neighboring nodes in these graphs. 

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.7 \linewidth ]{fig3_label_agreement.pdf}
    \caption{Coherence between attention coefficients and label agreement for \methodname-trained models, compared to baseline. Lower KL divergence implies greater coherence. Point colors and sizes have the same meaning as in \textbf{Figure} \ref{fig:figure_2}. $p$-values are computed from one-tailed paired Wilcoxon signed-rank tests evaluating the improvement of \methodname-trained models over the baseline models.}
    \label{fig:figure_3}
\end{figure}

\paragraph{Comparison to homophily-based regularization} 
%We also evaluated the degree to which aligning attention mechanisms with their causal effects contributed to this improved generalization performance. 
We next assessed if the performance gains by our causal approach could be replicated by a non-causal approach that systematically aligns attention coefficients with a generic measure of homophily. To do so, we performed an ablation study in which we replace the causal effects $c_{ij}^{(n)}$ computed from the network being trained (\textbf{Equation} \ref{eqn:causal_effect}) with an alternative score derived from a homophily-based classification scheme. Briefly, this scheme entails assigning a prediction for each node based on the counts of its neighbors' labels (see \textbf{Appendix} \ref{appen:neighbor_vote} for details). By regularizing attention with respect to this homophily-based classification scheme, the attention mechanism for a network will be guided no longer by causal effects associated with the network but rather this separate measure of homophily.

% Separately, we also we simply draw each causal effect $c_{i,j}^{(n)}$ from a uniform distribution on the interval $[0,1)$ 

We compared \methodname-trained models with those trained with homophily-based regularization by evaluating the consistency of their test loss improvements relative to the baseline models without regularization. We used the one-tailed paired Wilcoxon signed-rank test to evaluate the significance of the regularized models' test loss improvements across the set of model architecture and hyperparameter choices, focusing on models trained with the higher $\lambda \in \{1,5\}$ regularization strengths. Models trained when regularizing attention coefficients with the homophily-based scheme underperformed those trained with \methodname in 7 of the 8 datasets (\textbf{Table} \ref{table:ablation}). Interestingly, the homophily-based -based regularization showed an overall gain in performance relative to the baseline models (i.e., those trained without any regularization), suggesting that even non-specific regularization can be somewhat useful for training attention. Overall, these results demonstrate the effectiveness of using \methodname to improve generalization performance for many node classification tasks.

\begin{table}[h!]
\smallskip
\centering
% \caption{Generalization performance of \methodname-trained models with ablations compared to baseline \\($-\log_{10}(p)$, one-tailed paired Wilcoxon signed-rank test)}
\caption{Ablation study comparing improvements in performance using \methodname regularization and homophily-based regularization ($-\log_{10}(p)$, one-tailed paired Wilcoxon signed-rank test)}
\label{table:ablation}
\renewcommand{\arraystretch}{1.2}
\resizebox{14cm}{!}{%

\begin{tabular}{ r  c  c  c  c  c  c  c  c } 
    % \multirow{3}{*}{\bf Method}  &\multicolumn{2}{c}{\bf Cora} &\multicolumn{2}{c}{\bf CiteSeer} &\multicolumn{2}{c}{\bf PubMed} &\multicolumn{2}{c}{\bf orgn-arxiv} &\multicolumn{2}{c}{\bf Chameleon} &\multicolumn{2}{c}{\bf Squirrel} \\ 
    & \textbf{Cora} & \textbf{CiteSeer} & \textbf{PubMed} & \textbf{ogbn-arxiv} & \textbf{Chameleon} & \textbf{Squirrel} & \textbf{Cornell} & \textbf{Wisconsin} \\
    % \cmidrule(lr){2-3}\cmidrule(lr){3-4}\cmidrule(lr){5-6}
    \hline
    \methodname & \textbf{12.36} & \textbf{5.92} & \textbf{10.51} & \textbf{1.81} & \textbf{12.77} & 9.72 & \textbf{6.72} & \textbf{9.34} \\
    % \hline
    Homophily &  10.04 & 5.59 & 7.30 & 0.53 & 12.34 & \textbf{10.97} & 4.15 & 8.20 \\
    \hline
    % \methodname & \textbf{8.99} & \textbf{4.34} & \textbf{7.81} & \textbf{0.655} & \textbf{10.84} & 9.56 & \textbf{3.84} & \textbf{6.24} \\
    % % \hline
    % Neighbor Voting & 8.89 & 3.62 & 4.78 & 0.233 & 9.20 & 10.84 & 2.28 & 5.30 \\
    % \hline
    % Random & X & X & X & X & X & X \\
\end{tabular}}
\end{table}
\vspace*{-0.2cm}

% \begin{table}[h!]
% \centering
% \caption{\methodname-trained graph attention mechanisms attend to homophilous edges in node classification}
% \label{table:attn_homophily}
% \renewcommand{\arraystretch}{2.5}
% \begin{tabular}{ c  c  c  c  c  c  c } 
%     & Cora & CiteSeer & PubMed & ogbn-arxiv & Chameleon & Squirrel \\
%     % \cmidrule(lr){2-3}\cmidrule(lr){3-4}\cmidrule(lr){5-6}
%     \hline
%     Baseline & 0.81 \pm 0.01 & 0.76 \pm 0.01 & 0.81 \pm 0.01 & 0.70 \pm 0.01 &  \\
%     \hline
%     Baseline & 0.81 \pm 0.01 & 0.76 \pm 0.01 & 0.81 \pm 0.01 & 0.70 \pm 0.01 & 
% \end{tabular}
% \end{table}


% \subsubsection{Cheeger Constant}
% \TM{Do we have results here? Because the graphs are all disconnected, this might be difficult to interpret.}
% Next, we turn our attention to a series of experiments intended to understand the topological changes that our graph undergoes due to our causal regularization method. 

% Because our method prunes edges, we are specifically interested in understanding whether our method is introducing bottlenecks that would make us more susceptible to over-squashing. To answer this question, we compute Cheeger constant as a function of regularization strength for the Cora dataset.

% Furthermore, we computed the curvature of the original graph, pruned graph, and removed edges; and present the kernel density estimates below.

% \subsubsection{Graph Diffusion Distance}
% \TM{Do we have results here? It feels like a nice to have but probably a P1/P2 priority.}
% Next, we are interested to understand whether our proposed method is simply removing edges that are ``topologically noisy''. To answer this question, we have computed the graph diffusion distance defined as

% \begin{equation}
%  d^{(u,v)}_{GDD}(A_1, A_2) = \sqrt{ \argmax_{t} \left | \left |  e^{-t L}  - e^{-t L\backslash ({u,v}) } \right | \right |^2_F},
% \end{equation}

% where $L$ is the graph Laplacian, and $L\backslash ({u,v})$ is the graph Laplacian with the edge from $u$ to $v$ deleted. We use this metric because it provides a global measure of graph diffusion, which is intimately connected to message passing.

\paragraph{Additional applications}
To explore the utility of \methodname as a general-purpose framework, we employed \methodname for graph pruning. 
% For graph property prediction, we evaluated \methodname on ogbg-molbace, a dataset for binary classification, and ogbg-molfreesolv, which features a regression task \citep{ogb}. We trained models with \methodname across a broad range of graph attention mechanisms and hyperparameter choices. For both datasets, we found that \methodname-trained models consistently outperformed those that were trained without \methodname ($p < 0.05$, one-tailed paired Wilcoxon signed-rank test, see \textbf{Appendix} \ref{appen:graph_property_pred} for details).
% We also explored a \methodname-guided graph pruning approach. 
\methodname directly uses local pruning (i.e. edge interventions) to guide the training of graph attention in a manner that down-weights task-irrelevant edges. As such, we reasoned that attention coefficients produced by \methodname-trained models could be used to prune task-irrelevant edges (see \textbf{Appendix} \ref{appen:graph_rewiring} for more details). In this approach, we used \methodname's edge pruning procedure as a pre-processing step for training and inference with GCNs, which are more scalable than graph attention networks \citep{sign} but indiscriminate in how they aggregate information over node neighborhoods. We found that using \methodname-guided pruning improved the test accuracy of GCNs, outperforming vanilla GCNs trained and evaluated over the full graph as well as GCNs trained and evaluated on graphs pruned with baseline graph attention mechanisms. These preliminary results open the door for further exploration of \methodname's utility on these tasks.


\subsection{Interpreting Attention Coefficients: Qualitative Analysis}
\label{subsec:results:qa}
%Previous perturbative approaches to guide GNN training did not directly intervene on edges in a task-specific way, making their interpretability less clear.
In addition to providing a robust way to increase both model quality and generalization, we explored the interpretability of \methodname attention coefficients in a \textit{post hoc} analysis. Here, we evaluated the edge-wise difference of the attention coefficients between our method and a baseline GAT applied to the \textrm{ogbn-arxiv} dataset. In this dataset, nodes represent arXiv papers, edges are citation links, and the prediction task is to classify papers into their subject areas. 

We manually reviewed citations that were up/down-weighted by \methodname-trained models and observed that these citations broadly fit into one of three categories:  (i) down-weighting self-citations, (ii) down-weighting popular ``anchor'' papers, or (iii) upweighting topically-narrow papers with few citations. In the first case, we found that \methodname down-weights edges associated with self-citations (\textbf{Table}~\ref{tab:self-cites}). The causal story here is clear--- machine learning is a fast-moving field with authors moving into the field and changing specialties as those specialties are born. Because of this, the narrative arc that a set of authors constructs to present this idea can include citations to their own previous work from different sub-fields. While these citations help situate the work within the broader literature and can provide background that readers might find valuable, they are not relevant to the subject area prediction task. 

\begin{table}[ht]
\small
\caption{\label{tab:self-cites}Down-weighted self-citations. }
\renewcommand{\arraystretch}{1}
\begin{center}
\begin{tabular}{p{0.42\linewidth} p{0.42\linewidth} p{0.10\linewidth}}
Paper Title & Cited Title (from a different subject area) & $\Delta$ \\
 \hline 
\textit{Viterbinet a Deep Learning Based Viterbi Algorithm for Symbol Detection} &
\textit{Frequency Shift Filtering for Ofdm Signal Recovery in Narrowband Power Line Communications} & -89.91 \% \\
% \smallskip \\
\textit{Solving Underdetermined Systems with Error Correcting Codes} &
\textit{Systems of MDS Codes from Units and Idempotents} & -89.80 \% \\
% \smallskip \\
\textit{Performance Analysis for Multichannel Reception of OOFSK Signaling} &
\textit{On-Off Frequency-Shift Keying for Wideband Fading Channels} & -81.03 \% \\
\end{tabular}
\end{center}
\end{table}

In the second case, we found that \methodname down-weights edges directed towards popular or otherwise seminal ``anchor'' papers (\textbf{Appendix}~\ref{appen:interpret_qual}, \textbf{Table}~\ref{tab:anchor-cites}). These papers tends to be included in introductions to provide references for common concepts or methods, such as Adam, ResNet, and ImageNet. They are also widely cited across subject areas and hence have little bearing on the subject area prediction task. Notably, \methodname does not simply learn to ignore edges from high-degree nodes. For the Word2Vec paper, we observed notable increases in attention coefficients for edges connecting it to multiple highly related papers, including a $2.5\times 10^6$ \% increase for \textit{Efficient Graph Computation for Node2Vec} and a $2.0\times 10^6$ \% increase for \textit{Multi-Dimensional Explanation of Reviews	}.

In the final case, we observed that \methodname up-weighted edges directed towards deeply related but largely unnoticed papers (\textbf{Appendix}~\ref{appen:interpret_qual},\textbf{Table}~\ref{tab:up-cites}). In our manual exploration of the data, we observed that these papers are those that are close to the proposed method. These papers are the type that are often found only after a thorough literature review. Such edges should play a key role in predicting a paper's topic and should be up-weighted.


==> iclr2023/backup-20230214/theory.tex <==
\subsection{Graph Attention Networks}

Attention mechanisms have been effectively used in many domains by enabling models to dynamically attend to the specific parts of an input that are relevant to a prediction task \citep{attention_survey}. In graph settings, attention mechanisms compute the relevance of edges in the graph for a prediction task. A neighbor aggregation operator then uses this information to weight the contribution of each edge \citep{gat_survey,gated_graph_sequence,self_attn_graph_pooling}. 

The approach for computing attention is similar in many graph attention mechanisms. A graph attention layer takes as input a set of node features $\mathbf{h} = \{\vec{h}_1,...,\vec{h}_N\}$, $\vec{h}_i \in \mathbb{R}^F$, where $N$ is the number of nodes. The graph attention layer uses these node features to compute attention coefficients for each edge: $\alpha_{ij} = a(\mathbf{W}\vec{h}_i,\mathbf{W}\vec{h}_j)$, 
% \begin{equation}
%     \label{eqn:attn_edges}
%     e_{ij} = a(\mathbf{W}\vec{h}_i,\mathbf{W}\vec{h}_j),
% \end{equation}
where $a : \mathbb{R}^{F'} \times \mathbb{R}^{F'} \rightarrow (0,1)$ is the attention mechanism function, and the attention coefficient $\alpha_{ij}$ for an edge indicates the importance of node $i$'s input features to node $j$.
% $\mathbf{W}\in \mathbb{R}^{F' \times F}$ projects the input features into a new feature space. The attention mechanism function $a : \mathbb{R}^{F'} \times \mathbb{R}^{F'} \rightarrow [0,1]$ uses these new node features to compute an attention coefficient $\alpha_{ij}$ for each edge that indicates the importance of node $i$'s input features to node $j$. 
% These attention coefficients are typically normalized with respect to the 1-hop neighborhood of each node using the softmax function, yielding normalized attention coefficients $\alpha_{ij}$ that indicate the importance of node $i$'s input features to node $j$.
For a node $j$, these attention coefficients are then used to compute a linear combination of its neighbors' features: $\vec{h}_j' =  \sum_{i\in N(j)}\alpha_{ij}\mathbf{W}\vec{h}_i, ~ ~ \mathit{s.t.} ~ \sum_{i\in N(j)} \alpha_{ij} = 1$.
For multi-headed attention, each of the $K$ heads first independently calculates its own attention coefficients $\alpha_{i,j}^{(k)}$ with its head-specific attention mechanism $a^{(k)}(\cdot,\cdot)$, after which the head-specific outputs are averaged. 
% \begin{equation}
%     \label{eqn:attn_aggr}
%     \vec{h}_j' =  \sum_{i\in N(j)}\alpha_{ij}\mathbf{W}\vec{h}_i,
%     ~ ~ \mathit{s.t.} ~ 
%     \sum_{i\in N(j)} \alpha_{ij} = 1
% \end{equation} 
% 

%RS: commenting out to save some space and make room for causal in the intro
%
%se attention coefficients are used to compute attention-head specific node outputs $\vec{h}_j'^{(k)}$, which are then averaged across the $K$ attention heads.
%
% \begin{equation}
%     \label{eqn:attn_heads}
%     \vec{h}_j' = \frac{1}{K}\sum_{k=1}^{K}\vec{h}_j'^{(k)}
% \end{equation}

In this paper, we focus on three widely used graph attention architectures: the original graph attention network (GAT) \citep{gat}, a modified version of this original network (GATv2) \citep{gatv2}, and the Graph Transformer network \citep{transformerconv}. %These graph attention architecture variants are distinguished by the manner in which they compute the unnormalized attention coefficients $e_{ij}$ (Table \ref{table:gat_variants}). 
The three architectures and their equations for computing attention  are presented in \textbf{Appendix} \ref{appen:gat_variants}. 

% In the original graph attention network (GAT) framework, the unnormalized attention coefficients are computed as follows \citep{gat}. Here, $||$ denotes concatenation and the concatenated node features are passed through a single-layer feedforward neural network featuring a weight vector $\mathbf{a} \in \mathbb{R}^{2F'}$ and the LeakyRELU nonlinearity. 
% \begin{equation}
%     \label{eqn:gat_attn}
%     e_{ij} = \text{LeakyReLU}\big(\vec{\mathbf{a}}^T [ \mathbf{W}\vec{h}_i || \mathbf{W}\vec{h}_j \big)]\big)
% \end{equation}
% GATv2 was proposed to improve upon the expressiveness of the original graph attention mechanism by applying the linear projection to concatenated input node features instead of individual node features \citep{gatv2}.
% \begin{equation}
%     \label{eqn:gatv2_attn}
%     e_{ij} = \vec{\mathbf{a}}^T\text{LeakyReLU}\big( \mathbf{W} \vec{h}_i || \mathbf{W} \vec{h}_j \big)
% \end{equation}
% Lastly, the Graph Transformer network extends the Transformer architecture used in natural language processing \citep{transformer} to graphs and computes the attention coefficients as follows, where as above $F'$ is the dimensionality of the new feature space \citep{transformerconv}. 
% \begin{equation}
%     \label{eqn:transformer_attn}
%     e_{ij} = \frac{(\mathbf{W}\vec{h}_i)^T(\mathbf{W}\vec{h}_j)}{\sqrt{F'}}
% \end{equation}

\begin{figure}
    \centering
    %\includegraphics[width=0.95 \linewidth ]{iclr2023/causal_attn_fig1_rs-v4.pdf}
    \includegraphics[width=0.9 \linewidth ]{car_regularization_overview.pdf}
    \caption{Schematic of \methodname: Graph attention networks learn the relative importance of each node-neighbor for a given prediction task. However, their inferred attention coefficients can be miscalibrated due to noise, spurious correlations, or confounders (e.g., node size here). Our causal approach directly intervenes on a sampled subset of edges and supervises an auxiliary task that aligns an edge's causal importance to the task with its attention coefficient.}
    \label{fig:figure_1}
\end{figure}

\subsection{Causal Attention Regularization: an Invariance Prediction Formulation}

\methodname is motivated by the invariant prediction (IP) formulation of causal inference \citep{RePEc:bla:jorssb:v:78:y:2016:i:5:p:947-1012,graph_ood}. The central insight of this formulation is that, given sub-models that each contain a different set of predictor variables, the underlying causal model of a system is comprised of the set of all sub-models for which the predicted class distributions are equivalent, up to a noise term. This approach is capable of providing statistically rigorous estimates for both the causal effect strength of predictor variables as well as confidence intervals. With \methodname, our core insight is that the graph structure itself, in addition to the set of node features, comprise the set of predictor variables.
% that are traditionally explored in causal regularization frameworks. 
This is equivalent to the intuition that relevant edges for a particular task should not only be assigned high attention coefficients but also be important to the predictive accuracy of the model (\textbf{Figure} \ref{fig:figure_1}). The removal of these relevant edges from the graph should cause the predictions that rely on them to substantially worsen. 

We leverage the residual formulation of IP to formalize this intuition. This formulation assumes that we can generate sub-models for different sets of predictor variables, each corresponding to a separate experiment $e \in \mathcal{E}$. For each sub-model $S^e$, we compute the predictions $Y^e = g(\mathcal{G}^e_\mathcal{S}, \mathcal{X}^e_\mathcal{S}, \epsilon^e)$ where $\mathcal{G}$ is the graph structure,  $\mathcal{X}$ is the set of features associated with $\mathcal{G}$, $\epsilon^e$ is the noise distribution, and $\mathcal{S}$ is the set of predictor variables corresponding to $S^e$. We next compute the residuals $\mathcal{R} = Y - Y^e$. IP requires that we perform a hypothesis test on the means of the residuals, with the generic approach being to perform an F-test for each sub-model against the null-hypothesis. The relevant assumptions ($\epsilon^e \sim F_\epsilon$, and $\epsilon^e \indep S^e$ for all $e \in \mathcal{E}$) are satisfied if and only if the conditionals $Y^e|S^e$ and $Y^f | S^f$ are identical for all experiments $e, f \in \mathcal{E}$.

We use an edge intervention-based strategy that corresponds precisely to this IP-based formulation. However, we differ from the standard IP formulation in how we estimate the final causal model. While IP provides a method to explicitly construct an estimator of the true causal model (by taking the intersection of all models for which the null hypothesis was rejected), we rely on  intervention-guided regularization of graph attention coefficients as a way to aggregate sub-models while balancing model complexity and runtime considerations. In our setting, each sub-model corresponds to a set of edge interventions and, thus, slightly different graph structures. The same GNN architecture is trained on each of these sub-models. Given a set of experiments $\mathcal{E} = \{e\}$ with sub-models $S^e$, outputs $Y^e$ and errors $\epsilon^e$, we regularize the attention coefficients to align with sub-model errors, thus learning a GNN architecture primarily from causal sub-models. Incorporating this regularization as an auxiliary task, we seek to minimize the following loss:
%
% . Including this regularization loss as an auxiliary task alongside the primary prediction task then encourages GNN architectures learned primarily from causal sub-models. Specifically, we seek to minimize the following loss:
%
% % We begin by briefly presenting the residual formulation of invariant prediction and then discuss in detail our notion of predictor variable, experiment generation, and experiment test. 
% We leverage the residual formulation of IP, which assumes that we can generate many sub-models with different sets of predictor variables $S^e$ corresponding to many different experiments. We can compute the predictions, $Y^e$ for every sub-model as well as the residuals $\mathcal{R} = Y - Y^e$. IP requires that we perform a hypothesis test on the means of the residuals. The generic method for invariant prediction is to test each hypothetical set of features against the null-hypothesis, $H_{0,S}(\mathcal{E})$, such that there exists $g: \mathbb{R}^{|S|} \times \mathbb{R} \rightarrow \mathbb{R}$ and $\epsilon^e$ that $Y^e = g(\mathcal{G}^e_S, \mathcal{X}^e_S, \epsilon^e)$, $\epsilon^e \sim F_\epsilon$ and $\epsilon^e \indep S^e$ for all $e \in \mathcal{E}$. This is satisfied if the conditionals $Y^e|S^e$ and $Y^f | S^f$ are identical for all experiments $e, f \in \mathcal{E}$. IP then provides a method to construct an estimator of the true causal model by taking the intersection of all models for which the null hypothesis was rejected. 
% % A key question in causal inference is the identification of identifiable models. Theorem 2 of \citet{RePEc:bla:jorssb:v:78:y:2016:i:5:p:947-1012} indicates that do-interventions such explicit edge deletions generate identifiable causal models in the limit that all predictor variables have been independently intervened upon. While this would be computationally intractable, 
% Rather than explicitly construct our estimator, we rely on regularization as a way to balance the complexity and instability of the model in the following way:
\begin{equation}
    \label{eqn:full_objective}
    \mathcal{L} = \mathcal{L}^{p} + \lambda \mathcal{L}^{c}
\end{equation}

The full loss function $\mathcal{L}$ consists of the loss associated with the prediction $\mathcal{L}^p$, the loss associated with causal attention task $\mathcal{L}^{c}$, and a causal regularization strength hyperparameter $\lambda$ that mediates the contribution of the regularization loss to the objective. For the prediction loss, we have $\mathcal{L}^p=\frac{1}{N}\sum_{n=1}^{N}\ell^p(\hat{y}^{(n)}, y^{(n)})$, where $N$ is the size of the training set, $\ell^p(\cdot,\cdot)$ corresponds to the loss function for the given prediction task, $\hat{y}^{(n)}$ is the prediction for entity $n$, and $y^{(n)}$ is the ground truth value for entity $n$. We seek to align the attention coefficient for an edge with the causal effect of removing that edge through the use of the following loss function:
\begin{equation}
    \label{eqn:causal_reg}
    \mathcal{L}^{c} = \frac{1}{R} \sum^{R}_{r=1} \bigg( \frac{1}{\left| S^{\left( r \right )} \right|}\sum_{\left(n, i, j \right) \in S^{\left( r \right ) }} \ell^{c} \left( \alpha_{ij}^{(n)}, c_{ij}^{(n)} \right) \bigg)
\end{equation}
Here, $n$ represents a single entity for which we aim to make a prediction. For a node prediction task, the entity $n$ corresponds to a node, and in a graph prediction task, $n$ corresponds to a graph. In this paper, we assume that all edges are directed and, if necessary, decompose an undirected edge into two directed edges. In each mini-batch, we generate $R$ separate sub-models, each of which consists of a set of edge interventions $S^{(r)}$, $r=1,\ldots,R$. Each edge intervention in $S^{(r)}$ is represented by a set of tuples $(n,i,j)$ which denote a selected edge $(i,j)$ for an entity $n$. Note that in a node classification task, $n$ is the same as $j$ (i.e., the node with the incoming edge). More details for the edge intervention procedure and causal effect calculations can be found in the sections below. The causal effect $c_{ij}^{(n)}$ scores the impact of deleting edge $(i,j)$ through a likelihood ratio test. This causal effect is compared to the edge's attention coefficient $\alpha_{ij}^{(n)}$ via the loss function $\ell^c(\cdot,\cdot)$. A detailed algorithm for \methodname is provided in algorithm~\ref{alg:cap}.

\begin{algorithm}
\caption{\methodname Framework}\label{alg:cap}
\begin{algorithmic}
\Require Training set $\mathcal{D}_{train}$, validation set $\mathcal{D}_{val}$, model $\mathcal{M}$, regularization strength $\lambda$
% \Ensure $y = x^n$
\Repeat % For {$\text{epoch } i \gets 1 \text{ to } M$}
    \ForEach {$\text{mini-batch } \{ \mathcal{B}^k = \{n_j^{(k)}\}_{j=1}^{b_k}\}$}
    \State $\text{Prediction loss: } \mathcal{L}^p \gets \frac{1}{|\mathcal{B}^k|}\sum_{n \in \mathcal{B}^k}\ell^p(\hat{y}^{(n)}, y^{(n)}) $
    \Procedure{Edge intervention}{}
    \State $\text{Causal attention loss: } \mathcal{L}^c \gets 0$
    \For {$\text{round } r \gets 1 \text{ to } R$}
        \State {$\text{Set of edge interventions } S(r) \gets \{\}$}
        \ForEach {$\text{entity } \{n_j^{(k)}\}_{j=1}^{b_k}$}
        \State $\text{Sample edge }(i,j) \sim E_{n_j^{(k)}}$ \Comment{$E_{n_j^{(k)}}$ set of edges related to entity $n_j^{(k)}$}
        %\If {$(i,j) \text{ only affects } n_j^{(k)}$} \Comment{See ``Edge intervention procedure"}
        \If {$(i,j) \text{ independent of } S(r)$} \Comment{See ``Edge intervention procedure"}
            \State $S(r) \gets S(r) \text{ } \cup (n_j^{(k)},i,j)$  \Comment{Add edge to set of edge interventions}
            \State $\text{Compute causal effect } c_{ij}^{(n)} \gets \sigma \big( \big( \rho^{(n)}_{ij} \big)^{d(n)} - 1 \big)$ \Comment{Equation 5}
        \EndIf
        \EndFor
    \State $\mathcal{L}^{c} \gets \mathcal{L}^{c} + \frac{1}{R}  \frac{1}{\left| S^{\left( r \right )} \right|}\sum_{\left(n, i, j \right) \in S^{\left( r \right ) }} \ell^{c} \left( \alpha_{ij}^{(n)}, c_{ij}^{(n)} \right)$ \Comment{Equation 3}
    \EndFor
    \EndProcedure
    \State $\text{Total loss: } \mathcal{L} = \mathcal{L}^{p} + \lambda\mathcal{L}^{c}$
    \State $\text{Update model parameters to minimize } \mathcal{L}$
    \EndFor
\Until $\text{Convergence criterion}$ \Comment{We use convergence of the validation prediction loss.}
% \EndFor
\end{algorithmic}
\end{algorithm}

% For models with multiple attention heads, $\alpha_{ij}^{(n)}$ is the mean attention coefficient across heads.

% We regularize the attention mechanism in accordance with the learned causal effects from edge interventions. Thus, our full objective function $\mathcal{L}$ includes the loss associated with the prediction $\mathcal{L}^p$, the loss associated with causal attention task $\mathcal{L}^{c}$, and a causal regularization strength hyperparameter $\lambda$ that mediates the contribution of the causal attention task to the objective. 

% We formalize this intuition by devising an auxiliary supervised prediction task that aims to align the attention coefficient for an edge with the causal effect of removing that edge as per the following loss function:


% \paragraph{Causal attention objective}
% We leverage the intuition that relevant node-neighbor relations for a particular task should not only be assigned high attention coefficients but also be important to the predictive accuracy of the model (\textbf{Figure} \ref{fig:figure_1}). When removed from the graph, these relevant edges should cause the predictions that rely on them to substantially worsen. We formalize this intuition by devising an auxiliary supervised prediction task that aims to align the attention coefficient for an edge with the causal effect of removing that edge as per the following loss function:
% \begin{equation}
%     \label{eqn:causal_reg}
%     \mathcal{L}^{c} = \frac{1}{R} \sum^{R}_{r=1} \bigg( \frac{1}{\left| S^{\left( r \right )} \right|}\sum_{\left(n, i, j \right) \in S^{\left( r \right ) }} \ell^{c} \left( \alpha_{ij}^{(n)}, c_{ij}^{(n)} \right) \bigg)
% \end{equation}
% \begin{equation}
%     \label{eqn:causal_reg}
%     \mathcal{L}^{c} = \frac{1}{N} \sum^{N}_{n=1} \frac{1}{\left| S^{\left( n \right )} \right|} \sum_{\left( i, j \right) \in S^{\left( n \right ) }} \ell^{c} \left( \alpha_{ij}^{(n)}, c_{ij}^{(n)} \right)
% \end{equation}

% Here, $n$ represents a single entity for which we aim to make a prediction. For a node prediction task, $n$ corresponds to a node, while in a graph prediction task, $n$ corresponds to a graph. $N$ represents the number of such entities in the training set. $\alpha_{ij}^{(n)}$ is the attention coefficient associated with edge $(i,j)$ for entity $n$. For models with multiple attention heads, $\alpha_{ij}^{(n)}$ is the mean attention coefficient for edge $(i,j)$ for entity $n$ across the attention heads. 

% $S^{(n)}$ denotes a set of edges $(i,j)$ associated with entity $n$ that will be individually removed from the training data to compute the causal effect $c_{ij}^{(n)}$. Importantly, we select only one edge per entity to remove in computing $c_{ij}^{(n)}$, so that the direct causal effect of each intervention can be calculated independently of other interventions. $\ell^c(\cdot,\cdot)$ is the loss function used to compare the attention coefficients and the causal effects, which we refer to as the causal regularization loss. 


% Here, $n$ represents a single entity for which we aim to make a prediction. For a node prediction task, the entity $n$ corresponds to a node, and in a graph prediction task, $n$ corresponds to a graph. In this paper, we assume that all edges are directed and, if necessary, decompose an undirected edge into two directed edges. In each mini-batch, we perform $R$ separate rounds of causal effect calculations, each of which consists of a set of edge interventions $S^{(r)}$, $r=1,\ldots,R$. More details for the edge intervention procedure and causal effect calculations can be found in the sections below. 

% Each edge intervention in $S^{(r)}$ is represented by a set of tuples $(n,i,j)$ which denote a selected edge $(i,j)$ for an entity $n$. Note that in a node classification task, $n$ is the same as $j$ (i.e., the node with the incoming edge). The causal effect $c_{ij}^{(n)}$ scores the impact of deleting edge $(i,j)$ on predictive performance. This causal effect is compared to the edge's attention coefficient $\alpha_{ij}^{(n)}$ via the loss function $\ell^c(\cdot,\cdot)$. For models with multiple attention heads, $\alpha_{ij}^{(n)}$ is the mean attention coefficient across heads.

% We regularize the attention mechanism in accordance with the learned causal effects from edge interventions. Thus, our full objective function $\mathcal{L}$ includes the loss associated with the prediction $\mathcal{L}^p$, the loss associated with causal attention task $\mathcal{L}^{c}$, and a causal regularization strength hyperparameter $\lambda$ that mediates the contribution of the causal attention task to the objective. 

% \begin{equation}
%     \label{eqn:full_objective}
%     \mathcal{L} = \mathcal{L}^{p} + \lambda \mathcal{L}^{c}
% \end{equation}
% Here, we have $\mathcal{L}^p=\frac{1}{N}\sum_{n=1}^{N}\ell^p(\hat{y}^{(n)}, y^{(n)})$, where $N$ is the size of the training set, $\ell^p(\cdot,\cdot)$ corresponds to the loss function for the given prediction task, $\hat{y}^{(n)}$ is the prediction for entity $n$, and $y^{(n)}$ is the ground truth value for entity $n$. A detailed algorithm for \methodname is provided in \textbf{Appendix} \ref{appen:algo}.

\paragraph{Edge intervention procedure}
% Classification tasks on graphs can be understood as estimating $p( C | \mathcal{G}, \mathcal{X} ) = p(C | S) $, where $\mathcal{G}$ is the graph structure, $\mathcal{X}$ is the set of features associated with the graph $\mathcal{G}$, and $S$ is the set of predictor variables. For node classification, the node label is the target variable of interest, and the model is composed of the adjacency matrix and the method by which probabilities are computed. To construct a GNN capable of causal inference, we require a technique to generate different sub-models and experiments with different conditional dependence structures. Each sub-model will have the same GNN structure but a slightly different graph structure generated via edge-removal. Given a set of experiments $\{ \mathcal{E} \}$, with target variables $Y^e$ and predictor variables $S^e$, we say that the subset of latent variables, $S^*$, is causal for the prediction of target variable $Y$ if for all $e \in \mathcal{E}$, $S^e$ has an arbitrary distribution and $Y^e = g(S^e, \epsilon^e)$ where $g$ is our statistical model, and $\epsilon^e \sim F_{\epsilon}$ is the error distribution.
%
We sample a set of edges in each round $r$ such that the prediction for each entity will strictly be affected by at most one edge intervention in that round to ensure effect independence. For example, in a node classification task for a model with one GNN layer, a round of edge interventions entails removing only a single incoming edge for each node being classified. In the graph property prediction case, only one edge will be removed from each graph per round. Because a model with one GNN layer only aggregates information over a 1-hop neighborhood, the removal of each edge will only affect the model's prediction for that edge's target node. To select a set of edges in the $L$-layer GNN case, edges are sampled from the 1-hop neighborhood of each node being classified, and sampled edges that lie in more than one target nodes' $L$-hop neighborhood are removed from consideration as intervention candidates. %; this limits the computational expense of interventions. 

This edge intervention selection procedure is crucial, as it enables the causal effect of each selected intervention $c_{ij}^{(n)}$ on an entity $n$ to be calculated independently of other interventions on a graph. Moreover, by selecting only one intervention per entity within each round, we can parallelize the computation of these causal effects across all entities per round instead of iteratively evaluating just one intervention for the entire graph per entity, significantly aiding scalability. 
 
\paragraph{Calculating task-specific causal effects}
\label{subsec:methods:causaleffect}
We quantify the causal effect of an intervention at edge $(i,j)$ on entity $n$ through the use of an approximate likelihood-ratio test

% as the relative change in the prediction loss for entity $n$ upon removal of that edge.
% \begin{equation}
%     \label{eqn:causal_effect}
%     c_{ij}^{(n)} = \sigma \bigg( \bigg( \frac{\ell^p \bigl( \hat{y}_{\backslash ij}^{(n)}, y^{(n)} \bigr)} {\ell^p \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)} \bigg)^{d(n)}  -1 \bigg)
% \end{equation}

\begin{equation}
    \label{eqn:causal_effect}
    c_{ij}^{(n)} = \sigma \bigg( \bigg( \rho^{(n)}_{ij} \bigg)^{d(n)} - 1 \bigg)\;\;\;\text{where}\;\; \rho^{(n)}_{ij} = \frac{\ell^p \bigl( \hat{y}_{\backslash ij}^{(n)}, y^{(n)} \bigr)} {\ell^p \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)}
\end{equation}

% \begin{equation}
%     \label{eqn:causal_effect}
%     c_{ij}^{(n)} = \sigma \bigg( \frac{\ell^p \bigl( \hat{y}_{\backslash ij}^{(n)}, y^{(n)} \bigr)-\ell^p \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)} {\ell^p \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)} \bigg)
% \end{equation}
Here, $\hat{y}_{\backslash ij}^{(n)}$ is the prediction for entity $n$ upon removal of edge $(i,j)$. $d(n)$ represents the node degree for node classification, while it represents the number of edges in a graph for graph classification. Interventions will likely have smaller effects on higher degree nodes due to the increased likelihood of there being multiple edges that are relevant and beneficial for predictions for such nodes. In graph classification, graphs with many edges are likely to be less affected by interventions as well. Exponentiating the relative intervention effect $\rho^{(n)}_{ij}$ by $d(n)$ is intended to adjust for these biases. We have experimented both with and without raising $\rho$ to the factor of $d$, but have found empirically better results with. We do not have a rigorous explanation as to why, although we suspect the correlated nature of edges implies some amount of shrinkage is necessary. 

% $\ell^p \bigl( \hat{y}_{\backslash ij}^{(n)}, y^{(n)} \bigr) / \ell^p \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)$ so as to account for the number of edges contributing to the prediction for entity $n$. For example, in node classification tasks, predictions for a high-degree node will involve aggregating information over many neighbors, so the effect of a single edge intervention is adjusted via this $d(n)$ term to account for this specific node's high-degree context. 
The link function $\sigma : \mathbb{R} \rightarrow (0,1)$ maps its input to the support of the distribution of attention coefficients. The predictions $\hat{y}^{(n)}$ and $\hat{y}_{\backslash ij}^{(n)}$ are generated from the graph attention network being trained with \methodname. We emphasize that $\hat{y}^{(n)}$ and $\hat{y}_{\backslash ij}^{(n)}$ are both computed during the same training run, rather than in two separate runs. 

% \RS{@AW: the two y's are computed in a single run, right? pls clarify that as a line here?}
% \AW{added another sentence. is this what you mean?}
% %Furthermore, by using the prediction loss in these calculations, \methodname guides attention learning in a manner that is aware of the causal effects on the specific prediction task at hand. 

\paragraph{Scalability}
\methodname increases the computational cost of training in two ways: (i) additional evaluations of the loss function due to the causal effect calculations, and (ii) searches to ensure independent interventions. \methodname performs $\mathcal{O}(RN)$ interventions, where $R$ is the number of interventions per entity and $N$ is the number of entities in the training set. Because our edge intervention procedure ensures that the sampled interventions per round are independent, the causal effects of these interventions can be computed in parallel. In addition, if edge interventions were sampled uniformly across the graph, ensuring the independence each intervention would require a $L$-layer deep BFS that has time complexity $\mathcal{O}(b^L)$, resulting in a worst case time complexity of $\mathcal{O}(R N b^L)$, where $L$ is the depth of the GNN, and $b$ is the mean in-degree. We note that, in practice, GNNs usually have $L \leq 2$ layers since greater depth increases the computational cost and the risk of oversmoothing~\citep{gcn_oversmoothing,measuring_oversmoothing,topping2022understanding}. The contribution of this intervention overlap search step would, therefore, be minimal for most GNNs. We are also able to mitigate much of the computational cost by parallelizing these searches. Further speedups can achieved by identifying non-overlapping interventions as a preprocessing step. In summary, we have found \methodname to have a modest effect on the scalability of graph attention methods, with training runtimes that are only increased by 1.5-2 fold (\textbf{Appendix} \ref{appen:runtime_memory}).

%We have found \methodname to be highly scalable, with training runtimes that are only 1.5-2x of non-regularized attention training (Appendix \ref{appen:runtime_memory}).

% \TM{ Number of interventions scales as $O(C * |V|)$. Each intervention scales as $O(b^2l)$ due to the BFS to ensure non-overlapping interventions, where b is the branching factor and l is the number of layers. In the long run, we're unconcerned about the identification of non-overlapping interventions can be done as a preprocessing step, similar to the generation of graph samples in graph sage.}


==> iclr2023/backup-20230214/todos.tex <==
\todo[inline]{
Todos: \\
1. P0 Results: \\
 \;\; - \sout{Abstract: need a summary stat or two} \\
 \;\; - Ablations: a) in appendix: need table of correlations between attn wts and homophily scores. b) put in line markers for what random baseline will be \\ 
 \;\; - \sout{Ablations: need label-propagation results} \\
 \;\; - Scalability: need runtimes and machine details \\
2. P0 Writing: \\
 \;\; - \sout{Interpretability: which dataset? \TM{ogbn-arxiv}} \\
3. P1 Results: \\
 \;\; - Fig 3: needs other 3 datasets (in appendix). Also needs p-values \\
 \;\; - Extra: graph property-prediction + graph rewiring. Ok to have limited examples \\
 \;\; - random/uniform regularization 
 \;\; - Should we worry about graph diffusion distance and cheeger constant stuff? Could be a solid appendix section

}


==> iclr2023/backup-20230214/v1_theory.tex <==
\subsection{Graph Attention Networks}

Attention mechanisms have been effectively used across many domains by enabling models to dynamically attend to the specific parts of an input that are most relevant to a prediction task \citep{attention_survey}. In graph settings, attention mechanisms compute the relevance of node-neighbor relations. The neighbor aggregation operator in GNNs then uses this information to weight the contribution of each node-neighbor relation in the prediction task. 

Across the multitude of graph attention mechanisms that have been proposed \citep{gat_survey}, the procedures for computing attention take on a general form \citep{gat}. A graph attention layer takes as input a set of node features $\mathbf{h} = \{\vec{h}_1,...,\vec{h}_N\}$, $\vec{h}_i \in \mathbb{R}^F$, where $N$ is the number of nodes and $F$ is the dimensionality of the node features. From these node features, the graph attention layer in a GAT computes unnormalized attention weights for each edge $(i,j)$
\begin{equation}
    \label{eqn:attn_edges}
    e_{ij} = a(\mathbf{W}\vec{h}_i,\mathbf{W}\vec{h}_j),
\end{equation}
where $\mathbf{W}\in \mathbb{R}^{F' \times F}$ linearly projects the input features into a new feature space and the attention mechanism function $a : \mathbb{R}^{F'} \times \mathbb{R}^{F'} \rightarrow \mathbb{R}$ uses these new node features to compute an attention weight for each edge. These attention weights are typically normalized with respect to the 1-hop neighborhood of each node using the softmax function, yielding normalized attention coefficients $\alpha_{ij}$ that indicate the importance of node $i$'s input features to node $j$. For a node $j$, these normalized attention weights are then used to compute a linear combination of the new features for node $j$'s neighbors, which serves as the output of the graph attention layer for node $j$.
\begin{equation}
    \label{eqn:attn_aggr}
    \vec{h}_j' =  \sum_{i\in N_j}\alpha_{ij}\mathbf{W}\vec{h}_i
\end{equation} 
% 
To employ multi-headed attention with $K$ heads, each of the $K$ attention mechanisms first independently calculates its respective normalized attention weights $\alpha_{i,j}^{(k)}$ using its own attention mechanism function $a^{(k)}( \cdot )$ and linear projection weights $\mathbf{W}^{(k)}$. These attention weights are used to compute attention head-specific node outputs $\vec{h}_j'^{(k)}$, which are then averaged across the $K$ attention heads.
\begin{equation}
    \label{eqn:attn_heads}
    \vec{h}_j' = \frac{1}{K}\sum_{k=1}^{K}\vec{h}_j'^{(k)}
\end{equation}

In this paper, we focus on three widely used graph attention architectures: the original graph attention network (GAT) \citep{gat}, a modified version of this original network (GATv2) \citep{gatv2}, and the Graph Transformer network \cite{transformerconv}. These graph attention architecture variants are distinguished by the manner in which they compute the unnormalized attention weights $e_{ij}$ (Table \ref{table:gat_variants}). Here, $||$ denotes concatenation. For GAT and GATv2, the concatenated node features are passed through a single-layer feedforward neural network featuring a weight vector $\mathbf{a} \in \mathbb{R}^{2F'}$ and the LeakyReLU nonlinearity. 

\begin{table}[h!]
\centering
\caption{Attention weight calculation across graph attention architecture variants}
\label{table:gat_variants}
\renewcommand{\arraystretch}{2.5}
\begin{tabular}{ | c | c |} 
    \hline
    GAT \citep{gat} & \(\displaystyle e_{ij} = \text{LeakyReLU}\big(\vec{\mathbf{a}}^T [ \mathbf{W}\vec{h}_i || \mathbf{W}\vec{h}_j \big)]\big) \)  \\
    \hline
    GATv2 \citep{gatv2} & \(\displaystyle e_{ij} = \vec{\mathbf{a}}^T\text{LeakyReLU}\big( \mathbf{W} \vec{h}_i || \mathbf{W} \vec{h}_j \big) \) \\ 
    \hline
    Graph Transformer \citep{transformerconv} & \(\displaystyle e_{ij} = \frac{(\mathbf{W}\vec{h}_i)^T(\mathbf{W}\vec{h}_j)}{\sqrt{F'}} \) \\ 
    \hline
\end{tabular}
\end{table}

% In the original graph attention network (GAT) framework, the unnormalized attention weights are computed as follows \citep{gat}. Here, $||$ denotes concatenation and the concatenated node features are passed through a single-layer feedforward neural network featuring a weight vector $\mathbf{a} \in \mathbb{R}^{2F'}$ and the LeakyRELU nonlinearity. 
% \begin{equation}
%     \label{eqn:gat_attn}
%     e_{ij} = \text{LeakyReLU}\big(\vec{\mathbf{a}}^T [ \mathbf{W}\vec{h}_i || \mathbf{W}\vec{h}_j \big)]\big)
% \end{equation}
% GATv2 was proposed to improve upon the expressiveness of the original graph attention mechanism by applying the linear projection to concatenated input node features instead of individual node features \citep{gatv2}.
% \begin{equation}
%     \label{eqn:gatv2_attn}
%     e_{ij} = \vec{\mathbf{a}}^T\text{LeakyReLU}\big( \mathbf{W} \vec{h}_i || \mathbf{W} \vec{h}_j \big)
% \end{equation}
% Lastly, the Graph Transformer network extends the Transformer architecture used in natural language processing \citep{transformer} to graphs and computes the attention weights as follows, where as above $F'$ is the dimensionality of the new feature space \citep{transformerconv}. 
% \begin{equation}
%     \label{eqn:transformer_attn}
%     e_{ij} = \frac{(\mathbf{W}\vec{h}_i)^T(\mathbf{W}\vec{h}_j)}{\sqrt{F'}}
% \end{equation}

\subsection{Causal Attention Regularization Scheme}

We propose a general-purpose regularization framework for graph attention networks that enhances a given learning task by including an attention learning scheme based on active graph interventions. In this framework, we leverage the intuition that relevant node-neighbor relations for a particular task should not only be assigned high attention weights but also be important to the predictive accuracy of the model. When removed from the graph, these relevant edges should cause the predictions that rely on them to dramatically worsen. 

\subsubsection{Causal Attention Objective}
We formalize this intuition by devising a weakly supervised prediction task that aims to align the attention weight for an edge with the causal effect of removing that edge. The objective function for this task is as follows. 
\\
\begin{equation}
    \label{eqn:causal_reg}
    \mathcal{L}^{c} = \frac{1}{R} \sum^{R}_{r=1} \frac{1}{\left| S^{\left( r \right )} \right|}\sum_{\left(n, i, j \right) \in S^{\left( r \right ) }} \ell^{c} \left( \alpha_{ij}^{(n)}, c_{ij}^{(n)} \right)
\end{equation}
% \begin{equation}
%     \label{eqn:causal_reg}
%     \mathcal{L}^{c} = \frac{1}{N} \sum^{N}_{n=1} \frac{1}{\left| S^{\left( n \right )} \right|} \sum_{\left( i, j \right) \in S^{\left( n \right ) }} \ell^{c} \left( \alpha_{ij}^{(n)}, c_{ij}^{(n)} \right)
% \end{equation}

% Here, $n$ represents a single entity for which we aim to make a prediction. For a node prediction task, $n$ corresponds to a node, while in a graph prediction task, $n$ corresponds to a graph. $N$ represents the number of such entities in the training set. $\alpha_{ij}^{(n)}$ is the attention weight associated with edge $(i,j)$ for entity $n$. For models with multiple attention heads, $\alpha_{ij}^{(n)}$ is the mean attention weight for edge $(i,j)$ for entity $n$ across the attention heads. 

% $S^{(n)}$ denotes a set of edges $(i,j)$ associated with entity $n$ that will be individually removed from the training data to compute the causal effect $c_{ij}^{(n)}$. Importantly, we select only one edge per entity to remove in computing $c_{ij}^{(n)}$, so that the direct causal effect of each intervention can be calculated independently of other interventions. $\ell^c(\cdot,\cdot)$ is the loss function used to compare the attention weights and the causal effects, which we refer to as the causal regularization loss. 

Here, $n$ represents a single entity for which we aim to make a prediction. For a node prediction task, $n$ corresponds to a node, while in a graph prediction task, $n$ corresponds to a graph. We perform $R$ rounds of edge interventions per mini-batch, sampling a set of edges in each round such that the prediction for each entity in the mini-batch will strictly be affected by at most one edge intervention in that round. For example, in a node classification task for a model with one GNN layer, one round of edge interventions for a mini-batch entails removing only a single incoming edge for each node being classified in the mini-batch. Because a model with one GNN layer only aggregates information over a 1-hop neighborhood, the removal of each edge will only affect the model's prediction for that edge's target node. Similarly, in the graph property prediction case, only one edge will be removed from each graph per round. $S^{(r)}$ denotes a set of tuples $(n,i,j)$, each of which corresponds to a selected edge $(i,j)$ for an entity $n$ in round $r$. 

This edge intervention selection procedure is crucial, as it enables the direct causal effect of each selected intervention $c_{ij}^{(n)}$ on an entity $n$ to be calculated independently of other interventions. Furthermore, by selecting only one intervention per entity within each round, we can parallelize the computation of these direct causal effects across all entities per round, enabling the causal effect calculations to be highly scalable. Each causal effect $c_{ij}^{(n)}$ is compared to the attention weight $\alpha_{ij}^{(n)}$ of its corresponding edge via the loss function $\ell^c(\cdot,\cdot)$. For models with multiple attention heads, $\alpha_{ij}^{(n)}$ is the mean attention weight for edge $(i,j)$ for entity $n$ across the attention heads.

We quantify the causal effect $c_{ij}$ of removing edge $(i,j)$ on the prediction for entity $n$ as follows. 
\begin{equation}
    \label{eqn:causal_effect}
    c_{ij}^{(n)} = \sigma \bigg( \frac{\ell \bigl( \hat{y}_{\backslash ij}^{(n)}, y^{(n)} \bigr)-\ell \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)} {\ell \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)} \bigg)
\end{equation}
% talk about importance of using prediction loss to compute causal effect instead of just change in predictions???
$\ell^p(\cdot,\cdot)$ corresponds to the loss function for the given prediction task, $\hat{y}^{(n)}$ is the prediction for entity $n$, $\hat{y}_{\backslash ij}^{(n)}$ is the prediction for entity $n$ upon removal of edge $(i,j)$, and $y^{(n)}$ is the ground truth value for entity $n$. We also include $\sigma(\cdot)$ as a link function that maps its input to the support of the distribution of attention weights. 

We include the above learning task as an additional task to be optimized during training so as to regularize the attention mechanism in accordance with the learned causal effects from edge interventions. Thus, our full objective function $\mathcal{L}$ includes the loss associated with the prediction $\mathcal{L}^p$, the loss associated with causal attention task $\mathcal{L}^{c}$, and a causal regularization strength hyperparameter $\lambda$ that mediates the contribution of the causal attention task to the objective.
\begin{equation}
    \label{eqn:full_objective}
    \mathcal{L} = \mathcal{L}^{p} + \lambda \mathcal{L}^{c}
\end{equation}

==> iclr2023/backup-20230214/v2_theory.tex <==
\subsection{Graph Attention Networks}

Attention mechanisms have been effectively used in many domains by enabling models to dynamically attend to the specific parts of an input that are relevant to a prediction task \citep{attention_survey}. In graph settings, attention mechanisms compute the relevance of edges in the graph for a prediction task. A neighbor aggregation operator then uses this information to weight the contribution of each edge \citep{gat_survey,gated_graph_sequence,self_attn_graph_pooling}. 

The approach for computing attention is similar in many graph attention mechanisms. A graph attention layer takes as input a set of node features $\mathbf{h} = \{\vec{h}_1,...,\vec{h}_N\}$, $\vec{h}_i \in \mathbb{R}^F$, where $N$ is the number of nodes. The graph attention layer uses these node features to compute attention coefficients for each edge: $\alpha_{ij} = a(\mathbf{W}\vec{h}_i,\mathbf{W}\vec{h}_j)$, 
% \begin{equation}
%     \label{eqn:attn_edges}
%     e_{ij} = a(\mathbf{W}\vec{h}_i,\mathbf{W}\vec{h}_j),
% \end{equation}
where $a : \mathbb{R}^{F'} \times \mathbb{R}^{F'} \rightarrow (0,1)$ is the attention mechanism function, and the attention coefficient $\alpha_{ij}$ for an edge indicates the importance of node $i$'s input features to node $j$.
% $\mathbf{W}\in \mathbb{R}^{F' \times F}$ projects the input features into a new feature space. The attention mechanism function $a : \mathbb{R}^{F'} \times \mathbb{R}^{F'} \rightarrow [0,1]$ uses these new node features to compute an attention coefficient $\alpha_{ij}$ for each edge that indicates the importance of node $i$'s input features to node $j$. 
% These attention coefficients are typically normalized with respect to the 1-hop neighborhood of each node using the softmax function, yielding normalized attention coefficients $\alpha_{ij}$ that indicate the importance of node $i$'s input features to node $j$.
For a node $j$, these attention coefficients are then used to compute a linear combination of its neighbors' features: $\vec{h}_j' =  \sum_{i\in N(j)}\alpha_{ij}\mathbf{W}\vec{h}_i, ~ ~ \mathit{s.t.} ~ \sum_{i\in N(j)} \alpha_{ij} = 1$.
For multi-headed attention, each of the $K$ heads first independently calculates its own attention coefficients $\alpha_{i,j}^{(k)}$ with its head-specific attention mechanism $a^{(k)}(\cdot,\cdot)$, after which the head-specific outputs are averaged. 
% \begin{equation}
%     \label{eqn:attn_aggr}
%     \vec{h}_j' =  \sum_{i\in N(j)}\alpha_{ij}\mathbf{W}\vec{h}_i,
%     ~ ~ \mathit{s.t.} ~ 
%     \sum_{i\in N(j)} \alpha_{ij} = 1
% \end{equation} 
% 

%RS: commenting out to save some space and make room for causal in the intro
%
%se attention coefficients are used to compute attention-head specific node outputs $\vec{h}_j'^{(k)}$, which are then averaged across the $K$ attention heads.
%
% \begin{equation}
%     \label{eqn:attn_heads}
%     \vec{h}_j' = \frac{1}{K}\sum_{k=1}^{K}\vec{h}_j'^{(k)}
% \end{equation}

In this paper, we focus on three widely used graph attention architectures: the original graph attention network (GAT) \citep{gat}, a modified version of this original network (GATv2) \citep{gatv2}, and the Graph Transformer network \citep{transformerconv}. %These graph attention architecture variants are distinguished by the manner in which they compute the unnormalized attention coefficients $e_{ij}$ (Table \ref{table:gat_variants}). 
The three architectures and their equations for computing attention  are presented in \textbf{Appendix} \ref{appen:gat_variants}. 

% In the original graph attention network (GAT) framework, the unnormalized attention coefficients are computed as follows \citep{gat}. Here, $||$ denotes concatenation and the concatenated node features are passed through a single-layer feedforward neural network featuring a weight vector $\mathbf{a} \in \mathbb{R}^{2F'}$ and the LeakyRELU nonlinearity. 
% \begin{equation}
%     \label{eqn:gat_attn}
%     e_{ij} = \text{LeakyReLU}\big(\vec{\mathbf{a}}^T [ \mathbf{W}\vec{h}_i || \mathbf{W}\vec{h}_j \big)]\big)
% \end{equation}
% GATv2 was proposed to improve upon the expressiveness of the original graph attention mechanism by applying the linear projection to concatenated input node features instead of individual node features \citep{gatv2}.
% \begin{equation}
%     \label{eqn:gatv2_attn}
%     e_{ij} = \vec{\mathbf{a}}^T\text{LeakyReLU}\big( \mathbf{W} \vec{h}_i || \mathbf{W} \vec{h}_j \big)
% \end{equation}
% Lastly, the Graph Transformer network extends the Transformer architecture used in natural language processing \citep{transformer} to graphs and computes the attention coefficients as follows, where as above $F'$ is the dimensionality of the new feature space \citep{transformerconv}. 
% \begin{equation}
%     \label{eqn:transformer_attn}
%     e_{ij} = \frac{(\mathbf{W}\vec{h}_i)^T(\mathbf{W}\vec{h}_j)}{\sqrt{F'}}
% \end{equation}

\begin{figure}
    \centering
    %\includegraphics[width=0.95 \linewidth ]{iclr2023/causal_attn_fig1_rs-v4.pdf}
    \includegraphics[width=0.9 \linewidth ]{car_regularization_overview.pdf}
    \caption{Schematic of \methodname: Graph attention networks learn the relative importance of each node-neighbor for a given prediction task. However, their inferred attention coefficients can be miscalibrated due to noise, spurious correlations, or confounders (e.g., node size here). Our causal approach directly intervenes on a sampled subset of edges and supervises an auxiliary task that aligns an edge's causal importance to the task with its attention coefficient.}
    \label{fig:figure_1}
\end{figure}

\subsection{Causal Attention Regularization Scheme}

\methodname is motivated by the invariant prediction (IP) formulation of causal inference \citep{RePEc:bla:jorssb:v:78:y:2016:i:5:p:947-1012}. The central insight of this formulation is that, given sub-models that each contain a different set of predictor variables, the underlying causal model of a system is comprised of the set of all sub-models for which the target-variable marginals are equivalent. This approach is capable of providing statistically rigorous estimates for both the causal effect strength of predictor variables as well as confidence intervals. We leverage the residual formulation of IP, which assumes that we can generate many sub-models with different sets of predictor variables $S^e$ corresponding to many different experiments. We can compute the predictions, $Y^e$ for every sub-model as well as the residuals $\mathcal{R} = Y - Y^e$. IP requires that we perform a hypothesis test on the means of the residuals. The generic method for invariant prediction is to test each hypothetical set of features against the null-hypothesis, $H_{0,S}(\mathcal{E})$, such that there exists $g: \mathbb{R}^{|S|} \times \mathbb{R} \rightarrow \mathbb{R}$ and $\epsilon^e$ that $Y^e = g(\mathcal{G}^e_S, \mathcal{X}^e_S, \epsilon^e)$, $\epsilon^e \sim F_\epsilon$ and $\epsilon^e \indep S^e$ for all $e \in \mathcal{E}$. This is satisfied if the conditionals $Y^e|S^e$ and $Y^f | S^f$ are identical for all experiments $e, f \in \mathcal{E}$. IP then provides a method to construct an estimator of the true causal model by taking the intersection of all models for which the null hypothesis was rejected. 

% Classification tasks on graphs can be understood as estimating $p( C | \mathcal{G}, \mathcal{X} ) = p(C | S) $, where $\mathcal{G}$ is the graph structure, $\mathcal{X}$ is the set of features associated with the graph $\mathcal{G}$, and $S$ is the set of predictor variables. For node classification, the node label is the target variable of interest, and the model is composed of the adjacency matrix and the method by which probabilities are computed. 

To construct a GNN capable of causal inference, we require a technique to generate different sub-models and experiments with different conditional dependence structures. Each sub-model will have the same GNN structure but a slightly different graph structure generated via edge-removal. Given a set of experiments $\{ \mathcal{E} \}$, with target variables $Y^e$ and predictor variables $S^e$, we say that the subset of latent variables, $S^*$, is causal for the prediction of target variable $Y$ if for all $e \in \mathcal{E}$, $S^e$ has an arbitrary distribution and $Y^e = g(S^e, \epsilon^e)$ where $g$ is our statistical model, and $\epsilon^e \sim F_{\epsilon}$ is the error distribution.

The core insight of \methodname is that the graph structure itself is a set of predictor variables in addition to the set of node features.
% that are traditionally explored in causal regularization frameworks. 
This is equivalent to the intuition that relevant edges for a particular task should not only be assigned high attention coefficients but also be important to the predictive accuracy of the model (\textbf{Figure} \ref{fig:figure_1}). When removed from the graph, these relevant edges should cause the predictions that rely on them to substantially worsen. We formalize this intuition by devising an auxiliary supervised prediction task that aims to align the attention coefficient for an edge with the causal effect of removing that edge as per the following loss function:
\begin{equation}
    \label{eqn:causal_reg}
    \mathcal{L}^{c} = \frac{1}{R} \sum^{R}_{r=1} \bigg( \frac{1}{\left| S^{\left( r \right )} \right|}\sum_{\left(n, i, j \right) \in S^{\left( r \right ) }} \ell^{c} \left( \alpha_{ij}^{(n)}, c_{ij}^{(n)} \right) \bigg)
\end{equation}

% We begin by briefly presenting the residual formulation of invariant prediction and then discuss in detail our notion of predictor variable, experiment generation, and experiment test. 
% A key question in causal inference is the identification of identifiable models. Theorem 2 of \citet{RePEc:bla:jorssb:v:78:y:2016:i:5:p:947-1012} indicates that do-interventions such explicit edge deletions generate identifiable causal models in the limit that all predictor variables have been independently intervened upon. While this would be computationally intractable, 

Here, $n$ represents a single entity for which we aim to make a prediction. For a node prediction task, the entity $n$ corresponds to a node, and in a graph prediction task, $n$ corresponds to a graph. In this paper, we assume that all edges are directed and, if necessary, decompose an undirected edge into two directed edges. In each mini-batch, we perform generate $R$ separate sub-models, each of which consists of a set of edge interventions $S^{(r)}$, $r=1,\ldots,R$. Each edge intervention in $S^{(r)}$ is represented by a set of tuples $(n,i,j)$ which denote a selected edge $(i,j)$ for an entity $n$. Note that in a node classification task, $n$ is the same as $j$ (i.e., the node with the incoming edge). More details for the edge intervention procedure and causal effect calculations can be found in the sections below. The causal effect $c_{ij}^{(n)}$ scores the impact of deleting edge $(i,j)$ through a likelihood ratio test. This causal effect is compared to the edge's attention coefficient $\alpha_{ij}^{(n)}$ via the loss function $\ell^c(\cdot,\cdot)$. 
% For models with multiple attention heads, $\alpha_{ij}^{(n)}$ is the mean attention coefficient across heads.

We regularize the attention mechanism in accordance with the learned causal effects from edge interventions. Thus, our full objective function $\mathcal{L}$ includes the loss associated with the prediction $\mathcal{L}^p$, the loss associated with causal attention task $\mathcal{L}^{c}$, and a causal regularization strength hyperparameter $\lambda$ that mediates the contribution of the causal attention task to the objective. 
Rather than explicitly construct our estimator, we rely on regularization as a way to balance the complexity and instability of the model in the following way:

\begin{equation}
    \label{eqn:full_objective}
    \mathcal{L} = \mathcal{L}^{p} + \lambda \mathcal{L}^{c}
\end{equation}
Here, we have $\mathcal{L}^p=\frac{1}{N}\sum_{n=1}^{N}\ell^p(\hat{y}^{(n)}, y^{(n)})$, where $N$ is the size of the training set, $\ell^p(\cdot,\cdot)$ corresponds to the loss function for the given prediction task, $\hat{y}^{(n)}$ is the prediction for entity $n$, and $y^{(n)}$ is the ground truth value for entity $n$. A detailed algorithm for \methodname is provided in \textbf{Appendix} \ref{appen:algo}. We seek to align the attention coefficient for an edge with the causal effect of removing that edge through the use of the following loss function:


% \paragraph{Causal attention objective}
% We leverage the intuition that relevant node-neighbor relations for a particular task should not only be assigned high attention coefficients but also be important to the predictive accuracy of the model (\textbf{Figure} \ref{fig:figure_1}). When removed from the graph, these relevant edges should cause the predictions that rely on them to substantially worsen. We formalize this intuition by devising an auxiliary supervised prediction task that aims to align the attention coefficient for an edge with the causal effect of removing that edge as per the following loss function:
% \begin{equation}
%     \label{eqn:causal_reg}
%     \mathcal{L}^{c} = \frac{1}{R} \sum^{R}_{r=1} \bigg( \frac{1}{\left| S^{\left( r \right )} \right|}\sum_{\left(n, i, j \right) \in S^{\left( r \right ) }} \ell^{c} \left( \alpha_{ij}^{(n)}, c_{ij}^{(n)} \right) \bigg)
% \end{equation}
% \begin{equation}
%     \label{eqn:causal_reg}
%     \mathcal{L}^{c} = \frac{1}{N} \sum^{N}_{n=1} \frac{1}{\left| S^{\left( n \right )} \right|} \sum_{\left( i, j \right) \in S^{\left( n \right ) }} \ell^{c} \left( \alpha_{ij}^{(n)}, c_{ij}^{(n)} \right)
% \end{equation}

% Here, $n$ represents a single entity for which we aim to make a prediction. For a node prediction task, $n$ corresponds to a node, while in a graph prediction task, $n$ corresponds to a graph. $N$ represents the number of such entities in the training set. $\alpha_{ij}^{(n)}$ is the attention coefficient associated with edge $(i,j)$ for entity $n$. For models with multiple attention heads, $\alpha_{ij}^{(n)}$ is the mean attention coefficient for edge $(i,j)$ for entity $n$ across the attention heads. 

% $S^{(n)}$ denotes a set of edges $(i,j)$ associated with entity $n$ that will be individually removed from the training data to compute the causal effect $c_{ij}^{(n)}$. Importantly, we select only one edge per entity to remove in computing $c_{ij}^{(n)}$, so that the direct causal effect of each intervention can be calculated independently of other interventions. $\ell^c(\cdot,\cdot)$ is the loss function used to compare the attention coefficients and the causal effects, which we refer to as the causal regularization loss. 


% Here, $n$ represents a single entity for which we aim to make a prediction. For a node prediction task, the entity $n$ corresponds to a node, and in a graph prediction task, $n$ corresponds to a graph. In this paper, we assume that all edges are directed and, if necessary, decompose an undirected edge into two directed edges. In each mini-batch, we perform $R$ separate rounds of causal effect calculations, each of which consists of a set of edge interventions $S^{(r)}$, $r=1,\ldots,R$. More details for the edge intervention procedure and causal effect calculations can be found in the sections below. 

% Each edge intervention in $S^{(r)}$ is represented by a set of tuples $(n,i,j)$ which denote a selected edge $(i,j)$ for an entity $n$. Note that in a node classification task, $n$ is the same as $j$ (i.e., the node with the incoming edge). The causal effect $c_{ij}^{(n)}$ scores the impact of deleting edge $(i,j)$ on predictive performance. This causal effect is compared to the edge's attention coefficient $\alpha_{ij}^{(n)}$ via the loss function $\ell^c(\cdot,\cdot)$. For models with multiple attention heads, $\alpha_{ij}^{(n)}$ is the mean attention coefficient across heads.

% We regularize the attention mechanism in accordance with the learned causal effects from edge interventions. Thus, our full objective function $\mathcal{L}$ includes the loss associated with the prediction $\mathcal{L}^p$, the loss associated with causal attention task $\mathcal{L}^{c}$, and a causal regularization strength hyperparameter $\lambda$ that mediates the contribution of the causal attention task to the objective. 

% \begin{equation}
%     \label{eqn:full_objective}
%     \mathcal{L} = \mathcal{L}^{p} + \lambda \mathcal{L}^{c}
% \end{equation}
% Here, we have $\mathcal{L}^p=\frac{1}{N}\sum_{n=1}^{N}\ell^p(\hat{y}^{(n)}, y^{(n)})$, where $N$ is the size of the training set, $\ell^p(\cdot,\cdot)$ corresponds to the loss function for the given prediction task, $\hat{y}^{(n)}$ is the prediction for entity $n$, and $y^{(n)}$ is the ground truth value for entity $n$. A detailed algorithm for \methodname is provided in \textbf{Appendix} \ref{appen:algo}.

\paragraph{Edge intervention procedure}
% Classification tasks on graphs can be understood as estimating $p( C | \mathcal{G}, \mathcal{X} ) = p(C | S) $, where $\mathcal{G}$ is the graph structure, $\mathcal{X}$ is the set of features associated with the graph $\mathcal{G}$, and $S$ is the set of predictor variables. For node classification, the node label is the target variable of interest, and the model is composed of the adjacency matrix and the method by which probabilities are computed. To construct a GNN capable of causal inference, we require a technique to generate different sub-models and experiments with different conditional dependence structures. Each sub-model will have the same GNN structure but a slightly different graph structure generated via edge-removal. Given a set of experiments $\{ \mathcal{E} \}$, with target variables $Y^e$ and predictor variables $S^e$, we say that the subset of latent variables, $S^*$, is causal for the prediction of target variable $Y$ if for all $e \in \mathcal{E}$, $S^e$ has an arbitrary distribution and $Y^e = g(S^e, \epsilon^e)$ where $g$ is our statistical model, and $\epsilon^e \sim F_{\epsilon}$ is the error distribution.

We sample a set of edges in each round $r$ such that the prediction for each entity will strictly be affected by at most one edge intervention in that round to ensure effect independence. For example, in a node classification task for a model with one GNN layer, a round of edge interventions entails removing only a single incoming edge for each node being classified. In the graph property prediction case, only one edge will be removed from each graph per round. Because a model with one GNN layer only aggregates information over a 1-hop neighborhood, the removal of each edge will only affect the model's prediction for that edge's target node. To select a set of edges in the $L$-layer GNN case, edges are sampled from the 1-hop neighborhood of each node being classified, and sampled edges that lie in more than one target nodes' $L$-hop neighborhood are removed from consideration as intervention candidates. %; this limits the computational expense of interventions. 

This edge intervention selection procedure is crucial, as it enables the causal effect of each selected intervention $c_{ij}^{(n)}$ on an entity $n$ to be calculated independently of other interventions on a graph. Moreover, by selecting only one intervention per entity within each round, we can parallelize the computation of these causal effects across all entities per round instead of iteratively evaluating just one intervention for the entire graph per entity, significantly aiding scalability. 
 
\paragraph{Calculating task-specific causal effects}
\label{subsec:methods:causaleffect}
We quantify the causal effect of an intervention at edge $(i,j)$ on entity $n$ through the use of an approximate likelihood-ratio test

% as the relative change in the prediction loss for entity $n$ upon removal of that edge.
% \begin{equation}
%     \label{eqn:causal_effect}
%     c_{ij}^{(n)} = \sigma \bigg( \bigg( \frac{\ell^p \bigl( \hat{y}_{\backslash ij}^{(n)}, y^{(n)} \bigr)} {\ell^p \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)} \bigg)^{d(n)}  -1 \bigg)
% \end{equation}

\begin{equation}
    \label{eqn:causal_effect}
    c_{ij}^{(n)} = \sigma \bigg( \bigg( \rho^{(n)}_{ij} \bigg)^{d(n)} - 1 \bigg)\;\;\;\text{where}\;\; \rho^{(n)}_{ij} = \frac{\ell^p \bigl( \hat{y}_{\backslash ij}^{(n)}, y^{(n)} \bigr)} {\ell^p \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)}
\end{equation}

% \begin{equation}
%     \label{eqn:causal_effect}
%     c_{ij}^{(n)} = \sigma \bigg( \frac{\ell^p \bigl( \hat{y}_{\backslash ij}^{(n)}, y^{(n)} \bigr)-\ell^p \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)} {\ell^p \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)} \bigg)
% \end{equation}
Here, $\hat{y}_{\backslash ij}^{(n)}$ is the prediction for entity $n$ upon removal of edge $(i,j)$. $d(n)$ represents the node degree for node classification, while it represents the number of edges in a graph for graph classification. Interventions will likely have smaller effects on higher degree nodes due to the increased likelihood of there being multiple edges that are relevant and beneficial for predictions for such nodes. In graph classification, graphs with many edges are likely to be less affected by interventions as well. Exponentiating the relative intervention effect $\rho^{(n)}_{ij}$ by $d(n)$ is intended to adjust for these biases. We have experimented both with and without raising $\rho$ to the factor of $d$, but have found empirically better results with. We do not have a rigorous explanation as to why, although we suspect the correlated nature of edges implies some amount of shrinkage is necessary. 

% $\ell^p \bigl( \hat{y}_{\backslash ij}^{(n)}, y^{(n)} \bigr) / \ell^p \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)$ so as to account for the number of edges contributing to the prediction for entity $n$. For example, in node classification tasks, predictions for a high-degree node will involve aggregating information over many neighbors, so the effect of a single edge intervention is adjusted via this $d(n)$ term to account for this specific node's high-degree context. 
The link function $\sigma : \mathbb{R} \rightarrow (0,1)$ maps its input to the support of the distribution of attention coefficients. The predictions $\hat{y}^{(n)}$ and $\hat{y}_{\backslash ij}^{(n)}$ are generated from the graph attention network being trained with \methodname. We emphasize that $\hat{y}^{(n)}$ and $\hat{y}_{\backslash ij}^{(n)}$ are both computed during the same training run, rather than in two separate runs. 

% \RS{@AW: the two y's are computed in a single run, right? pls clarify that as a line here?}
% \AW{added another sentence. is this what you mean?}
% %Furthermore, by using the prediction loss in these calculations, \methodname guides attention learning in a manner that is aware of the causal effects on the specific prediction task at hand. 

\paragraph{Scalability}
\methodname increases the computational cost of training in two ways: (i) additional evaluations of the loss function due to the causal effect calculations, and (ii) searches to ensure independent interventions. \methodname performs $\mathcal{O}(RN)$ interventions, where $R$ is the number of interventions per entity and $N$ is the number of entities in the training set. Because our edge intervention procedure ensures that the sampled interventions per round are independent, the causal effects of these interventions can be computed in parallel. In addition, if edge interventions were sampled uniformly across the graph, ensuring the independence each intervention would require a $L$-layer deep BFS that has time complexity $\mathcal{O}(b^L)$, resulting in a worst case time complexity of $\mathcal{O}(R N b^L)$, where $L$ is the depth of the GNN, and $b$ is the mean in-degree. We note that, in practice, GNNs usually have $L \leq 2$ layers since greater depth increases the computational cost and the risk of oversmoothing~\citep{gcn_oversmoothing,measuring_oversmoothing,topping2022understanding}. The contribution of this intervention overlap search step would, therefore, be minimal for most GNNs. We are also able to mitigate much of the computational cost by parallelizing these searches. Further speedups can achieved by identifying non-overlapping interventions as a preprocessing step. In summary, we have found \methodname to have a modest effect on the scalability of graph attention methods, with training runtimes that are only increased by 1.5-2 fold (\textbf{Appendix} \ref{appen:runtime_memory}).

%We have found \methodname to be highly scalable, with training runtimes that are only 1.5-2x of non-regularized attention training (Appendix \ref{appen:runtime_memory}).

% \TM{ Number of interventions scales as $O(C * |V|)$. Each intervention scales as $O(b^2l)$ due to the BFS to ensure non-overlapping interventions, where b is the branching factor and l is the number of layers. In the long run, we're unconcerned about the identification of non-overlapping interventions can be done as a preprocessing step, similar to the generation of graph samples in graph sage.}


==> iclr2023/conclusion.tex <==
We introduced \methodname, an invariance principle-based causal regularization scheme that can be applied to graph attention architectures. Unlike other invariance-based approaches \citep{graph_ood}, our focus is on scalably improving overall generalization rather than handling distribution shifts. Towards that, we introduce an efficient scheme to directly intervene on multiple edges in parallel. Applying it to both homophilic and heterophilic node-classification tasks, we found accuracy improvements and loss reductions in almost all circumstances. We performed ablation studies for a deeper understanding, and found that \methodname aligns attention with task-specific homophily and does so better than a homophily-based regularizer. A qualitative review also suggested that the attention-weight changes produced by \methodname are intuitive and interpretable. 

Understanding how, and improving what, GNNs learn remains a major open problem and is an active area of research. For instance, \cite{heterophily} have discussed the challenges that GNNs face when handling low-homophily graphs or when different tasks could be specified on the same underlying graph (e.g., predicting citation year vs. topic in obgn-arxiv). Towards this, our method provides a principled and scalable approach to align attention coefficients with the relevant task. Our work bridges two families of techniques: attention regularization and causal interventions. The synthesis of these techniques is not only a promising direction for enhancing the performance and interpretability of graph attention but also opens the door for leveraging similar techniques for general GNNs without attention as well.
%In addition, while our work is causally inspired, we do not currently formalize the causal foundations of our method. Future work may benefit from utilizing the tools of causal inference theory, like do-calculus \citep{pearl2021do_calculus}, for selecting and analyzing edge interventions. 
Lastly, while our graph pruning results are preliminary, they also suggest a promising direction for future work on scaling \methodname-based insights to web-scale graphs.

% While \methodname is not be guaranteed to uncover rigorous causal mechanisms, future research will explore extending \methodname with rigorous causal inference.

% Causality is a frequently misused term, and \methodname may not uncover rigorously causal mechanisms. However, \methodname is strongly influenced by the invariant prediction~\citep{} framework for causal inference.

==> iclr2023/iclr_directions.tex <==

ICLR requires electronic submissions, processed by
\url{https://openreview.net/}. See ICLR's website for more instructions.

If your paper is ultimately accepted, the statement {\tt
  {\textbackslash}iclrfinalcopy} should be inserted to adjust the
format to the camera ready requirements.

The format for the submissions is a variant of the NeurIPS format.
Please read carefully the instructions below, and follow them
faithfully.

\subsection{Style}

Papers to be submitted to ICLR 2023 must be prepared according to the
instructions presented here.

%% Please note that we have introduced automatic line number generation
%% into the style file for \LaTeXe. This is to help reviewers
%% refer to specific lines of the paper when they make their comments. Please do
%% NOT refer to these line numbers in your paper as they will be removed from the
%% style file for the final version of accepted papers.

Authors are required to use the ICLR \LaTeX{} style files obtainable at the
ICLR website. Please make sure you use the current files and
not previous versions. Tweaking the style files may be grounds for rejection.

\subsection{Retrieval of style files}

The style files for ICLR and other conference information are available online at:
\begin{center}
   \url{http://www.iclr.cc/}
\end{center}
The file \verb+iclr2023_conference.pdf+ contains these
instructions and illustrates the
various formatting requirements your ICLR paper must satisfy.
Submissions must be made using \LaTeX{} and the style files
\verb+iclr2023_conference.sty+ and \verb+iclr2023_conference.bst+ (to be used with \LaTeX{}2e). The file
\verb+iclr2023_conference.tex+ may be used as a ``shell'' for writing your paper. All you
have to do is replace the author, title, abstract, and text of the paper with
your own.

The formatting instructions contained in these style files are summarized in
sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.

\section{General formatting instructions}
\label{gen_inst}

The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).
Use 10~point type with a vertical spacing of 11~points. Times New Roman is the
preferred typeface throughout. Paragraphs are separated by 1/2~line space,
with no indentation.

Paper title is 17~point, in small caps and left-aligned.
All pages should start at 1~inch (6~picas) from the top of the page.

Authors' names are
set in boldface, and each name is placed above its corresponding
address. The lead author's name is to be listed first, and
the co-authors' names are set to follow. Authors sharing the
same address can be on the same line.

Please pay special attention to the instructions in section \ref{others}
regarding figures, tables, acknowledgments, and references.


There will be a strict upper limit of 9 pages for the main text of the initial submission, with unlimited additional pages for citations. 

\section{Headings: first level}
\label{headings}

First level headings are in small caps,
flush left and in point size 12. One line space before the first level
heading and 1/2~line space after the first level heading.

\subsection{Headings: second level}

Second level headings are in small caps,
flush left and in point size 10. One line space before the second level
heading and 1/2~line space after the second level heading.

\subsubsection{Headings: third level}

Third level headings are in small caps,
flush left and in point size 10. One line space before the third level
heading and 1/2~line space after the third level heading.

\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone, regardless of the formatter being used.

\subsection{Citations within the text}

Citations within the text should be based on the \texttt{natbib} package
and include the authors' last names and year (with the ``et~al.'' construct
for more than two authors). When the authors or the publication are
included in the sentence, the citation should not be in parenthesis using \verb|\citet{}| (as
in ``See \citet{Hinton06} for more information.''). Otherwise, the citation
should be in parenthesis using \verb|\citep{}| (as in ``Deep learning shows promise to make progress
towards AI~\citep{Bengio+chapter2007}.'').

The corresponding references are to be listed in alphabetical order of
authors, in the \textsc{References} section. As to the format of the
references themselves, any style is acceptable as long as it is used
consistently.

\subsection{Footnotes}

Indicate footnotes with a number\footnote{Sample of the first footnote} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches
(12~picas).\footnote{Sample of the second footnote}

\subsection{Figures}

All artwork must be neat, clean, and legible. Lines should be dark
enough for purposes of reproduction; art work should not be
hand-drawn. The figure number and caption always appear after the
figure. Place one line space before the figure caption, and one line
space after the figure. The figure caption is lower case (except for
first word and proper nouns); figures are numbered consecutively.

Make sure the figure caption does not get separated from the figure.
Leave sufficient space to avoid splitting the figure and figure caption.

You may use color figures.
However, it is best for the
figure captions and the paper body to make sense if the paper is printed
either in black/white or in color.
\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
\end{center}
\caption{Sample figure caption.}
\end{figure}

\subsection{Tables}

All tables must be centered, neat, clean and legible. Do not use hand-drawn
tables. The table number and title always appear before the table. See
Table~\ref{sample-table}.

Place one line space before the table title, one line space after the table
title, and one line space after the table. The table title must be lower case
(except for first word and proper nouns); tables are numbered consecutively.

\begin{table}[t]
\caption{Sample table title}
\label{sample-table}
\begin{center}
\begin{tabular}{ll}
\multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION}
\\ \hline \\
Dendrite         &Input terminal \\
Axon             &Output terminal \\
Soma             &Cell body (contains cell nucleus) \\
\end{tabular}
\end{center}
\end{table}

\section{Default Notation}

In an attempt to encourage standardized notation, we have included the
notation file from the textbook, \textit{Deep Learning}
\cite{goodfellow2016deep} available at
\url{https://github.com/goodfeli/dlbook_notation/}.  Use of this style
is not required and can be disabled by commenting out
\texttt{math\_commands.tex}.


\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}



\section{Final instructions}
Do not change any aspects of the formatting parameters in the style files.
In particular, do not modify the width or length of the rectangle the text
should fit into, and do not change font sizes (except perhaps in the
\textsc{References} section; see below). Please note that pages should be
numbered.

\section{Preparing PostScript or PDF files}

Please prepare PostScript or PDF files with paper size ``US Letter'', and
not, for example, ``A4''. The -t
letter option on dvips will produce US Letter files.

Consider directly generating PDF files using \verb+pdflatex+
(especially if you are a MiKTeX user).
PDF figures must be substituted for EPS figures, however.

Otherwise, please generate your PostScript and PDF files with the following commands:
\begin{verbatim}
dvips mypaper.dvi -t letter -Ppdf -G0 -o mypaper.ps
ps2pdf mypaper.ps mypaper.pdf
\end{verbatim}

\subsection{Margins in LaTeX}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+
from the graphicx package. Always specify the figure width as a multiple of
the line width as in the example below using .eps graphics
\begin{verbatim}
   \usepackage[dvips]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.eps}
\end{verbatim}
or % Apr 2009 addition
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
for .pdf graphics.
See section~4.4 in the graphics bundle documentation (\url{http://www.ctan.org/tex-archive/macros/latex/required/graphics/grfguide.ps})

A number of width problems arise when LaTeX cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command.

\subsubsection*{Author Contributions}
If you'd like to, you may include  a section for author contributions as is done
in many journals. This is optional and at the discretion of the authors.

\subsubsection*{Acknowledgments}
Use unnumbered third level headings for the acknowledgments. All
acknowledgments, including those to funding agencies, go at the end of the paper.

==> iclr2023/intro.tex <==
Graphs encode rich relational information that can be leveraged in learning tasks across a wide variety of domains. Graph neural networks (GNNs) can learn powerful node, edge or graph-level representations by aggregating a node's representations with that of its neighbors. 
%Graph neural networks (GNNs) have demonstrated considerable promise in recent years by using these graph relations to supplement node representations with information from node neighbors.
%However, t
The specifics of a GNN's neighborhood aggregation scheme are critical to its effectiveness on a prediction task.
For instance, graph convolutional networks (GCNs) aggregate information via a simple averaging or max-pooling of neighbor features. 
%\citep{gcn_kipf_welling,graphsage}.
% While GCNs scales well, they are also indiscriminate. 
GCNs are prone to suffer in many real-world scenarios where uninformative or noisy connections exist between nodes \citep{gcn_kipf_welling,graphsage}. 
% GCNs may also over-smooth, with nodes in a graph taking on indistinguishable representations due to the indiscriminate aggregation operation \citep{gcn_oversmoothing,measuring_oversmoothing,topping2022understanding}. 
Graph-based attention mechanisms combat these issues by quantifying the relevance of node-neighbor relations and softly selecting neighbors in the aggregation step accordingly \citep{gat,gatv2,transformerconv}. This process of attending to select neighbors has contributed to significant performance gains for GNNs across a variety of tasks \citep{gnn_review, 2022message}. Similar to the use of attention in natural language processing and computer vision, attention in graph settings also enables the interpretability of model predictions via the examination of attention coefficients \citep{attn_interpret}. 

% Paramount to the effectiveness of attention mechanisms in GNNs is their ability to discern the specific graph connectivity patterns that underlie accurate, generalizable predictions. %As graph training data often contains noisy features and/or connections,
However, graph attention mechanisms can be prone to spurious edges and correlations that mislead them in how they attend to node neighbors, which manifests as a failure to generalize to unseen data \citep{attn_generalization}. One approach to improve GNNs' generalizability is to regularize attention coefficients in order to make them more robust to spurious correlations/connections in the training data. Previous work has focused on $L_0$ regularization of attention coefficients to enforce sparsity \citep{ye2021sparse} or has co-optimized a link prediction task using attention \citep{kim2021how}. Since these regularization strategies are formulated independently of the primary prediction task, they align the attention mechanism with some intrinsic property of the input graph without regard for the training objective. 
%Some of the previous work is also specific to the kind of graph attention mechanism chosen. 
% the inability of attention mechanisms to select the appropriate node neighbors also suggests an inability to determine the graph connections that causally contribute to a particular prediction.

% We take a different approach. We begin our study with the question: ``What is the importance of a specific edge to the prediction task?''
We take a different approach and consider the question: ``What is the importance of a specific edge to the prediction task?'' Our answer comes from the perspective of regularization: we introduce \methodname, a causal attention regularization framework that is broadly suitable for graph attention network architectures (\textbf{Figure}~\ref{fig:figure_1}). Intuitively, an edge in the input graph is important to a prediction task if removing it leads to substantial degradation in the prediction performance of the GNN. The key conceptual advance of this work is to scalably leverage active interventions on node neighborhoods (i.e., deletion of specific edges) to align graph attention training with the causal impact of these interventions on task performance. Theoretically, our approach is motivated by the invariant prediction framework for causal inference ~\citep{RePEc:bla:jorssb:v:78:y:2016:i:5:p:947-1012,graph_ood}. While some efforts have previously been made to infuse notions of causality into GNNs, these causal approaches have been largely limited to using causal effects from pre-trained models as features for a separate model \citep{trust_neigh,attn_generalization} or decoupling causal from non-causal effects \citep{causal_attn_graph}. 
% Causality is a frequently misused term, and \methodname may not uncover rigorously causal mechanisms. Nonetheless, 
%\methodname is motivated by the invariant prediction framework for causal inference ~\citep{RePEc:bla:jorssb:v:78:y:2016:i:5:p:947-1012,graph_ood}.

% Our work builds on previous findings \citep{attn_generalization} that an explicit focus on improving attention coefficients can pay rich dividends.
We apply \methodname on three graph attention architectures across eight node classification tasks, finding that it consistently improves test loss and accuracy. \methodname is able to fine-tune graph attention by improving its alignment with task-specific homophily. Correspondingly, we found that as graph heterophily increases, the margin of \methodname's outperformance widens. In contrast, a non-causal approach that directly regularizes with respect to label similarity generalizes less well. On the ogbn-arxiv network, we investigate the citations up/down-weighted by \methodname and found them to broadly group into three intuitive themes. Our causal approach can thus enhance the interpretability of attention coefficients, and we provide a qualitative analysis of this improved interpretability. We also present preliminary results demonstrating the applicability of \methodname to graph pruning tasks. 
%Lastly, by applying it on sample sub-networks for a large social media-sized network, \methodname can enable us to learn the attention coefficients that would generalize to the broader network. 
Due to the size of industrially relevant graphs, it is common to use GCNs or sampling-based approaches on them. There, using attention coefficients learned by \methodname on sampled subnetworks may guide graph rewiring of the full network to improve the results obtained with convolutional techniques. %while retaining scalability.

%Understanding how, and improving what, GNNs learn remains a major open problem and an active area of research. Towards this, our work bridges two families of techniques (attention regularization and causal interventions) which we believe could be a promising direction of future research. 

% performance gains
% intepretability
% issues: spurious correlations (training data size?, training data network connectivity), limitations of interpretability
% sensitivity to initialization

% themes:
% graph attention
% determining relevant neighbors
% causal modeling: interventions ("causal view of robustness...", "matching learned causal effects...")
% causal attention
% causal regularization: KDD paper + ICML paper (causal effects domain priors)
% 

==> iclr2023/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> iclr2023/related_work.tex <==
The performance gains associated with graph attention networks have led to a number of efforts to enhance and better understand graph attention mechanisms \citep{gat_survey}. One category of methods aims to improve the expressive power of graph attention mechanisms by supplementing a given prediction objective with a supervised attention mechanism~\citep{trust_neigh}, or a self-supervised connectivity prediction approach~\citep{kim2021how}. A related set of methods leverage signals from interventions on graphs from a causal perspective to aid in training GNNs. One class of techniques performs interventions on nodes~\citep{attn_generalization, trust_neigh}. CAL ~\citep{causal_attn_graph}, a method designed for graph property prediction tasks, performs abstract interventions on representations of entire graphs instead of specific nodes or edges to identify the causally attended subgraph for a given task. Specifically, it uses these interventions to achieve robustness rather than directly leveraging information about the effect of these interventions on model predictions. 
% Meanwhile, other methods such as CAL~\citep{causal_attn_graph}  or CFLP~\citep{2106.02172} aim to separate causal and non-causal effects with auxiliary tasks, with CAL and CFLP designed specifically for graph property prediction and link prediction tasks, respectively.

Our intervention-oriented framework can also be understood as a graph structure perturbation method. Perturbation methods can be broadly split into three different categories: graph data augmentation~\citep{2202.08871}, structural graph rewiring~\citep{DBLP:conf/iclr/RongHXH20}, and geometric graph rewiring~\citep{topping2022understanding}. Inspired by the success of data augmentation approaches in computer vision, graph data augmentation methods seek to generate new training samples through different augmentation techniques. One of the earliest methods is DropEdge~\citep{DBLP:conf/iclr/RongHXH20} reduces overfitting by randomly selecting edges from a uniform distribution to delete. Other methods build on DropEdge and select edges according to additional constraints including geometrical invariants~\citep{gao2021training}, target probability distributions~\citep{NEURIPS2021_9e7ba617}, and information criteria~\citep{suresh2021adversarial}. EERM, a powerful invariance-based approach by \cite{graph_ood} takes a graph-editing approach to learn GNNs that are robust to distribution shifts in the data. % In contrast to \methodname, EERM requires learning a graph generation policy for sampling subgraphs.
Structural graph rewiring instead seeks to enforce structural priors such as sparsity or homophily during the graph alteration phase. Examples of these rewiring priors include fairness~\citep{2201.08549, 9645324}, temporal structure~\citep{NEURIPS2021_0b0b0994}, predicted homophily~\citep{measuring_oversmoothing}, sparsity\citep{10.1145/3394486.3403049, pmlr-v119-zheng20d}, or information transfer efficiency~\citep{10.5555/3454287.3455484}. Geometric approaches, instead, choose to view the graph as a discrete geometry and alter the connectivity according to the balanced Forman curvature~\citep{topping2022understanding}, the stochastic discrete Ricci flows~\citep{2207.08026}, commute times~\citep{2206.07369}, or algebraic connectivity\citep{2206.07369}. All of these approaches are designed either for use either in self-supervised learning or in a task-agnostic fashion, and consider the input graph independently of the task at hand.

To summarize, \methodname introduces a combination of advances not previously reported: applicability to diverse attention architectures; task-based supervised regularization (rather than task-agnostic or self-supervised regularization) that leads to improved generalization; and a causal approach that scalably and directly relates an edge's importance to its attention coefficient, enhancing interpretability. 

% A key innovation of our design is an edge selection scheme for performing multiple interventions in parallel, ensuring scalability. 

% Unlike these approaches, \methodname takes a more direct and interpretable approach to graph perturbation, and applies this to node classification and graph property prediction. \methodname achieves this by supervising the attention coefficients through active interventions on sampled edges during training. The active intervention framework directly enables the measurement of the individual treatment effect, so that we can perform task-specific casual regularization of the attention coefficients for arbitrary attention-based models. While \methodname can be understood through the lens of graph sparsification, \methodname does not seek to explicitly alter the edge connectivity through structural perturbations that may be deleterious to generalization. Moreover, \methodname alters the underlying geometry in \textit{task specific} ways.

% Unlike these approaches, \methodname takes a more direct and interpretable approach to graph perturbation, and applies this to node classification and graph property prediction. \methodname achieves this by supervising the attention coefficients by active interventions on sampled edges during training. The active intervention framework directly enables the measurement of the individual treatment effect, so that we can perform task-specific casual regularization of the attention coefficients for arbitrary attention-based models.

% The performance gains associated with graph attention networks have led to a number of efforts to enhance and better understand graph attention mechanisms \citep{gat_survey}. One category of methods aims to improve the expressive power of graph attention mechanisms by supplementing a given prediction objective with one or more tasks. \cite{attn_review} found that adding the supervised training of attention as an auxiliary task dramatically improved classification accuracy and that classification accuracy depended exponentially on attention correctness in their experiments. Such settings with ground truth attention are rare, though, so alternative tasks have been proposed to learn better attention coefficients. For example, SuperGAT adds an edge self-supervision task that is task-agnostic, using the connectivity patterns of existing edges in a graph to inform the assignment of attention coefficients to edges \citep{kim2021how}.

% A related set of methods leverage signals from interventions on graphs to aid in training GNNs. \cite{attn_review} devised an auxiliary weakly-supervised attention learning task based on changes in a pre-trained GCN's predictions that stem from node-level interventions. Causal GCN Inference (CGI) uses the outcomes of node-level interventions on a pre-trained GCN as well but as features in a classifier rather than as a means of informing attention \citep{trust_neigh}. Meanwhile, the Causal Attention Learning (CAL) strategy \citep{causal_attn_graph} aims to decouple causal and non-causal effects by introducing an additional task that encourages robustness to abstract interventions on graph representations rather than specific nodes or edges. Unlike these approaches, \methodname takes a more direct and interpretable approach, supervising the attention coefficients by active interventions on sampled edges during training and measuring the causal effect on the prediction task.

% Perhaps the method most comparable to ours is CFLP~\citep{2106.02172}, which treats an edge's existence as an individual treatment effect and constructs a causal model to predict the average treatment effect directly. However, it differs from \methodname substantially, both in application and approach. \methodname uses an estimate of the individual treatment effect to regularize the attention coefficients for arbitrary attention-based models, rather than alter the data distribution that is used for training. Additionally, CFLP is aimed at link-prediction which requires positional, rather than structural, representations~\citep{Srinivasan2020On}, whereas our work is aimed at node and graph classification for which structural representations are sufficient.

% % Graph data augmentation
% Inspired by the success of data augmentation approaches in computer vision, graph perturbations have also found their use in graph data augmentation~\cite{2202.08871}. In DropEdge~\citep{DBLP:conf/iclr/RongHXH20}, edges are randomly deleted in subgraph samples to reduce overfitting. Dropping edges indiscriminately can result in pathological examples that limit generalization. 
% TADropEdge~\citep{gao2021training} seeks to limit this effect by drawing edges according to topological invariants. MH-Aug~\cite{NEURIPS2021_9e7ba617} instead uses Metropolis-Hastings to generate new training examples through a set of graph mutation rules. 
% AD-GCL~\cite{suresh2021adversarial} constructs a contrastive learning framework to drop edges by minimizing the information lost by dropping each edge. All of these approaches are designed either for self-supervised learning (e.g., AD-GCL) or in a task-agnostic fashion (e.g., DropEdge), distinguishing them from \methodname. % This is done to increase generalization by reducing the number of repeated structural features that are learned.

% % Graph Rewiring

% Many methods have explored graph rewiring as a way to improve inferential accuracy, predictive performance, or improve generalization. GDC~\cite{10.5555/3454287.3455484} seeks to improve information diffusion while reducing noise through densification and then sparsification steps. In an attempt to debias learned representations, FairAug~\cite{2201.08549} and FairDrop~\cite{9645324} remove edges according to a defined fairness metric. MeTa~\cite{NEURIPS2021_0b0b0994} generates new subgraphs through temporal edge-sampling, and then learns to pass messages between temporally distinct subgraphs. This method has clear causal intuition, but without the interventional semantic of \methodname. The AdaEdge method~\cite{measuring_oversmoothing}, supervised edge-perturbation is performed through multiple full-training runs where the graph is rewired to optimize for predicted-homophily.

% % Graph Geometry
% \RS{@TM: ok if we kill/shrink this paragraph if we are still running short on space?}
% Another related set of methods have observed that intrinsic properties of the graph, such as sparsity or curvature, can be leveraged to rewire the graph to increase task generalization. Pro-GNN\cite{10.1145/3394486.3403049} co-learns a GNN and a sparsified graph structure to build methods that are robust to external perturbation. Sparsification is learned through structural optimization of the adjacency matrix. Similar to \methodname, NeuralSparse~\cite{pmlr-v119-zheng20d} seeks to sparsify by removing task-irrelevant edges. NeuralSparse, however, chooses to do so by learning a generative distribution over graph perturbations. Moving beyond sparsification, work based on the balanced Forman curvature~\cite{topping2022understanding} rewires the graph to improve information flow through the graph, which yielded state of the art performance on a variety of benchmarks. This idea is pushed further in by Bober \textit{et al.}~\cite{2207.08026} where they view a graph as a discrete geometry and use tools for discrete differential geometry. Alternatively, DiffWire~\cite{2206.07369} presents two different GCN layers: CT and GAP that are fully differentiable and optimize graph connectivity according to commute times or the algebraic connectivity. While \methodname can be understood through the lens of graph sparsification, \methodname does not seek to explicitly alter the edge connectivity through structural perturbations that may be deleterious to generalization. Moreover, \methodname alters the underlying geometry in \textit{task specific} ways.


% \RS{@TM/AW: new paragraph, pls check} To summarize, \methodname introduces a combination of advances not previously reported: applicability to diverse attention architectures; task-based supervised regularization (rather than task-agnostic or self-supervised regularization) leading to improved generalization; and a causal approach that directly relates an edge's importance to its attention coefficient, enhancing interpretability. A key innovation of our design is an edge selection scheme for performing multiple interventions in parallel, ensuring scalability. 


% edge-level interventions
% during training (accounts for ability of GAT to adjust weights of neighbors vs. indiscriminate pooling as in GCNs)

% \noindent \textbf{Attention in GNNs:}

% \noindent \textbf{Graph Attention Regularization:} 

% self-supervised learning: friendly neighbors
% weakly supervised learning: graph attention generalization (attention over nodes, intervention w/ weak supervision)
% causal: granger-causal attentive mixtures of experts, trust neighbors?
% l0 regularization: ye2021 - graph rewiring too

% \cite{attn_review} found that, in cases where ground-truth attention is available, supervised training of attention contributed to improved generalization performance of models to unseen and noisy graph inputs. 

% Hence, efforts have been made to design graph attention through supplementing learning tasks with self-supervision \cite{friendly_neigh} or by .

% using causal effects from pre-trained models as features for a separate model \citep{trust_neigh} or decoupling causal from non-causal effects \citep{causal_attn_graph}. To our knowledge, no efforts have . 

% graph attention
% graph causal modeling
% causal explanations
% causal regularization (graph domain priors, CAL) + supervised attention

==> iclr2023/reproducibility.tex <==
To ensure the reproducibility of the results in this paper, we have included the source code for our method as supplementary materials. The datasets used in this paper are all publicly available, and we also use the publicly available train/validation/test splits for these datasets. We provide details on these datasets in the Appendix and have provided references to them in both the main text and the Appendix. In addition, we have provided detailed descriptions of the experimental setup, model training schemes, model architecture design choices, and hyperparameter choices in the ``Experimental Setup'' section as well as in Appendix \ref{appen:arch_hyper}.


==> iclr2023/results.tex <==
\subsection{Experimental Setup}
We assessed the effectiveness of \methodname by comparing the performance of a diverse range of models trained with and without \methodname on 8 node classification datasets.
% (see additional applications in \S \ref{subsec:methods:investigation}). 
Specifically, we aimed to assess the consistency of \methodname's outperformance 
over matching baseline models across various graph attention mechanism and hyperparameter choices. Accordingly, we evaluated numerous combinations of such configurations (48 settings for each dataset and graph attention mechanism), rather than testing only a limited set of optimized hyperparameter configurations. 
% to assess the effect of using \methodname on each configuration. 
The configurable model design and hyperparameter choices that we evaluated include the graph attention mechanism (GAT, GATv2, or Graph Transformer), the number of graph attention layers $L=\{1,2\}$, the number of attention heads $K=\{1,3,5\}$, the number of hidden dimensions $F'=\{10,25,100,200\}$, and the regularization strength $\lambda=\{0.1,0.5,1,5\}$. See \textbf{Appendix} \ref{appen:arch_hyper} for details on the network architecture, hyperparameters, and training configurations. 

\subsection{Node Classification}
\noindent \textbf{Datasets and evaluation:} We used a total of 8 real-world node classification datasets of varying sizes and degrees of homophily: Cora, CiteSeer, PubMed, ogbn-arxiv, Chameleon, Squirrel, Cornell and Wisconsin. Each model was evaluated according to its accuracy on a held-out test set. We also evaluated the test cross-entropy loss, as it accounts for the full distribution of per-class predictions rather than just the highest-valued prediction considered in accuracy calculations. See \textbf{Appendix} \ref{appen:node_class_datasets} for details on dataset statistics, splits, and references. % Runtimes for training models with \methodname ranged from roughly 2 seconds to 5 minutes on the evaluated datasets, with \methodname's runtime only 1.5-2 times that of standard training on average (see \textbf{Appendix} \ref{appen:runtime_memory} for details). 

\noindent \textbf{Generalization performance:} We compared both the test accuracy and the test loss of each model when trained with and without \methodname. Across all model architecture and hyperparameter choices for a dataset, we applied the one-tailed paired Wilcoxon signed-rank test to quantify the overall outperformance of models trained with \methodname against models trained without it. \methodname resulted in higher test accuracy in 7 of the 8 node classification datasets and a lower test loss in all 8 datasets (\textbf{Figure} \ref{fig:figure_2}, $p < 0.05$). We report the relative performance when averaging over all hyperparameter choices in \textbf{Table}~\ref{table:loss_results} (test loss), \textbf{Table}~\ref{table:acc_results} (test accuracy, in \textbf{Appendix} \ref{appen:node_class_acc}), and \textbf{Appendix} \ref{appen:percent_change_acc_loss}. We also observed that even small values of $R$ were effective (\textbf{Appendix} \ref{appen:num_interventions}). We believe that this is due to there being an adequate number of causal-effect examples for regularization, as even in the minimum $R=1$ case, we have roughly one causal-effect example per training example. 

We also compared \methodname with \cite{causal_attn_graph}'s CAL, a method for graph property prediction that relies on an alternative formulation of causal attention with interventions on implicit representations. We adapted CAL for node classification by removing its final pooling layer. \methodname-trained models substantially outperformed CAL (\textbf{Appendix} \ref{appen:compare_cal}), suggesting that \methodname's direct edge-intervention approach results in better generalization. Taken together, these results highlight the consistency of performance gains achieved with \methodname and its broad applicability across across graph attention architectures and hyperparameters. 
% Furthermore, in comparing \methodname with a modified version of CAL, a method that relies on an alternative formulation of causal attention for graph property predictions ~\citep{2106.02172}, we observed that \methodname-trained models drastically outperformed CAL as well (\textbf{Appendix} \ref{appen:compare_cal}).

% \AW{do we want to condense the accuracy and loss tables into one table with just the mean values of each? we can then show the full tables with the standard deviations in the appendix.}

\begin{table}[ht]
\caption{Test loss on 8 node classification datasets}
\label{table:loss_results}
\centering
\small
\renewcommand{\arraystretch}{1.5}
\begin{center}
\resizebox{14cm}{!}{%
\begin{tabular}{l c c c c c c c c }
    & \textbf{Cora} & \textbf{CiteSeer} & \textbf{PubMed} & \textbf{ogbn-arxiv} & \textbf{Chameleon} & \textbf{Squirrel} & \textbf{Cornell} & \textbf{Wisconsin} \\
    \hline
    GAT &  2.33 $\pm$ 0.75 & 3.68 $\pm$ 2.64 & 1.05 $\pm$ 0.24 & 1.49 $\pm$ 0.02 & 1.29 $\pm$ 0.03 & 1.48 $\pm$ 0.02 & 1.19 $\pm$ 0.23 & 0.88 $\pm$ 0.11  \\
    % \hline
    GAT + \methodname & \textbf{1.82 $\pm$ 0.77} & \textbf{3.06 $\pm$ 2.34} & \textbf{0.89 $\pm$ 0.18} & 1.49 $\pm$ 0.02 & \textbf{1.26 $\pm$ 0.03} & \textbf{1.47 $\pm$ 0.02} & \textbf{1.14 $\pm$ 0.17} & \textbf{0.84 $\pm$ 0.13} \\
    \hline
    GATv2 &  2.26 $\pm$ 0.54 & 3.08 $\pm$ 1.06 & 1.07 $\pm$ 0.29 & 1.48 $\pm$ 0.02 & 1.28 $\pm$ 0.03 & 1.48 $\pm$ 0.02 & 1.09 $\pm$ 0.11 & 0.88 $\pm$ 0.15 \\
    GATv2 + \methodname & \textbf{1.63 $\pm$ 0.59} & \textbf{3.04 $\pm$ 2.07} & \textbf{0.90 $\pm$ 0.17} & \textbf{1.47 $\pm$ 0.03} & \textbf{1.24 $\pm$ 0.03} & \textbf{1.46 $\pm$ 0.02} & \textbf{1.04 $\pm$ 0.10} & \textbf{0.81 $\pm$ 0.09} \\
    \hline
    Transformer & 3.43 $\pm$ 1.61 & 9.78 $\pm$ 8.27 & 1.79 $\pm$ 0.88 & 1.50 $\pm$ 0.03 & 1.38 $\pm$ 0.06 & 1.50 $\pm$ 0.02 & 1.22 $\pm$ 0.25 & 1.03 $\pm$ 0.28 \\
    Transf.\ + \methodname & \textbf{1.71 $\pm$ 0.50} & \textbf{3.92 $\pm$ 2.25} & \textbf{1.60 $\pm$ 0.59} & 1.50 $\pm$ 0.03 & \textbf{1.33 $\pm$ 0.04} & \textbf{1.48 $\pm$ 0.03} & \textbf{1.07 $\pm$ 0.12} & \textbf{0.86 $\pm$ 0.13} \\ 
    \hline
\end{tabular}}
\end{center}
\end{table}
\vspace*{-0.5cm}

\subsection{Model Investigation and Ablation Studies}
\label{subsec:methods:investigation}
%%\RS{points to make: a) \methodname accentuates correlation with homophily, more so for heterophilic networks [label agreement result?]; b) effect of hyperparameter $\lambda$ (b.1: violin plot; b.2: dialed-up/down cora homophily)  c) an ablation where label propagation was directly used to regularize also helps but not as much as \methodname, esp for heterophilic networks; \sout{d) random edge ablation?}}

\paragraph{Impact of regularization strength} 
We explored 4 settings of $\lambda$: $\{0.1, 0.5, 1, 5\}$. For 6 of the 8 node classification datasets, \methodname models trained with the higher causal regularization strengths ($\lambda=\{1,\,5\}$) demonstrated significantly larger reductions in test loss ($p < 0.05$, one-tailed Welch's $t$-test) compared to those trained with weaker regularization ($\lambda=\{0.1,\,0.5\}$). Notably, all four of the datasets with lower homophily (Chamelon, Squirrel, Cornell and Wisconsin) displayed significantly larger reductions in test loss with the higher regularization strengths, suggesting that stronger regularization may contribute to improved generalization in such settings (\textbf{Appendix} \ref{appen:compare_loss_lambda}).

%\noindent \textbf{Selecting $\lambda$ for \methodname in multi-layer GNNs:} (still include?)

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.995 \linewidth ]{fig2_causal_comparison_node.pdf}
    \caption{Test accuracy and negative loss on 8 node classification datasets. Each point corresponds to a comparison between a baseline model trained without \methodname and an identical model trained with \methodname. The point size represents the magnitude of the $\lambda$ value chosen for the \methodname-trained model. $p$-values are computed from one-tailed paired Wilcoxon signed-rank tests evaluating the improvement of \methodname-trained models over the baseline models.}
    \label{fig:figure_2}
\end{figure}



\paragraph{Connection to spurious correlations and homophily}

Graph attention networks that are prone to spurious correlations mistakenly attend to parts of the graph that are irrelevant to their prediction task. To evaluate if \methodname reduces the impact of such spurious correlations, we assessed if models trained with \methodname more effectively prioritized relevant edges. For node classification tasks, the relevant neighbors to a given node are expected to be those that share the same label as that node. We, therefore, used the label agreement between nodes connected by an edge as a proxy for the edge's ground-truth relevance. We assigned a reference attention coefficient $e_{ij}$ to an edge based on label agreement in the target node's neighborhood: $e_{ij} = \hat{e}_{ij}/\sum_{k\in N_j} \hat{e}_{kj}$ \citep{kim2021how}. Here, $\hat{e}_{ij} = 1$ if nodes $i$ and $j$ have the same label and $\hat{e}_{ij} = 0$ otherwise. $N_j$ denotes the in-neighbors of node $j$. We then calculated the KL divergence of an edge's attention coefficient $\alpha_{i,j}$ from its reference attention coefficient $e_{ij}$ and summarize a model's ability to identify relevant edges as the mean of these KL divergence values across the edges in the held-out test set. 

We compared these mean KL divergences between baseline models trained without \methodname and models trained with \methodname across the same broad range of model architecture and hyperparameter choices described above. We found that \methodname-trained models consistently yielded lower mean KL divergence values than models trained without \methodname  for 6 of 8 node classification datasets (\textbf{Figure }\ref{fig:figure_3},$p < 0.05$, one-tailed paired Wilcoxon signed-rank test). Notably, this enhanced prioritization of relevant edges was achieved without explicitly optimizing label agreement during training and is an inherent manifestation of aligning attention with the node classification tasks' causal effects.

% The improvement in AP for \methodname-trained models was particularly pronounced for the Chameleon and Squirrel datasets, which are characterized by lower homophily, while the higher homophily datasets (Cora, CiteSeer, PubMed) were not associated with such gains (Appendix \ref{appen:label_agreement_homophily}). 

Low homophily graphs are associated with greater proportions of task-irrelevant edges and thus may introduce more spurious correlations~\citep{heterophily}. We reasoned that \methodname's relative effectiveness should be greater in such settings. We assessed this by evaluating \methodname on 33 synthetic Cora datasets with varying levels of homophily \citep{homophily_syn_cora}. We observed that \methodname-trained models outperformed baseline models most substantially in low homophily settings, with performance gains generally increasing with decreasing homophily (\textbf{Appendix} \ref{appen:syn_cora}). Altogether, these results demonstrate that \methodname not only more accurately prioritizes the edges that are most relevant to the desired task but also highlights its utility in low homophily settings most prone to spurious correlations. 
%more effective greater sensitivity to spurious correlations, \methodname's effectiveness in such settings provides further evidence for its ability to enhance graph attention
% In addition, this result highlights the applicability of \methodname for low homophily graphs, as graph attention is essential in such settings due to the relative dissimilarity of neighboring nodes in these graphs. 

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.7 \linewidth ]{fig3_label_agreement.pdf}
    \caption{Coherence between attention coefficients and label agreement for \methodname-trained models, compared to baseline. Lower KL divergence implies greater coherence. Point colors and sizes have the same meaning as in \textbf{Figure} \ref{fig:figure_2}. $p$-values are computed from one-tailed paired Wilcoxon signed-rank tests evaluating the improvement of \methodname-trained models over the baseline models.}
    \label{fig:figure_3}
\end{figure}

\paragraph{Comparison to homophily-based regularization} 
%We also evaluated the degree to which aligning attention mechanisms with their causal effects contributed to this improved generalization performance. 
We next assessed if the performance gains by our causal approach could be replicated by a non-causal approach that systematically aligns attention coefficients with a generic measure of homophily. To do so, we performed an ablation study in which we replace the causal effects $c_{ij}^{(n)}$ computed from the network being trained (\textbf{Equation} \ref{eqn:causal_effect}) with an alternative score derived from a homophily-based classification scheme. Briefly, this scheme entails assigning a prediction for each node based on the counts of its neighbors' labels (see \textbf{Appendix} \ref{appen:neighbor_vote} for details). By regularizing attention with respect to this homophily-based classification scheme, the attention mechanism for a network will be guided no longer by causal effects associated with the network but rather this separate measure of homophily.

% Separately, we also we simply draw each causal effect $c_{i,j}^{(n)}$ from a uniform distribution on the interval $[0,1)$ 

We compared \methodname-trained models with those trained with homophily-based regularization by evaluating the consistency of their test loss improvements relative to the baseline models without regularization. We used the one-tailed paired Wilcoxon signed-rank test to evaluate the significance of the regularized models' test loss improvements across the set of model architecture and hyperparameter choices, focusing on models trained with the higher $\lambda \in \{1,5\}$ regularization strengths. Models trained when regularizing attention coefficients with the homophily-based scheme underperformed those trained with \methodname in 7 of the 8 datasets (\textbf{Table} \ref{table:ablation}). Interestingly, the homophily-based -based regularization showed an overall gain in performance relative to the baseline models (i.e., those trained without any regularization), suggesting that even non-specific regularization can be somewhat useful for training attention. Overall, these results demonstrate the effectiveness of using \methodname to improve generalization performance for many node classification tasks.

\begin{table}[h!]
\smallskip
\centering
% \caption{Generalization performance of \methodname-trained models with ablations compared to baseline \\($-\log_{10}(p)$, one-tailed paired Wilcoxon signed-rank test)}
\caption{Ablation study comparing improvements in performance using \methodname regularization and homophily-based regularization ($-\log_{10}(p)$, one-tailed paired Wilcoxon signed-rank test)}
\label{table:ablation}
\renewcommand{\arraystretch}{1.2}
\resizebox{14cm}{!}{%

\begin{tabular}{ r  c  c  c  c  c  c  c  c } 
    % \multirow{3}{*}{\bf Method}  &\multicolumn{2}{c}{\bf Cora} &\multicolumn{2}{c}{\bf CiteSeer} &\multicolumn{2}{c}{\bf PubMed} &\multicolumn{2}{c}{\bf orgn-arxiv} &\multicolumn{2}{c}{\bf Chameleon} &\multicolumn{2}{c}{\bf Squirrel} \\ 
    & \textbf{Cora} & \textbf{CiteSeer} & \textbf{PubMed} & \textbf{ogbn-arxiv} & \textbf{Chameleon} & \textbf{Squirrel} & \textbf{Cornell} & \textbf{Wisconsin} \\
    % \cmidrule(lr){2-3}\cmidrule(lr){3-4}\cmidrule(lr){5-6}
    \hline
    \methodname & \textbf{12.36} & \textbf{5.92} & \textbf{10.51} & \textbf{1.81} & \textbf{12.77} & 9.72 & \textbf{6.72} & \textbf{9.34} \\
    % \hline
    Homophily &  10.04 & 5.59 & 7.30 & 0.53 & 12.34 & \textbf{10.97} & 4.15 & 8.20 \\
    \hline
    % \methodname & \textbf{8.99} & \textbf{4.34} & \textbf{7.81} & \textbf{0.655} & \textbf{10.84} & 9.56 & \textbf{3.84} & \textbf{6.24} \\
    % % \hline
    % Neighbor Voting & 8.89 & 3.62 & 4.78 & 0.233 & 9.20 & 10.84 & 2.28 & 5.30 \\
    % \hline
    % Random & X & X & X & X & X & X \\
\end{tabular}}
\end{table}
\vspace*{-0.2cm}

% \begin{table}[h!]
% \centering
% \caption{\methodname-trained graph attention mechanisms attend to homophilous edges in node classification}
% \label{table:attn_homophily}
% \renewcommand{\arraystretch}{2.5}
% \begin{tabular}{ c  c  c  c  c  c  c } 
%     & Cora & CiteSeer & PubMed & ogbn-arxiv & Chameleon & Squirrel \\
%     % \cmidrule(lr){2-3}\cmidrule(lr){3-4}\cmidrule(lr){5-6}
%     \hline
%     Baseline & 0.81 \pm 0.01 & 0.76 \pm 0.01 & 0.81 \pm 0.01 & 0.70 \pm 0.01 &  \\
%     \hline
%     Baseline & 0.81 \pm 0.01 & 0.76 \pm 0.01 & 0.81 \pm 0.01 & 0.70 \pm 0.01 & 
% \end{tabular}
% \end{table}


% \subsubsection{Cheeger Constant}
% \TM{Do we have results here? Because the graphs are all disconnected, this might be difficult to interpret.}
% Next, we turn our attention to a series of experiments intended to understand the topological changes that our graph undergoes due to our causal regularization method. 

% Because our method prunes edges, we are specifically interested in understanding whether our method is introducing bottlenecks that would make us more susceptible to over-squashing. To answer this question, we compute Cheeger constant as a function of regularization strength for the Cora dataset.

% Furthermore, we computed the curvature of the original graph, pruned graph, and removed edges; and present the kernel density estimates below.

% \subsubsection{Graph Diffusion Distance}
% \TM{Do we have results here? It feels like a nice to have but probably a P1/P2 priority.}
% Next, we are interested to understand whether our proposed method is simply removing edges that are ``topologically noisy''. To answer this question, we have computed the graph diffusion distance defined as

% \begin{equation}
%  d^{(u,v)}_{GDD}(A_1, A_2) = \sqrt{ \argmax_{t} \left | \left |  e^{-t L}  - e^{-t L\backslash ({u,v}) } \right | \right |^2_F},
% \end{equation}

% where $L$ is the graph Laplacian, and $L\backslash ({u,v})$ is the graph Laplacian with the edge from $u$ to $v$ deleted. We use this metric because it provides a global measure of graph diffusion, which is intimately connected to message passing.

\paragraph{Additional applications}
To explore the utility of \methodname as a general-purpose framework, we employed \methodname for graph pruning. 
% For graph property prediction, we evaluated \methodname on ogbg-molbace, a dataset for binary classification, and ogbg-molfreesolv, which features a regression task \citep{ogb}. We trained models with \methodname across a broad range of graph attention mechanisms and hyperparameter choices. For both datasets, we found that \methodname-trained models consistently outperformed those that were trained without \methodname ($p < 0.05$, one-tailed paired Wilcoxon signed-rank test, see \textbf{Appendix} \ref{appen:graph_property_pred} for details).
% We also explored a \methodname-guided graph pruning approach. 
\methodname directly uses local pruning (i.e. edge interventions) to guide the training of graph attention in a manner that down-weights task-irrelevant edges. As such, we reasoned that attention coefficients produced by \methodname-trained models could be used to prune task-irrelevant edges (see \textbf{Appendix} \ref{appen:graph_rewiring} for more details). In this approach, we used \methodname's edge pruning procedure as a pre-processing step for training and inference with GCNs, which are more scalable than graph attention networks \citep{sign} but indiscriminate in how they aggregate information over node neighborhoods. We found that using \methodname-guided pruning improved the test accuracy of GCNs, outperforming vanilla GCNs trained and evaluated over the full graph as well as GCNs trained and evaluated on graphs pruned with baseline graph attention mechanisms. These preliminary results open the door for further exploration of \methodname's utility on these tasks.


\subsection{Interpreting Attention Coefficients: Qualitative Analysis}
\label{subsec:results:qa}
%Previous perturbative approaches to guide GNN training did not directly intervene on edges in a task-specific way, making their interpretability less clear.
In addition to providing a robust way to increase both model quality and generalization, we explored the interpretability of \methodname attention coefficients in a \textit{post hoc} analysis. Here, we evaluated the edge-wise difference of the attention coefficients between our method and a baseline GAT applied to the \textrm{ogbn-arxiv} dataset. In this dataset, nodes represent arXiv papers, edges are citation links, and the prediction task is to classify papers into their subject areas. 

We manually reviewed citations that were up/down-weighted by \methodname-trained models and observed that these citations broadly fit into one of three categories:  (i) down-weighting self-citations, (ii) down-weighting popular ``anchor'' papers, or (iii) upweighting topically-narrow papers with few citations. In the first case, we found that \methodname down-weights edges associated with self-citations (\textbf{Table}~\ref{tab:self-cites}). The causal story here is clear--- machine learning is a fast-moving field with authors moving into the field and changing specialties as those specialties are born. Because of this, the narrative arc that a set of authors constructs to present this idea can include citations to their own previous work from different sub-fields. While these citations help situate the work within the broader literature and can provide background that readers might find valuable, they are not relevant to the subject area prediction task. 

\begin{table}[ht]
\small
\caption{\label{tab:self-cites}Down-weighted self-citations. }
\renewcommand{\arraystretch}{1}
\begin{center}
\begin{tabular}{p{0.42\linewidth} p{0.42\linewidth} p{0.10\linewidth}}
Paper Title & Cited Title (from a different subject area) & $\Delta$ \\
 \hline 
\textit{Viterbinet a Deep Learning Based Viterbi Algorithm for Symbol Detection} &
\textit{Frequency Shift Filtering for Ofdm Signal Recovery in Narrowband Power Line Communications} & -89.91 \% \\
% \smallskip \\
\textit{Solving Underdetermined Systems with Error Correcting Codes} &
\textit{Systems of MDS Codes from Units and Idempotents} & -89.80 \% \\
% \smallskip \\
\textit{Performance Analysis for Multichannel Reception of OOFSK Signaling} &
\textit{On-Off Frequency-Shift Keying for Wideband Fading Channels} & -81.03 \% \\
\end{tabular}
\end{center}
\end{table}

In the second case, we found that \methodname down-weights edges directed towards popular or otherwise seminal ``anchor'' papers (\textbf{Appendix}~\ref{appen:interpret_qual}, \textbf{Table}~\ref{tab:anchor-cites}). These papers tends to be included in introductions to provide references for common concepts or methods, such as Adam, ResNet, and ImageNet. They are also widely cited across subject areas and hence have little bearing on the subject area prediction task. Notably, \methodname does not simply learn to ignore edges from high-degree nodes. For the Word2Vec paper, we observed notable increases in attention coefficients for edges connecting it to multiple highly related papers, including a $2.5\times 10^6$ \% increase for \textit{Efficient Graph Computation for Node2Vec} and a $2.0\times 10^6$ \% increase for \textit{Multi-Dimensional Explanation of Reviews	}.

In the final case, we observed that \methodname up-weighted edges directed towards deeply related but largely unnoticed papers (\textbf{Appendix}~\ref{appen:interpret_qual},\textbf{Table}~\ref{tab:up-cites}). In our manual exploration of the data, we observed that these papers are those that are close to the proposed method. These papers are the type that are often found only after a thorough literature review. Such edges should play a key role in predicting a paper's topic and should be up-weighted.


==> iclr2023/theory.tex <==
\subsection{Graph Attention Networks}

Attention mechanisms have been effectively used in many domains by enabling models to dynamically attend to the specific parts of an input that are relevant to a prediction task \citep{attention_survey}. In graph settings, attention mechanisms compute the relevance of edges in the graph for a prediction task. A neighbor aggregation operator then uses this information to weight the contribution of each edge \citep{gat_survey,gated_graph_sequence,self_attn_graph_pooling}. 

%The approach for computing attention is similar in many graph attention mechanisms. A graph attention layer takes as input a set of node features $\displaystyle \mh = \{\displaystyle \vh_1,...,\displaystyle \vh_N\}$, $\displaystyle \vh_i \in \mathbb{R}^F$, where $N$ is the number of nodes. The graph attention layer uses these node features to compute attention coefficients for each edge: $\alpha_{ij} = a(\displaystyle \mW \displaystyle \vh_i,\displaystyle \mW \displaystyle \vh_j)$, 

The approach for computing attention is similar in many graph attention mechanisms. A graph attention layer takes as input a set of node features = $\{\displaystyle \vh_1,...,\displaystyle \vh_N\}$, $\displaystyle \vh_i \in \mathbb{R}^F$, where $N$ is the number of nodes. The graph attention layer uses these node features to compute attention coefficients for each edge: $\alpha_{ij} = a(\displaystyle  \displaystyle \vh_i,\displaystyle  \displaystyle \vh_j)$, 

% \begin{equation}
%     \label{eqn:attn_edges}
%     e_{ij} = a(\displaystyle \mW\displaystyle \vh_i,\displaystyle \mW\displaystyle \vh_j),
% \end{equation}
where $a : \mathbb{R}^{F'} \times \mathbb{R}^{F'} \rightarrow (0,1)$ is the attention mechanism function, and the attention coefficient $\alpha_{ij}$ for an edge indicates the importance of node $i$'s input features to node $j$.
% $\displaystyle \mW\in \mathbb{R}^{F' \times F}$ projects the input features into a new feature space. The attention mechanism function $a : \mathbb{R}^{F'} \times \mathbb{R}^{F'} \rightarrow [0,1]$ uses these new node features to compute an attention coefficient $\alpha_{ij}$ for each edge that indicates the importance of node $i$'s input features to node $j$. 
% These attention coefficients are typically normalized with respect to the 1-hop neighborhood of each node using the softmax function, yielding normalized attention coefficients $\alpha_{ij}$ that indicate the importance of node $i$'s input features to node $j$.
For a node $j$, these attention coefficients are then used to compute a linear combination of its neighbors' features: $\displaystyle \vh_j' =  \sum_{i\in N(j)}\alpha_{ij}\displaystyle \mW\displaystyle \vh_i, ~ ~ \mathit{s.t.} ~ \sum_{i\in N(j)} \alpha_{ij} = 1$.
For multi-headed attention, each of the $K$ heads first independently calculates its own attention coefficients $\alpha_{i,j}^{(k)}$ with its head-specific attention mechanism $a^{(k)}(\cdot,\cdot)$, after which the head-specific outputs are averaged. 
% \begin{equation}
%     \label{eqn:attn_aggr}
%     \displaystyle \vh_j' =  \sum_{i\in N(j)}\alpha_{ij}\displaystyle \mW\displaystyle \vh_i,
%     ~ ~ \mathit{s.t.} ~ 
%     \sum_{i\in N(j)} \alpha_{ij} = 1
% \end{equation} 
% 

%RS: commenting out to save some space and make room for causal in the intro
%
%se attention coefficients are used to compute attention-head specific node outputs $\displaystyle \vh_j'^{(k)}$, which are then averaged across the $K$ attention heads.
%
% \begin{equation}
%     \label{eqn:attn_heads}
%     \displaystyle \vh_j' = \frac{1}{K}\sum_{k=1}^{K}\displaystyle \vh_j'^{(k)}
% \end{equation}

In this paper, we focus on three widely used graph attention architectures: the original graph attention network (GAT) \citep{gat}, a modified version of this original network (GATv2) \citep{gatv2}, and the Graph Transformer network \citep{transformerconv}. %These graph attention architecture variants are distinguished by the manner in which they compute the unnormalized attention coefficients $e_{ij}$ (Table \ref{table:gat_variants}). 
The three architectures and their equations for computing attention  are presented in \textbf{Appendix} \ref{appen:gat_variants}. 

% In the original graph attention network (GAT) framework, the unnormalized attention coefficients are computed as follows \citep{gat}. Here, $||$ denotes concatenation and the concatenated node features are passed through a single-layer feedforward neural network featuring a weight vector $\mathbf{a} \in \mathbb{R}^{2F'}$ and the LeakyRELU nonlinearity. 
% \begin{equation}
%     \label{eqn:gat_attn}
%     e_{ij} = \text{LeakyReLU}\big(\vec{\mathbf{a}}^T [ \displaystyle \mW\displaystyle \vh_i || \displaystyle \mW\displaystyle \vh_j \big)]\big)
% \end{equation}
% GATv2 was proposed to improve upon the expressiveness of the original graph attention mechanism by applying the linear projection to concatenated input node features instead of individual node features \citep{gatv2}.
% \begin{equation}
%     \label{eqn:gatv2_attn}
%     e_{ij} = \vec{\mathbf{a}}^T\text{LeakyReLU}\big( \displaystyle \mW \displaystyle \vh_i || \displaystyle \mW \displaystyle \vh_j \big)
% \end{equation}
% Lastly, the Graph Transformer network extends the Transformer architecture used in natural language processing \citep{transformer} to graphs and computes the attention coefficients as follows, where as above $F'$ is the dimensionality of the new feature space \citep{transformerconv}. 
% \begin{equation}
%     \label{eqn:transformer_attn}
%     e_{ij} = \frac{(\displaystyle \mW\displaystyle \vh_i)^T(\displaystyle \mW\displaystyle \vh_j)}{\sqrt{F'}}
% \end{equation}

\begin{figure}
    \centering
    %\includegraphics[width=0.95 \linewidth ]{iclr2023/causal_attn_fig1_rs-v4.pdf}
    \includegraphics[width=0.9 \linewidth ]{car_regularization_overview.pdf}
    \caption{Schematic of \methodname: Graph attention networks learn the relative importance of each node-neighbor for a given prediction task. However, their inferred attention coefficients can be miscalibrated due to noise, spurious correlations, or confounders (e.g., node size here). Our causal approach directly intervenes on a sampled subset of edges and supervises an auxiliary task that aligns an edge's causal importance to the task with its attention coefficient.}
    \label{fig:figure_1}
\end{figure}

\subsection{Causal Attention Regularization: an Invariance Prediction Formulation}

\methodname is motivated by the invariant prediction (IP) formulation of causal inference \citep{RePEc:bla:jorssb:v:78:y:2016:i:5:p:947-1012,graph_ood}. The central insight of this formulation is that, given sub-models that each contain a different set of predictor variables, the underlying causal model of a system is comprised of the set of all sub-models for which the predicted class distributions are equivalent, up to a noise term. This approach is capable of providing statistically rigorous estimates for both the causal effect strength of predictor variables as well as confidence intervals. With \methodname, our core insight is that the graph structure itself, in addition to the set of node features, comprise the set of predictor variables.
% that are traditionally explored in causal regularization frameworks. 
This is equivalent to the intuition that relevant edges for a particular task should not only be assigned high attention coefficients but also be important to the predictive accuracy of the model (\textbf{Figure} \ref{fig:figure_1}). The removal of these relevant edges from the graph should cause the predictions that rely on them to substantially worsen. 

We leverage the residual formulation of IP to formalize this intuition. This formulation assumes that we can generate sub-models for different sets of predictor variables, each corresponding to a separate experiment $e \in \mathcal{E}$. For each sub-model $S^e$, we compute the predictions $Y^e = g(\mathcal{G}^e_\mathcal{S}, \mathcal{X}^e_\mathcal{S}, \epsilon^e)$ where $\mathcal{G}$ is the graph structure,  $\mathcal{X}$ is the set of features associated with $\mathcal{G}$, $\epsilon^e$ is the noise distribution, and $\mathcal{S}$ is the set of predictor variables corresponding to $S^e$. We next compute the residuals $\mathcal{R} = Y - Y^e$. IP requires that we perform a hypothesis test on the means of the residuals, with the generic approach being to perform an F-test for each sub-model against the null-hypothesis. The relevant assumptions ($\epsilon^e \sim F_\epsilon$, and $\epsilon^e \indep S^e$ for all $e \in \mathcal{E}$) are satisfied if and only if the conditionals $Y^e|S^e$ and $Y^f | S^f$ are identical for all experiments $e, f \in \mathcal{E}$.

We use an edge intervention-based strategy that corresponds precisely to this IP-based formulation. However, we differ from the standard IP formulation in how we estimate the final causal model. While IP provides a method to explicitly construct an estimator of the true causal model (by taking the intersection of all models for which the null hypothesis was rejected), we rely on  intervention-guided regularization of graph attention coefficients as a way to aggregate sub-models while balancing model complexity and runtime considerations. In our setting, each sub-model corresponds to a set of edge interventions and, thus, slightly different graph structures. The same GNN architecture is trained on each of these sub-models. Given a set of experiments $\mathcal{E} = \{e\}$ with sub-models $S^e$, outputs $Y^e$ and errors $\epsilon^e$, we regularize the attention coefficients to align with sub-model errors, thus learning a GNN architecture primarily from causal sub-models. Incorporating this regularization as an auxiliary task, we seek to minimize the following loss:
%
% . Including this regularization loss as an auxiliary task alongside the primary prediction task then encourages GNN architectures learned primarily from causal sub-models. Specifically, we seek to minimize the following loss:
%
% % We begin by briefly presenting the residual formulation of invariant prediction and then discuss in detail our notion of predictor variable, experiment generation, and experiment test. 
% We leverage the residual formulation of IP, which assumes that we can generate many sub-models with different sets of predictor variables $S^e$ corresponding to many different experiments. We can compute the predictions, $Y^e$ for every sub-model as well as the residuals $\mathcal{R} = Y - Y^e$. IP requires that we perform a hypothesis test on the means of the residuals. The generic method for invariant prediction is to test each hypothetical set of features against the null-hypothesis, $H_{0,S}(\mathcal{E})$, such that there exists $g: \mathbb{R}^{|S|} \times \mathbb{R} \rightarrow \mathbb{R}$ and $\epsilon^e$ that $Y^e = g(\mathcal{G}^e_S, \mathcal{X}^e_S, \epsilon^e)$, $\epsilon^e \sim F_\epsilon$ and $\epsilon^e \indep S^e$ for all $e \in \mathcal{E}$. This is satisfied if the conditionals $Y^e|S^e$ and $Y^f | S^f$ are identical for all experiments $e, f \in \mathcal{E}$. IP then provides a method to construct an estimator of the true causal model by taking the intersection of all models for which the null hypothesis was rejected. 
% % A key question in causal inference is the identification of identifiable models. Theorem 2 of \citet{RePEc:bla:jorssb:v:78:y:2016:i:5:p:947-1012} indicates that do-interventions such explicit edge deletions generate identifiable causal models in the limit that all predictor variables have been independently intervened upon. While this would be computationally intractable, 
% Rather than explicitly construct our estimator, we rely on regularization as a way to balance the complexity and instability of the model in the following way:
\begin{equation}
    \label{eqn:full_objective}
    \mathcal{L} = \mathcal{L}^{p} + \lambda \mathcal{L}^{c}
\end{equation}

The full loss function $\mathcal{L}$ consists of the loss associated with the prediction $\mathcal{L}^p$, the loss associated with causal attention task $\mathcal{L}^{c}$, and a causal regularization strength hyperparameter $\lambda$ that mediates the contribution of the regularization loss to the objective. For the prediction loss, we have $\mathcal{L}^p=\frac{1}{N}\sum_{n=1}^{N}\ell^p(\hat{y}^{(n)}, y^{(n)})$, where $N$ is the size of the training set, $\ell^p(\cdot,\cdot)$ corresponds to the loss function for the given prediction task, $\hat{y}^{(n)}$ is the prediction for entity $n$, and $y^{(n)}$ is the ground truth value for entity $n$. We seek to align the attention coefficient for an edge with the causal effect of removing that edge through the use of the following loss function:
\begin{equation}
    \label{eqn:causal_reg}
    \mathcal{L}^{c} = \frac{1}{R} \sum^{R}_{r=1} \bigg( \frac{1}{\left| S^{\left( r \right )} \right|}\sum_{\left(n, i, j \right) \in S^{\left( r \right ) }} \ell^{c} \left( \alpha_{ij}^{(n)}, c_{ij}^{(n)} \right) \bigg)
\end{equation}
Here, $n$ represents a single entity for which we aim to make a prediction. For a node prediction task, the entity $n$ corresponds to a node, and in a graph prediction task, $n$ corresponds to a graph. In this paper, we assume that all edges are directed and, if necessary, decompose an undirected edge into two directed edges. In each mini-batch, we generate $R$ separate sub-models, each of which consists of a set of edge interventions $S^{(r)}$, $r=1,\ldots,R$. Each edge intervention in $S^{(r)}$ is represented by a set of tuples $(n,i,j)$ which denote a selected edge $(i,j)$ for an entity $n$. Note that in a node classification task, $n$ is the same as $j$ (i.e., the node with the incoming edge). More details for the edge intervention procedure and causal effect calculations can be found in the sections below. The causal effect $c_{ij}^{(n)}$ scores the impact of deleting edge $(i,j)$ through a likelihood ratio test. This causal effect is compared to the edge's attention coefficient $\alpha_{ij}^{(n)}$ via the loss function $\ell^c(\cdot,\cdot)$. A detailed algorithm for \methodname is provided in algorithm~\ref{alg:cap}.

\begin{algorithm}
\caption{\methodname Framework}\label{alg:cap}
\begin{algorithmic}
\Require Training set $\mathcal{D}_{train}$, validation set $\mathcal{D}_{val}$, model $\mathcal{M}$, regularization strength $\lambda$
% \Ensure $y = x^n$
\Repeat % For {$\text{epoch } i \gets 1 \text{ to } M$}
    \ForEach {$\text{mini-batch } \{ \mathcal{B}^k = \{n_j^{(k)}\}_{j=1}^{b_k}\}$}
    \State $\text{Prediction loss: } \mathcal{L}^p \gets \frac{1}{|\mathcal{B}^k|}\sum_{n \in \mathcal{B}^k}\ell^p(\hat{y}^{(n)}, y^{(n)}) $
    \Procedure{Edge intervention}{}
    \State $\text{Causal attention loss: } \mathcal{L}^c \gets 0$
    \For {$\text{round } r \gets 1 \text{ to } R$}
        \State {$\text{Set of edge interventions } S(r) \gets \{\}$}
        \ForEach {$\text{entity } \{n_j^{(k)}\}_{j=1}^{b_k}$}
        \State $\text{Sample edge }(i,j) \sim E_{n_j^{(k)}}$ \Comment{$E_{n_j^{(k)}}$ set of edges related to entity $n_j^{(k)}$}
        %\If {$(i,j) \text{ only affects } n_j^{(k)}$} \Comment{See ``Edge intervention procedure"}
        \If {$(i,j) \text{ independent of } S(r)$} \Comment{See ``Edge intervention procedure"}
            \State $S(r) \gets S(r) \text{ } \cup (n_j^{(k)},i,j)$  \Comment{Add edge to set of edge interventions}
            \State $\text{Compute causal effect } c_{ij}^{(n)} \gets \sigma \big( \big( \rho^{(n)}_{ij} \big)^{d(n)} - 1 \big)$ \Comment{Equation 5}
        \EndIf
        \EndFor
    \State $\mathcal{L}^{c} \gets \mathcal{L}^{c} + \frac{1}{R}  \frac{1}{\left| S^{\left( r \right )} \right|}\sum_{\left(n, i, j \right) \in S^{\left( r \right ) }} \ell^{c} \left( \alpha_{ij}^{(n)}, c_{ij}^{(n)} \right)$ \Comment{Equation 3}
    \EndFor
    \EndProcedure
    \State $\text{Total loss: } \mathcal{L} = \mathcal{L}^{p} + \lambda\mathcal{L}^{c}$
    \State $\text{Update model parameters to minimize } \mathcal{L}$
    \EndFor
\Until $\text{Convergence criterion}$ \Comment{We use convergence of the validation prediction loss.}
% \EndFor
\end{algorithmic}
\end{algorithm}

% For models with multiple attention heads, $\alpha_{ij}^{(n)}$ is the mean attention coefficient across heads.

% We regularize the attention mechanism in accordance with the learned causal effects from edge interventions. Thus, our full objective function $\mathcal{L}$ includes the loss associated with the prediction $\mathcal{L}^p$, the loss associated with causal attention task $\mathcal{L}^{c}$, and a causal regularization strength hyperparameter $\lambda$ that mediates the contribution of the causal attention task to the objective. 

% We formalize this intuition by devising an auxiliary supervised prediction task that aims to align the attention coefficient for an edge with the causal effect of removing that edge as per the following loss function:


% \paragraph{Causal attention objective}
% We leverage the intuition that relevant node-neighbor relations for a particular task should not only be assigned high attention coefficients but also be important to the predictive accuracy of the model (\textbf{Figure} \ref{fig:figure_1}). When removed from the graph, these relevant edges should cause the predictions that rely on them to substantially worsen. We formalize this intuition by devising an auxiliary supervised prediction task that aims to align the attention coefficient for an edge with the causal effect of removing that edge as per the following loss function:
% \begin{equation}
%     \label{eqn:causal_reg}
%     \mathcal{L}^{c} = \frac{1}{R} \sum^{R}_{r=1} \bigg( \frac{1}{\left| S^{\left( r \right )} \right|}\sum_{\left(n, i, j \right) \in S^{\left( r \right ) }} \ell^{c} \left( \alpha_{ij}^{(n)}, c_{ij}^{(n)} \right) \bigg)
% \end{equation}
% \begin{equation}
%     \label{eqn:causal_reg}
%     \mathcal{L}^{c} = \frac{1}{N} \sum^{N}_{n=1} \frac{1}{\left| S^{\left( n \right )} \right|} \sum_{\left( i, j \right) \in S^{\left( n \right ) }} \ell^{c} \left( \alpha_{ij}^{(n)}, c_{ij}^{(n)} \right)
% \end{equation}

% Here, $n$ represents a single entity for which we aim to make a prediction. For a node prediction task, $n$ corresponds to a node, while in a graph prediction task, $n$ corresponds to a graph. $N$ represents the number of such entities in the training set. $\alpha_{ij}^{(n)}$ is the attention coefficient associated with edge $(i,j)$ for entity $n$. For models with multiple attention heads, $\alpha_{ij}^{(n)}$ is the mean attention coefficient for edge $(i,j)$ for entity $n$ across the attention heads. 

% $S^{(n)}$ denotes a set of edges $(i,j)$ associated with entity $n$ that will be individually removed from the training data to compute the causal effect $c_{ij}^{(n)}$. Importantly, we select only one edge per entity to remove in computing $c_{ij}^{(n)}$, so that the direct causal effect of each intervention can be calculated independently of other interventions. $\ell^c(\cdot,\cdot)$ is the loss function used to compare the attention coefficients and the causal effects, which we refer to as the causal regularization loss. 


% Here, $n$ represents a single entity for which we aim to make a prediction. For a node prediction task, the entity $n$ corresponds to a node, and in a graph prediction task, $n$ corresponds to a graph. In this paper, we assume that all edges are directed and, if necessary, decompose an undirected edge into two directed edges. In each mini-batch, we perform $R$ separate rounds of causal effect calculations, each of which consists of a set of edge interventions $S^{(r)}$, $r=1,\ldots,R$. More details for the edge intervention procedure and causal effect calculations can be found in the sections below. 

% Each edge intervention in $S^{(r)}$ is represented by a set of tuples $(n,i,j)$ which denote a selected edge $(i,j)$ for an entity $n$. Note that in a node classification task, $n$ is the same as $j$ (i.e., the node with the incoming edge). The causal effect $c_{ij}^{(n)}$ scores the impact of deleting edge $(i,j)$ on predictive performance. This causal effect is compared to the edge's attention coefficient $\alpha_{ij}^{(n)}$ via the loss function $\ell^c(\cdot,\cdot)$. For models with multiple attention heads, $\alpha_{ij}^{(n)}$ is the mean attention coefficient across heads.

% We regularize the attention mechanism in accordance with the learned causal effects from edge interventions. Thus, our full objective function $\mathcal{L}$ includes the loss associated with the prediction $\mathcal{L}^p$, the loss associated with causal attention task $\mathcal{L}^{c}$, and a causal regularization strength hyperparameter $\lambda$ that mediates the contribution of the causal attention task to the objective. 

% \begin{equation}
%     \label{eqn:full_objective}
%     \mathcal{L} = \mathcal{L}^{p} + \lambda \mathcal{L}^{c}
% \end{equation}
% Here, we have $\mathcal{L}^p=\frac{1}{N}\sum_{n=1}^{N}\ell^p(\hat{y}^{(n)}, y^{(n)})$, where $N$ is the size of the training set, $\ell^p(\cdot,\cdot)$ corresponds to the loss function for the given prediction task, $\hat{y}^{(n)}$ is the prediction for entity $n$, and $y^{(n)}$ is the ground truth value for entity $n$. A detailed algorithm for \methodname is provided in \textbf{Appendix} \ref{appen:algo}.

\paragraph{Edge intervention procedure}
% Classification tasks on graphs can be understood as estimating $p( C | \mathcal{G}, \mathcal{X} ) = p(C | S) $, where $\mathcal{G}$ is the graph structure, $\mathcal{X}$ is the set of features associated with the graph $\mathcal{G}$, and $S$ is the set of predictor variables. For node classification, the node label is the target variable of interest, and the model is composed of the adjacency matrix and the method by which probabilities are computed. To construct a GNN capable of causal inference, we require a technique to generate different sub-models and experiments with different conditional dependence structures. Each sub-model will have the same GNN structure but a slightly different graph structure generated via edge-removal. Given a set of experiments $\{ \mathcal{E} \}$, with target variables $Y^e$ and predictor variables $S^e$, we say that the subset of latent variables, $S^*$, is causal for the prediction of target variable $Y$ if for all $e \in \mathcal{E}$, $S^e$ has an arbitrary distribution and $Y^e = g(S^e, \epsilon^e)$ where $g$ is our statistical model, and $\epsilon^e \sim F_{\epsilon}$ is the error distribution.
%
We sample a set of edges in each round $r$ such that the prediction for each entity will strictly be affected by at most one edge intervention in that round to ensure effect independence. For example, in a node classification task for a model with one GNN layer, a round of edge interventions entails removing only a single incoming edge for each node being classified. In the graph property prediction case, only one edge will be removed from each graph per round. Because a model with one GNN layer only aggregates information over a 1-hop neighborhood, the removal of each edge will only affect the model's prediction for that edge's target node. To select a set of edges in the $L$-layer GNN case, edges are sampled from the 1-hop neighborhood of each node being classified, and sampled edges that lie in more than one target nodes' $L$-hop neighborhood are removed from consideration as intervention candidates. %; this limits the computational expense of interventions. 

This edge intervention selection procedure is crucial, as it enables the causal effect of each selected intervention $c_{ij}^{(n)}$ on an entity $n$ to be calculated independently of other interventions on a graph. Moreover, by selecting only one intervention per entity within each round, we can parallelize the computation of these causal effects across all entities per round instead of iteratively evaluating just one intervention for the entire graph per entity, significantly aiding scalability. 
 
\paragraph{Calculating task-specific causal effects}
\label{subsec:methods:causaleffect}
We quantify the causal effect of an intervention at edge $(i,j)$ on entity $n$ through the use of an approximate likelihood-ratio test

% as the relative change in the prediction loss for entity $n$ upon removal of that edge.
% \begin{equation}
%     \label{eqn:causal_effect}
%     c_{ij}^{(n)} = \sigma \bigg( \bigg( \frac{\ell^p \bigl( \hat{y}_{\backslash ij}^{(n)}, y^{(n)} \bigr)} {\ell^p \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)} \bigg)^{d(n)}  -1 \bigg)
% \end{equation}

\begin{equation}
    \label{eqn:causal_effect}
    c_{ij}^{(n)} = \sigma \bigg( \bigg( \rho^{(n)}_{ij} \bigg)^{d(n)} - 1 \bigg)\;\;\;\text{where}\;\; \rho^{(n)}_{ij} = \frac{\ell^p \bigl( \hat{y}_{\backslash ij}^{(n)}, y^{(n)} \bigr)} {\ell^p \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)}
\end{equation}

% \begin{equation}
%     \label{eqn:causal_effect}
%     c_{ij}^{(n)} = \sigma \bigg( \frac{\ell^p \bigl( \hat{y}_{\backslash ij}^{(n)}, y^{(n)} \bigr)-\ell^p \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)} {\ell^p \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)} \bigg)
% \end{equation}
Here, $\hat{y}_{\backslash ij}^{(n)}$ is the prediction for entity $n$ upon removal of edge $(i,j)$. $d(n)$ represents the node degree for node classification, while it represents the number of edges in a graph for graph classification. Interventions will likely have smaller effects on higher degree nodes due to the increased likelihood of there being multiple edges that are relevant and beneficial for predictions for such nodes. In graph classification, graphs with many edges are likely to be less affected by interventions as well. Exponentiating the relative intervention effect $\rho^{(n)}_{ij}$ by $d(n)$ is intended to adjust for these biases. We have experimented both with and without raising $\rho$ to the factor of $d$, but have found empirically better results with. We do not have a rigorous explanation as to why, although we suspect the correlated nature of edges implies some amount of shrinkage is necessary. 

% $\ell^p \bigl( \hat{y}_{\backslash ij}^{(n)}, y^{(n)} \bigr) / \ell^p \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)$ so as to account for the number of edges contributing to the prediction for entity $n$. For example, in node classification tasks, predictions for a high-degree node will involve aggregating information over many neighbors, so the effect of a single edge intervention is adjusted via this $d(n)$ term to account for this specific node's high-degree context. 
The link function $\sigma : \mathbb{R} \rightarrow (0,1)$ maps its input to the support of the distribution of attention coefficients. The predictions $\hat{y}^{(n)}$ and $\hat{y}_{\backslash ij}^{(n)}$ are generated from the graph attention network being trained with \methodname. We emphasize that $\hat{y}^{(n)}$ and $\hat{y}_{\backslash ij}^{(n)}$ are both computed during the same training run, rather than in two separate runs. 

% \RS{@AW: the two y's are computed in a single run, right? pls clarify that as a line here?}
% \AW{added another sentence. is this what you mean?}
% %Furthermore, by using the prediction loss in these calculations, \methodname guides attention learning in a manner that is aware of the causal effects on the specific prediction task at hand. 

\paragraph{Scalability}
\methodname increases the computational cost of training in two ways: (i) additional evaluations of the loss function due to the causal effect calculations, and (ii) searches to ensure independent interventions. \methodname performs $\mathcal{O}(RN)$ interventions, where $R$ is the number of interventions per entity and $N$ is the number of entities in the training set. Because our edge intervention procedure ensures that the sampled interventions per round are independent, the causal effects of these interventions can be computed in parallel. In addition, if edge interventions were sampled uniformly across the graph, ensuring the independence each intervention would require a $L$-layer deep BFS that has time complexity $\mathcal{O}(b^L)$, resulting in a worst case time complexity of $\mathcal{O}(R N b^L)$, where $L$ is the depth of the GNN, and $b$ is the mean in-degree. We note that, in practice, GNNs usually have $L \leq 2$ layers since greater depth increases the computational cost and the risk of oversmoothing~\citep{gcn_oversmoothing,measuring_oversmoothing,topping2022understanding}. The contribution of this intervention overlap search step would, therefore, be minimal for most GNNs. We are also able to mitigate much of the computational cost by parallelizing these searches. Further speedups can achieved by identifying non-overlapping interventions as a preprocessing step. In summary, we have found \methodname to have a modest effect on the scalability of graph attention methods, with training runtimes that are only increased by 1.5-2 fold (\textbf{Appendix} \ref{appen:runtime_memory}).

%We have found \methodname to be highly scalable, with training runtimes that are only 1.5-2x of non-regularized attention training (Appendix \ref{appen:runtime_memory}).

% \TM{ Number of interventions scales as $O(C * |V|)$. Each intervention scales as $O(b^2l)$ due to the BFS to ensure non-overlapping interventions, where b is the branching factor and l is the number of layers. In the long run, we're unconcerned about the identification of non-overlapping interventions can be done as a preprocessing step, similar to the generation of graph samples in graph sage.}


==> iclr2023/todos.tex <==
\todo[inline]{
Todos: \\
1. P0 Results: \\
 \;\; - \sout{Abstract: need a summary stat or two} \\
 \;\; - Ablations: a) in appendix: need table of correlations between attn wts and homophily scores. b) put in line markers for what random baseline will be \\ 
 \;\; - \sout{Ablations: need label-propagation results} \\
 \;\; - Scalability: need runtimes and machine details \\
2. P0 Writing: \\
 \;\; - \sout{Interpretability: which dataset? \TM{ogbn-arxiv}} \\
3. P1 Results: \\
 \;\; - Fig 3: needs other 3 datasets (in appendix). Also needs p-values \\
 \;\; - Extra: graph property-prediction + graph rewiring. Ok to have limited examples \\
 \;\; - random/uniform regularization 
 \;\; - Should we worry about graph diffusion distance and cheeger constant stuff? Could be a solid appendix section

}


==> iclr2023/v1_theory.tex <==
\subsection{Graph Attention Networks}

Attention mechanisms have been effectively used across many domains by enabling models to dynamically attend to the specific parts of an input that are most relevant to a prediction task \citep{attention_survey}. In graph settings, attention mechanisms compute the relevance of node-neighbor relations. The neighbor aggregation operator in GNNs then uses this information to weight the contribution of each node-neighbor relation in the prediction task. 

Across the multitude of graph attention mechanisms that have been proposed \citep{gat_survey}, the procedures for computing attention take on a general form \citep{gat}. A graph attention layer takes as input a set of node features $\mathbf{h} = \{\vec{h}_1,...,\vec{h}_N\}$, $\vec{h}_i \in \mathbb{R}^F$, where $N$ is the number of nodes and $F$ is the dimensionality of the node features. From these node features, the graph attention layer in a GAT computes unnormalized attention weights for each edge $(i,j)$
\begin{equation}
    \label{eqn:attn_edges}
    e_{ij} = a(\mathbf{W}\vec{h}_i,\mathbf{W}\vec{h}_j),
\end{equation}
where $\mathbf{W}\in \mathbb{R}^{F' \times F}$ linearly projects the input features into a new feature space and the attention mechanism function $a : \mathbb{R}^{F'} \times \mathbb{R}^{F'} \rightarrow \mathbb{R}$ uses these new node features to compute an attention weight for each edge. These attention weights are typically normalized with respect to the 1-hop neighborhood of each node using the softmax function, yielding normalized attention coefficients $\alpha_{ij}$ that indicate the importance of node $i$'s input features to node $j$. For a node $j$, these normalized attention weights are then used to compute a linear combination of the new features for node $j$'s neighbors, which serves as the output of the graph attention layer for node $j$.
\begin{equation}
    \label{eqn:attn_aggr}
    \vec{h}_j' =  \sum_{i\in N_j}\alpha_{ij}\mathbf{W}\vec{h}_i
\end{equation} 
% 
To employ multi-headed attention with $K$ heads, each of the $K$ attention mechanisms first independently calculates its respective normalized attention weights $\alpha_{i,j}^{(k)}$ using its own attention mechanism function $a^{(k)}( \cdot )$ and linear projection weights $\mathbf{W}^{(k)}$. These attention weights are used to compute attention head-specific node outputs $\vec{h}_j'^{(k)}$, which are then averaged across the $K$ attention heads.
\begin{equation}
    \label{eqn:attn_heads}
    \vec{h}_j' = \frac{1}{K}\sum_{k=1}^{K}\vec{h}_j'^{(k)}
\end{equation}

In this paper, we focus on three widely used graph attention architectures: the original graph attention network (GAT) \citep{gat}, a modified version of this original network (GATv2) \citep{gatv2}, and the Graph Transformer network \cite{transformerconv}. These graph attention architecture variants are distinguished by the manner in which they compute the unnormalized attention weights $e_{ij}$ (Table \ref{table:gat_variants}). Here, $||$ denotes concatenation. For GAT and GATv2, the concatenated node features are passed through a single-layer feedforward neural network featuring a weight vector $\mathbf{a} \in \mathbb{R}^{2F'}$ and the LeakyReLU nonlinearity. 

\begin{table}[h!]
\centering
\caption{Attention weight calculation across graph attention architecture variants}
\label{table:gat_variants}
\renewcommand{\arraystretch}{2.5}
\begin{tabular}{ | c | c |} 
    \hline
    GAT \citep{gat} & \(\displaystyle e_{ij} = \text{LeakyReLU}\big(\vec{\mathbf{a}}^T [ \mathbf{W}\vec{h}_i || \mathbf{W}\vec{h}_j \big)]\big) \)  \\
    \hline
    GATv2 \citep{gatv2} & \(\displaystyle e_{ij} = \vec{\mathbf{a}}^T\text{LeakyReLU}\big( \mathbf{W} \vec{h}_i || \mathbf{W} \vec{h}_j \big) \) \\ 
    \hline
    Graph Transformer \citep{transformerconv} & \(\displaystyle e_{ij} = \frac{(\mathbf{W}\vec{h}_i)^T(\mathbf{W}\vec{h}_j)}{\sqrt{F'}} \) \\ 
    \hline
\end{tabular}
\end{table}

% In the original graph attention network (GAT) framework, the unnormalized attention weights are computed as follows \citep{gat}. Here, $||$ denotes concatenation and the concatenated node features are passed through a single-layer feedforward neural network featuring a weight vector $\mathbf{a} \in \mathbb{R}^{2F'}$ and the LeakyRELU nonlinearity. 
% \begin{equation}
%     \label{eqn:gat_attn}
%     e_{ij} = \text{LeakyReLU}\big(\vec{\mathbf{a}}^T [ \mathbf{W}\vec{h}_i || \mathbf{W}\vec{h}_j \big)]\big)
% \end{equation}
% GATv2 was proposed to improve upon the expressiveness of the original graph attention mechanism by applying the linear projection to concatenated input node features instead of individual node features \citep{gatv2}.
% \begin{equation}
%     \label{eqn:gatv2_attn}
%     e_{ij} = \vec{\mathbf{a}}^T\text{LeakyReLU}\big( \mathbf{W} \vec{h}_i || \mathbf{W} \vec{h}_j \big)
% \end{equation}
% Lastly, the Graph Transformer network extends the Transformer architecture used in natural language processing \citep{transformer} to graphs and computes the attention weights as follows, where as above $F'$ is the dimensionality of the new feature space \citep{transformerconv}. 
% \begin{equation}
%     \label{eqn:transformer_attn}
%     e_{ij} = \frac{(\mathbf{W}\vec{h}_i)^T(\mathbf{W}\vec{h}_j)}{\sqrt{F'}}
% \end{equation}

\subsection{Causal Attention Regularization Scheme}

We propose a general-purpose regularization framework for graph attention networks that enhances a given learning task by including an attention learning scheme based on active graph interventions. In this framework, we leverage the intuition that relevant node-neighbor relations for a particular task should not only be assigned high attention weights but also be important to the predictive accuracy of the model. When removed from the graph, these relevant edges should cause the predictions that rely on them to dramatically worsen. 

\subsubsection{Causal Attention Objective}
We formalize this intuition by devising a weakly supervised prediction task that aims to align the attention weight for an edge with the causal effect of removing that edge. The objective function for this task is as follows. 
\\
\begin{equation}
    \label{eqn:causal_reg}
    \mathcal{L}^{c} = \frac{1}{R} \sum^{R}_{r=1} \frac{1}{\left| S^{\left( r \right )} \right|}\sum_{\left(n, i, j \right) \in S^{\left( r \right ) }} \ell^{c} \left( \alpha_{ij}^{(n)}, c_{ij}^{(n)} \right)
\end{equation}
% \begin{equation}
%     \label{eqn:causal_reg}
%     \mathcal{L}^{c} = \frac{1}{N} \sum^{N}_{n=1} \frac{1}{\left| S^{\left( n \right )} \right|} \sum_{\left( i, j \right) \in S^{\left( n \right ) }} \ell^{c} \left( \alpha_{ij}^{(n)}, c_{ij}^{(n)} \right)
% \end{equation}

% Here, $n$ represents a single entity for which we aim to make a prediction. For a node prediction task, $n$ corresponds to a node, while in a graph prediction task, $n$ corresponds to a graph. $N$ represents the number of such entities in the training set. $\alpha_{ij}^{(n)}$ is the attention weight associated with edge $(i,j)$ for entity $n$. For models with multiple attention heads, $\alpha_{ij}^{(n)}$ is the mean attention weight for edge $(i,j)$ for entity $n$ across the attention heads. 

% $S^{(n)}$ denotes a set of edges $(i,j)$ associated with entity $n$ that will be individually removed from the training data to compute the causal effect $c_{ij}^{(n)}$. Importantly, we select only one edge per entity to remove in computing $c_{ij}^{(n)}$, so that the direct causal effect of each intervention can be calculated independently of other interventions. $\ell^c(\cdot,\cdot)$ is the loss function used to compare the attention weights and the causal effects, which we refer to as the causal regularization loss. 

Here, $n$ represents a single entity for which we aim to make a prediction. For a node prediction task, $n$ corresponds to a node, while in a graph prediction task, $n$ corresponds to a graph. We perform $R$ rounds of edge interventions per mini-batch, sampling a set of edges in each round such that the prediction for each entity in the mini-batch will strictly be affected by at most one edge intervention in that round. For example, in a node classification task for a model with one GNN layer, one round of edge interventions for a mini-batch entails removing only a single incoming edge for each node being classified in the mini-batch. Because a model with one GNN layer only aggregates information over a 1-hop neighborhood, the removal of each edge will only affect the model's prediction for that edge's target node. Similarly, in the graph property prediction case, only one edge will be removed from each graph per round. $S^{(r)}$ denotes a set of tuples $(n,i,j)$, each of which corresponds to a selected edge $(i,j)$ for an entity $n$ in round $r$. 

This edge intervention selection procedure is crucial, as it enables the direct causal effect of each selected intervention $c_{ij}^{(n)}$ on an entity $n$ to be calculated independently of other interventions. Furthermore, by selecting only one intervention per entity within each round, we can parallelize the computation of these direct causal effects across all entities per round, enabling the causal effect calculations to be highly scalable. Each causal effect $c_{ij}^{(n)}$ is compared to the attention weight $\alpha_{ij}^{(n)}$ of its corresponding edge via the loss function $\ell^c(\cdot,\cdot)$. For models with multiple attention heads, $\alpha_{ij}^{(n)}$ is the mean attention weight for edge $(i,j)$ for entity $n$ across the attention heads.

We quantify the causal effect $c_{ij}$ of removing edge $(i,j)$ on the prediction for entity $n$ as follows. 
\begin{equation}
    \label{eqn:causal_effect}
    c_{ij}^{(n)} = \sigma \bigg( \frac{\ell \bigl( \hat{y}_{\backslash ij}^{(n)}, y^{(n)} \bigr)-\ell \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)} {\ell \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)} \bigg)
\end{equation}
% talk about importance of using prediction loss to compute causal effect instead of just change in predictions???
$\ell^p(\cdot,\cdot)$ corresponds to the loss function for the given prediction task, $\hat{y}^{(n)}$ is the prediction for entity $n$, $\hat{y}_{\backslash ij}^{(n)}$ is the prediction for entity $n$ upon removal of edge $(i,j)$, and $y^{(n)}$ is the ground truth value for entity $n$. We also include $\sigma(\cdot)$ as a link function that maps its input to the support of the distribution of attention weights. 

We include the above learning task as an additional task to be optimized during training so as to regularize the attention mechanism in accordance with the learned causal effects from edge interventions. Thus, our full objective function $\mathcal{L}$ includes the loss associated with the prediction $\mathcal{L}^p$, the loss associated with causal attention task $\mathcal{L}^{c}$, and a causal regularization strength hyperparameter $\lambda$ that mediates the contribution of the causal attention task to the objective.
\begin{equation}
    \label{eqn:full_objective}
    \mathcal{L} = \mathcal{L}^{p} + \lambda \mathcal{L}^{c}
\end{equation}

==> iclr2023/v2_theory.tex <==
\subsection{Graph Attention Networks}

Attention mechanisms have been effectively used in many domains by enabling models to dynamically attend to the specific parts of an input that are relevant to a prediction task \citep{attention_survey}. In graph settings, attention mechanisms compute the relevance of edges in the graph for a prediction task. A neighbor aggregation operator then uses this information to weight the contribution of each edge \citep{gat_survey,gated_graph_sequence,self_attn_graph_pooling}. 

The approach for computing attention is similar in many graph attention mechanisms. A graph attention layer takes as input a set of node features $\mathbf{h} = \{\vec{h}_1,...,\vec{h}_N\}$, $\vec{h}_i \in \mathbb{R}^F$, where $N$ is the number of nodes. The graph attention layer uses these node features to compute attention coefficients for each edge: $\alpha_{ij} = a(\mathbf{W}\vec{h}_i,\mathbf{W}\vec{h}_j)$, 
% \begin{equation}
%     \label{eqn:attn_edges}
%     e_{ij} = a(\mathbf{W}\vec{h}_i,\mathbf{W}\vec{h}_j),
% \end{equation}
where $a : \mathbb{R}^{F'} \times \mathbb{R}^{F'} \rightarrow (0,1)$ is the attention mechanism function, and the attention coefficient $\alpha_{ij}$ for an edge indicates the importance of node $i$'s input features to node $j$.
% $\mathbf{W}\in \mathbb{R}^{F' \times F}$ projects the input features into a new feature space. The attention mechanism function $a : \mathbb{R}^{F'} \times \mathbb{R}^{F'} \rightarrow [0,1]$ uses these new node features to compute an attention coefficient $\alpha_{ij}$ for each edge that indicates the importance of node $i$'s input features to node $j$. 
% These attention coefficients are typically normalized with respect to the 1-hop neighborhood of each node using the softmax function, yielding normalized attention coefficients $\alpha_{ij}$ that indicate the importance of node $i$'s input features to node $j$.
For a node $j$, these attention coefficients are then used to compute a linear combination of its neighbors' features: $\vec{h}_j' =  \sum_{i\in N(j)}\alpha_{ij}\mathbf{W}\vec{h}_i, ~ ~ \mathit{s.t.} ~ \sum_{i\in N(j)} \alpha_{ij} = 1$.
For multi-headed attention, each of the $K$ heads first independently calculates its own attention coefficients $\alpha_{i,j}^{(k)}$ with its head-specific attention mechanism $a^{(k)}(\cdot,\cdot)$, after which the head-specific outputs are averaged. 
% \begin{equation}
%     \label{eqn:attn_aggr}
%     \vec{h}_j' =  \sum_{i\in N(j)}\alpha_{ij}\mathbf{W}\vec{h}_i,
%     ~ ~ \mathit{s.t.} ~ 
%     \sum_{i\in N(j)} \alpha_{ij} = 1
% \end{equation} 
% 

%RS: commenting out to save some space and make room for causal in the intro
%
%se attention coefficients are used to compute attention-head specific node outputs $\vec{h}_j'^{(k)}$, which are then averaged across the $K$ attention heads.
%
% \begin{equation}
%     \label{eqn:attn_heads}
%     \vec{h}_j' = \frac{1}{K}\sum_{k=1}^{K}\vec{h}_j'^{(k)}
% \end{equation}

In this paper, we focus on three widely used graph attention architectures: the original graph attention network (GAT) \citep{gat}, a modified version of this original network (GATv2) \citep{gatv2}, and the Graph Transformer network \citep{transformerconv}. %These graph attention architecture variants are distinguished by the manner in which they compute the unnormalized attention coefficients $e_{ij}$ (Table \ref{table:gat_variants}). 
The three architectures and their equations for computing attention  are presented in \textbf{Appendix} \ref{appen:gat_variants}. 

% In the original graph attention network (GAT) framework, the unnormalized attention coefficients are computed as follows \citep{gat}. Here, $||$ denotes concatenation and the concatenated node features are passed through a single-layer feedforward neural network featuring a weight vector $\mathbf{a} \in \mathbb{R}^{2F'}$ and the LeakyRELU nonlinearity. 
% \begin{equation}
%     \label{eqn:gat_attn}
%     e_{ij} = \text{LeakyReLU}\big(\vec{\mathbf{a}}^T [ \mathbf{W}\vec{h}_i || \mathbf{W}\vec{h}_j \big)]\big)
% \end{equation}
% GATv2 was proposed to improve upon the expressiveness of the original graph attention mechanism by applying the linear projection to concatenated input node features instead of individual node features \citep{gatv2}.
% \begin{equation}
%     \label{eqn:gatv2_attn}
%     e_{ij} = \vec{\mathbf{a}}^T\text{LeakyReLU}\big( \mathbf{W} \vec{h}_i || \mathbf{W} \vec{h}_j \big)
% \end{equation}
% Lastly, the Graph Transformer network extends the Transformer architecture used in natural language processing \citep{transformer} to graphs and computes the attention coefficients as follows, where as above $F'$ is the dimensionality of the new feature space \citep{transformerconv}. 
% \begin{equation}
%     \label{eqn:transformer_attn}
%     e_{ij} = \frac{(\mathbf{W}\vec{h}_i)^T(\mathbf{W}\vec{h}_j)}{\sqrt{F'}}
% \end{equation}

\begin{figure}
    \centering
    %\includegraphics[width=0.95 \linewidth ]{iclr2023/causal_attn_fig1_rs-v4.pdf}
    \includegraphics[width=0.9 \linewidth ]{car_regularization_overview.pdf}
    \caption{Schematic of \methodname: Graph attention networks learn the relative importance of each node-neighbor for a given prediction task. However, their inferred attention coefficients can be miscalibrated due to noise, spurious correlations, or confounders (e.g., node size here). Our causal approach directly intervenes on a sampled subset of edges and supervises an auxiliary task that aligns an edge's causal importance to the task with its attention coefficient.}
    \label{fig:figure_1}
\end{figure}

\subsection{Causal Attention Regularization Scheme}

\methodname is motivated by the invariant prediction (IP) formulation of causal inference \citep{RePEc:bla:jorssb:v:78:y:2016:i:5:p:947-1012}. The central insight of this formulation is that, given sub-models that each contain a different set of predictor variables, the underlying causal model of a system is comprised of the set of all sub-models for which the target-variable marginals are equivalent. This approach is capable of providing statistically rigorous estimates for both the causal effect strength of predictor variables as well as confidence intervals. We leverage the residual formulation of IP, which assumes that we can generate many sub-models with different sets of predictor variables $S^e$ corresponding to many different experiments. We can compute the predictions, $Y^e$ for every sub-model as well as the residuals $\mathcal{R} = Y - Y^e$. IP requires that we perform a hypothesis test on the means of the residuals. The generic method for invariant prediction is to test each hypothetical set of features against the null-hypothesis, $H_{0,S}(\mathcal{E})$, such that there exists $g: \mathbb{R}^{|S|} \times \mathbb{R} \rightarrow \mathbb{R}$ and $\epsilon^e$ that $Y^e = g(\mathcal{G}^e_S, \mathcal{X}^e_S, \epsilon^e)$, $\epsilon^e \sim F_\epsilon$ and $\epsilon^e \indep S^e$ for all $e \in \mathcal{E}$. This is satisfied if the conditionals $Y^e|S^e$ and $Y^f | S^f$ are identical for all experiments $e, f \in \mathcal{E}$. IP then provides a method to construct an estimator of the true causal model by taking the intersection of all models for which the null hypothesis was rejected. 

% Classification tasks on graphs can be understood as estimating $p( C | \mathcal{G}, \mathcal{X} ) = p(C | S) $, where $\mathcal{G}$ is the graph structure, $\mathcal{X}$ is the set of features associated with the graph $\mathcal{G}$, and $S$ is the set of predictor variables. For node classification, the node label is the target variable of interest, and the model is composed of the adjacency matrix and the method by which probabilities are computed. 

To construct a GNN capable of causal inference, we require a technique to generate different sub-models and experiments with different conditional dependence structures. Each sub-model will have the same GNN structure but a slightly different graph structure generated via edge-removal. Given a set of experiments $\{ \mathcal{E} \}$, with target variables $Y^e$ and predictor variables $S^e$, we say that the subset of latent variables, $S^*$, is causal for the prediction of target variable $Y$ if for all $e \in \mathcal{E}$, $S^e$ has an arbitrary distribution and $Y^e = g(S^e, \epsilon^e)$ where $g$ is our statistical model, and $\epsilon^e \sim F_{\epsilon}$ is the error distribution.

The core insight of \methodname is that the graph structure itself is a set of predictor variables in addition to the set of node features.
% that are traditionally explored in causal regularization frameworks. 
This is equivalent to the intuition that relevant edges for a particular task should not only be assigned high attention coefficients but also be important to the predictive accuracy of the model (\textbf{Figure} \ref{fig:figure_1}). When removed from the graph, these relevant edges should cause the predictions that rely on them to substantially worsen. We formalize this intuition by devising an auxiliary supervised prediction task that aims to align the attention coefficient for an edge with the causal effect of removing that edge as per the following loss function:
\begin{equation}
    \label{eqn:causal_reg}
    \mathcal{L}^{c} = \frac{1}{R} \sum^{R}_{r=1} \bigg( \frac{1}{\left| S^{\left( r \right )} \right|}\sum_{\left(n, i, j \right) \in S^{\left( r \right ) }} \ell^{c} \left( \alpha_{ij}^{(n)}, c_{ij}^{(n)} \right) \bigg)
\end{equation}

% We begin by briefly presenting the residual formulation of invariant prediction and then discuss in detail our notion of predictor variable, experiment generation, and experiment test. 
% A key question in causal inference is the identification of identifiable models. Theorem 2 of \citet{RePEc:bla:jorssb:v:78:y:2016:i:5:p:947-1012} indicates that do-interventions such explicit edge deletions generate identifiable causal models in the limit that all predictor variables have been independently intervened upon. While this would be computationally intractable, 

Here, $n$ represents a single entity for which we aim to make a prediction. For a node prediction task, the entity $n$ corresponds to a node, and in a graph prediction task, $n$ corresponds to a graph. In this paper, we assume that all edges are directed and, if necessary, decompose an undirected edge into two directed edges. In each mini-batch, we perform generate $R$ separate sub-models, each of which consists of a set of edge interventions $S^{(r)}$, $r=1,\ldots,R$. Each edge intervention in $S^{(r)}$ is represented by a set of tuples $(n,i,j)$ which denote a selected edge $(i,j)$ for an entity $n$. Note that in a node classification task, $n$ is the same as $j$ (i.e., the node with the incoming edge). More details for the edge intervention procedure and causal effect calculations can be found in the sections below. The causal effect $c_{ij}^{(n)}$ scores the impact of deleting edge $(i,j)$ through a likelihood ratio test. This causal effect is compared to the edge's attention coefficient $\alpha_{ij}^{(n)}$ via the loss function $\ell^c(\cdot,\cdot)$. 
% For models with multiple attention heads, $\alpha_{ij}^{(n)}$ is the mean attention coefficient across heads.

We regularize the attention mechanism in accordance with the learned causal effects from edge interventions. Thus, our full objective function $\mathcal{L}$ includes the loss associated with the prediction $\mathcal{L}^p$, the loss associated with causal attention task $\mathcal{L}^{c}$, and a causal regularization strength hyperparameter $\lambda$ that mediates the contribution of the causal attention task to the objective. 
Rather than explicitly construct our estimator, we rely on regularization as a way to balance the complexity and instability of the model in the following way:

\begin{equation}
    \label{eqn:full_objective}
    \mathcal{L} = \mathcal{L}^{p} + \lambda \mathcal{L}^{c}
\end{equation}
Here, we have $\mathcal{L}^p=\frac{1}{N}\sum_{n=1}^{N}\ell^p(\hat{y}^{(n)}, y^{(n)})$, where $N$ is the size of the training set, $\ell^p(\cdot,\cdot)$ corresponds to the loss function for the given prediction task, $\hat{y}^{(n)}$ is the prediction for entity $n$, and $y^{(n)}$ is the ground truth value for entity $n$. A detailed algorithm for \methodname is provided in \textbf{Appendix} \ref{appen:algo}. We seek to align the attention coefficient for an edge with the causal effect of removing that edge through the use of the following loss function:


% \paragraph{Causal attention objective}
% We leverage the intuition that relevant node-neighbor relations for a particular task should not only be assigned high attention coefficients but also be important to the predictive accuracy of the model (\textbf{Figure} \ref{fig:figure_1}). When removed from the graph, these relevant edges should cause the predictions that rely on them to substantially worsen. We formalize this intuition by devising an auxiliary supervised prediction task that aims to align the attention coefficient for an edge with the causal effect of removing that edge as per the following loss function:
% \begin{equation}
%     \label{eqn:causal_reg}
%     \mathcal{L}^{c} = \frac{1}{R} \sum^{R}_{r=1} \bigg( \frac{1}{\left| S^{\left( r \right )} \right|}\sum_{\left(n, i, j \right) \in S^{\left( r \right ) }} \ell^{c} \left( \alpha_{ij}^{(n)}, c_{ij}^{(n)} \right) \bigg)
% \end{equation}
% \begin{equation}
%     \label{eqn:causal_reg}
%     \mathcal{L}^{c} = \frac{1}{N} \sum^{N}_{n=1} \frac{1}{\left| S^{\left( n \right )} \right|} \sum_{\left( i, j \right) \in S^{\left( n \right ) }} \ell^{c} \left( \alpha_{ij}^{(n)}, c_{ij}^{(n)} \right)
% \end{equation}

% Here, $n$ represents a single entity for which we aim to make a prediction. For a node prediction task, $n$ corresponds to a node, while in a graph prediction task, $n$ corresponds to a graph. $N$ represents the number of such entities in the training set. $\alpha_{ij}^{(n)}$ is the attention coefficient associated with edge $(i,j)$ for entity $n$. For models with multiple attention heads, $\alpha_{ij}^{(n)}$ is the mean attention coefficient for edge $(i,j)$ for entity $n$ across the attention heads. 

% $S^{(n)}$ denotes a set of edges $(i,j)$ associated with entity $n$ that will be individually removed from the training data to compute the causal effect $c_{ij}^{(n)}$. Importantly, we select only one edge per entity to remove in computing $c_{ij}^{(n)}$, so that the direct causal effect of each intervention can be calculated independently of other interventions. $\ell^c(\cdot,\cdot)$ is the loss function used to compare the attention coefficients and the causal effects, which we refer to as the causal regularization loss. 


% Here, $n$ represents a single entity for which we aim to make a prediction. For a node prediction task, the entity $n$ corresponds to a node, and in a graph prediction task, $n$ corresponds to a graph. In this paper, we assume that all edges are directed and, if necessary, decompose an undirected edge into two directed edges. In each mini-batch, we perform $R$ separate rounds of causal effect calculations, each of which consists of a set of edge interventions $S^{(r)}$, $r=1,\ldots,R$. More details for the edge intervention procedure and causal effect calculations can be found in the sections below. 

% Each edge intervention in $S^{(r)}$ is represented by a set of tuples $(n,i,j)$ which denote a selected edge $(i,j)$ for an entity $n$. Note that in a node classification task, $n$ is the same as $j$ (i.e., the node with the incoming edge). The causal effect $c_{ij}^{(n)}$ scores the impact of deleting edge $(i,j)$ on predictive performance. This causal effect is compared to the edge's attention coefficient $\alpha_{ij}^{(n)}$ via the loss function $\ell^c(\cdot,\cdot)$. For models with multiple attention heads, $\alpha_{ij}^{(n)}$ is the mean attention coefficient across heads.

% We regularize the attention mechanism in accordance with the learned causal effects from edge interventions. Thus, our full objective function $\mathcal{L}$ includes the loss associated with the prediction $\mathcal{L}^p$, the loss associated with causal attention task $\mathcal{L}^{c}$, and a causal regularization strength hyperparameter $\lambda$ that mediates the contribution of the causal attention task to the objective. 

% \begin{equation}
%     \label{eqn:full_objective}
%     \mathcal{L} = \mathcal{L}^{p} + \lambda \mathcal{L}^{c}
% \end{equation}
% Here, we have $\mathcal{L}^p=\frac{1}{N}\sum_{n=1}^{N}\ell^p(\hat{y}^{(n)}, y^{(n)})$, where $N$ is the size of the training set, $\ell^p(\cdot,\cdot)$ corresponds to the loss function for the given prediction task, $\hat{y}^{(n)}$ is the prediction for entity $n$, and $y^{(n)}$ is the ground truth value for entity $n$. A detailed algorithm for \methodname is provided in \textbf{Appendix} \ref{appen:algo}.

\paragraph{Edge intervention procedure}
% Classification tasks on graphs can be understood as estimating $p( C | \mathcal{G}, \mathcal{X} ) = p(C | S) $, where $\mathcal{G}$ is the graph structure, $\mathcal{X}$ is the set of features associated with the graph $\mathcal{G}$, and $S$ is the set of predictor variables. For node classification, the node label is the target variable of interest, and the model is composed of the adjacency matrix and the method by which probabilities are computed. To construct a GNN capable of causal inference, we require a technique to generate different sub-models and experiments with different conditional dependence structures. Each sub-model will have the same GNN structure but a slightly different graph structure generated via edge-removal. Given a set of experiments $\{ \mathcal{E} \}$, with target variables $Y^e$ and predictor variables $S^e$, we say that the subset of latent variables, $S^*$, is causal for the prediction of target variable $Y$ if for all $e \in \mathcal{E}$, $S^e$ has an arbitrary distribution and $Y^e = g(S^e, \epsilon^e)$ where $g$ is our statistical model, and $\epsilon^e \sim F_{\epsilon}$ is the error distribution.

We sample a set of edges in each round $r$ such that the prediction for each entity will strictly be affected by at most one edge intervention in that round to ensure effect independence. For example, in a node classification task for a model with one GNN layer, a round of edge interventions entails removing only a single incoming edge for each node being classified. In the graph property prediction case, only one edge will be removed from each graph per round. Because a model with one GNN layer only aggregates information over a 1-hop neighborhood, the removal of each edge will only affect the model's prediction for that edge's target node. To select a set of edges in the $L$-layer GNN case, edges are sampled from the 1-hop neighborhood of each node being classified, and sampled edges that lie in more than one target nodes' $L$-hop neighborhood are removed from consideration as intervention candidates. %; this limits the computational expense of interventions. 

This edge intervention selection procedure is crucial, as it enables the causal effect of each selected intervention $c_{ij}^{(n)}$ on an entity $n$ to be calculated independently of other interventions on a graph. Moreover, by selecting only one intervention per entity within each round, we can parallelize the computation of these causal effects across all entities per round instead of iteratively evaluating just one intervention for the entire graph per entity, significantly aiding scalability. 
 
\paragraph{Calculating task-specific causal effects}
\label{subsec:methods:causaleffect}
We quantify the causal effect of an intervention at edge $(i,j)$ on entity $n$ through the use of an approximate likelihood-ratio test

% as the relative change in the prediction loss for entity $n$ upon removal of that edge.
% \begin{equation}
%     \label{eqn:causal_effect}
%     c_{ij}^{(n)} = \sigma \bigg( \bigg( \frac{\ell^p \bigl( \hat{y}_{\backslash ij}^{(n)}, y^{(n)} \bigr)} {\ell^p \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)} \bigg)^{d(n)}  -1 \bigg)
% \end{equation}

\begin{equation}
    \label{eqn:causal_effect}
    c_{ij}^{(n)} = \sigma \bigg( \bigg( \rho^{(n)}_{ij} \bigg)^{d(n)} - 1 \bigg)\;\;\;\text{where}\;\; \rho^{(n)}_{ij} = \frac{\ell^p \bigl( \hat{y}_{\backslash ij}^{(n)}, y^{(n)} \bigr)} {\ell^p \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)}
\end{equation}

% \begin{equation}
%     \label{eqn:causal_effect}
%     c_{ij}^{(n)} = \sigma \bigg( \frac{\ell^p \bigl( \hat{y}_{\backslash ij}^{(n)}, y^{(n)} \bigr)-\ell^p \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)} {\ell^p \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)} \bigg)
% \end{equation}
Here, $\hat{y}_{\backslash ij}^{(n)}$ is the prediction for entity $n$ upon removal of edge $(i,j)$. $d(n)$ represents the node degree for node classification, while it represents the number of edges in a graph for graph classification. Interventions will likely have smaller effects on higher degree nodes due to the increased likelihood of there being multiple edges that are relevant and beneficial for predictions for such nodes. In graph classification, graphs with many edges are likely to be less affected by interventions as well. Exponentiating the relative intervention effect $\rho^{(n)}_{ij}$ by $d(n)$ is intended to adjust for these biases. We have experimented both with and without raising $\rho$ to the factor of $d$, but have found empirically better results with. We do not have a rigorous explanation as to why, although we suspect the correlated nature of edges implies some amount of shrinkage is necessary. 

% $\ell^p \bigl( \hat{y}_{\backslash ij}^{(n)}, y^{(n)} \bigr) / \ell^p \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)$ so as to account for the number of edges contributing to the prediction for entity $n$. For example, in node classification tasks, predictions for a high-degree node will involve aggregating information over many neighbors, so the effect of a single edge intervention is adjusted via this $d(n)$ term to account for this specific node's high-degree context. 
The link function $\sigma : \mathbb{R} \rightarrow (0,1)$ maps its input to the support of the distribution of attention coefficients. The predictions $\hat{y}^{(n)}$ and $\hat{y}_{\backslash ij}^{(n)}$ are generated from the graph attention network being trained with \methodname. We emphasize that $\hat{y}^{(n)}$ and $\hat{y}_{\backslash ij}^{(n)}$ are both computed during the same training run, rather than in two separate runs. 

% \RS{@AW: the two y's are computed in a single run, right? pls clarify that as a line here?}
% \AW{added another sentence. is this what you mean?}
% %Furthermore, by using the prediction loss in these calculations, \methodname guides attention learning in a manner that is aware of the causal effects on the specific prediction task at hand. 

\paragraph{Scalability}
\methodname increases the computational cost of training in two ways: (i) additional evaluations of the loss function due to the causal effect calculations, and (ii) searches to ensure independent interventions. \methodname performs $\mathcal{O}(RN)$ interventions, where $R$ is the number of interventions per entity and $N$ is the number of entities in the training set. Because our edge intervention procedure ensures that the sampled interventions per round are independent, the causal effects of these interventions can be computed in parallel. In addition, if edge interventions were sampled uniformly across the graph, ensuring the independence each intervention would require a $L$-layer deep BFS that has time complexity $\mathcal{O}(b^L)$, resulting in a worst case time complexity of $\mathcal{O}(R N b^L)$, where $L$ is the depth of the GNN, and $b$ is the mean in-degree. We note that, in practice, GNNs usually have $L \leq 2$ layers since greater depth increases the computational cost and the risk of oversmoothing~\citep{gcn_oversmoothing,measuring_oversmoothing,topping2022understanding}. The contribution of this intervention overlap search step would, therefore, be minimal for most GNNs. We are also able to mitigate much of the computational cost by parallelizing these searches. Further speedups can achieved by identifying non-overlapping interventions as a preprocessing step. In summary, we have found \methodname to have a modest effect on the scalability of graph attention methods, with training runtimes that are only increased by 1.5-2 fold (\textbf{Appendix} \ref{appen:runtime_memory}).

%We have found \methodname to be highly scalable, with training runtimes that are only 1.5-2x of non-regularized attention training (Appendix \ref{appen:runtime_memory}).

% \TM{ Number of interventions scales as $O(C * |V|)$. Each intervention scales as $O(b^2l)$ due to the BFS to ensure non-overlapping interventions, where b is the branching factor and l is the number of layers. In the long run, we're unconcerned about the identification of non-overlapping interventions can be done as a preprocessing step, similar to the generation of graph samples in graph sage.}


==> iclr_directions.tex <==

ICLR requires electronic submissions, processed by
\url{https://openreview.net/}. See ICLR's website for more instructions.

If your paper is ultimately accepted, the statement {\tt
  {\textbackslash}iclrfinalcopy} should be inserted to adjust the
format to the camera ready requirements.

The format for the submissions is a variant of the NeurIPS format.
Please read carefully the instructions below, and follow them
faithfully.

\subsection{Style}

Papers to be submitted to ICLR 2023 must be prepared according to the
instructions presented here.

%% Please note that we have introduced automatic line number generation
%% into the style file for \LaTeXe. This is to help reviewers
%% refer to specific lines of the paper when they make their comments. Please do
%% NOT refer to these line numbers in your paper as they will be removed from the
%% style file for the final version of accepted papers.

Authors are required to use the ICLR \LaTeX{} style files obtainable at the
ICLR website. Please make sure you use the current files and
not previous versions. Tweaking the style files may be grounds for rejection.

\subsection{Retrieval of style files}

The style files for ICLR and other conference information are available online at:
\begin{center}
   \url{http://www.iclr.cc/}
\end{center}
The file \verb+iclr2023_conference.pdf+ contains these
instructions and illustrates the
various formatting requirements your ICLR paper must satisfy.
Submissions must be made using \LaTeX{} and the style files
\verb+iclr2023_conference.sty+ and \verb+iclr2023_conference.bst+ (to be used with \LaTeX{}2e). The file
\verb+iclr2023_conference.tex+ may be used as a ``shell'' for writing your paper. All you
have to do is replace the author, title, abstract, and text of the paper with
your own.

The formatting instructions contained in these style files are summarized in
sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.

\section{General formatting instructions}
\label{gen_inst}

The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).
Use 10~point type with a vertical spacing of 11~points. Times New Roman is the
preferred typeface throughout. Paragraphs are separated by 1/2~line space,
with no indentation.

Paper title is 17~point, in small caps and left-aligned.
All pages should start at 1~inch (6~picas) from the top of the page.

Authors' names are
set in boldface, and each name is placed above its corresponding
address. The lead author's name is to be listed first, and
the co-authors' names are set to follow. Authors sharing the
same address can be on the same line.

Please pay special attention to the instructions in section \ref{others}
regarding figures, tables, acknowledgments, and references.


There will be a strict upper limit of 9 pages for the main text of the initial submission, with unlimited additional pages for citations. 

\section{Headings: first level}
\label{headings}

First level headings are in small caps,
flush left and in point size 12. One line space before the first level
heading and 1/2~line space after the first level heading.

\subsection{Headings: second level}

Second level headings are in small caps,
flush left and in point size 10. One line space before the second level
heading and 1/2~line space after the second level heading.

\subsubsection{Headings: third level}

Third level headings are in small caps,
flush left and in point size 10. One line space before the third level
heading and 1/2~line space after the third level heading.

\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone, regardless of the formatter being used.

\subsection{Citations within the text}

Citations within the text should be based on the \texttt{natbib} package
and include the authors' last names and year (with the ``et~al.'' construct
for more than two authors). When the authors or the publication are
included in the sentence, the citation should not be in parenthesis using \verb|\citet{}| (as
in ``See \citet{Hinton06} for more information.''). Otherwise, the citation
should be in parenthesis using \verb|\citep{}| (as in ``Deep learning shows promise to make progress
towards AI~\citep{Bengio+chapter2007}.'').

The corresponding references are to be listed in alphabetical order of
authors, in the \textsc{References} section. As to the format of the
references themselves, any style is acceptable as long as it is used
consistently.

\subsection{Footnotes}

Indicate footnotes with a number\footnote{Sample of the first footnote} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches
(12~picas).\footnote{Sample of the second footnote}

\subsection{Figures}

All artwork must be neat, clean, and legible. Lines should be dark
enough for purposes of reproduction; art work should not be
hand-drawn. The figure number and caption always appear after the
figure. Place one line space before the figure caption, and one line
space after the figure. The figure caption is lower case (except for
first word and proper nouns); figures are numbered consecutively.

Make sure the figure caption does not get separated from the figure.
Leave sufficient space to avoid splitting the figure and figure caption.

You may use color figures.
However, it is best for the
figure captions and the paper body to make sense if the paper is printed
either in black/white or in color.
\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
\end{center}
\caption{Sample figure caption.}
\end{figure}

\subsection{Tables}

All tables must be centered, neat, clean and legible. Do not use hand-drawn
tables. The table number and title always appear before the table. See
Table~\ref{sample-table}.

Place one line space before the table title, one line space after the table
title, and one line space after the table. The table title must be lower case
(except for first word and proper nouns); tables are numbered consecutively.

\begin{table}[t]
\caption{Sample table title}
\label{sample-table}
\begin{center}
\begin{tabular}{ll}
\multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION}
\\ \hline \\
Dendrite         &Input terminal \\
Axon             &Output terminal \\
Soma             &Cell body (contains cell nucleus) \\
\end{tabular}
\end{center}
\end{table}

\section{Default Notation}

In an attempt to encourage standardized notation, we have included the
notation file from the textbook, \textit{Deep Learning}
\cite{goodfellow2016deep} available at
\url{https://github.com/goodfeli/dlbook_notation/}.  Use of this style
is not required and can be disabled by commenting out
\texttt{math\_commands.tex}.


\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}



\section{Final instructions}
Do not change any aspects of the formatting parameters in the style files.
In particular, do not modify the width or length of the rectangle the text
should fit into, and do not change font sizes (except perhaps in the
\textsc{References} section; see below). Please note that pages should be
numbered.

\section{Preparing PostScript or PDF files}

Please prepare PostScript or PDF files with paper size ``US Letter'', and
not, for example, ``A4''. The -t
letter option on dvips will produce US Letter files.

Consider directly generating PDF files using \verb+pdflatex+
(especially if you are a MiKTeX user).
PDF figures must be substituted for EPS figures, however.

Otherwise, please generate your PostScript and PDF files with the following commands:
\begin{verbatim}
dvips mypaper.dvi -t letter -Ppdf -G0 -o mypaper.ps
ps2pdf mypaper.ps mypaper.pdf
\end{verbatim}

\subsection{Margins in LaTeX}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+
from the graphicx package. Always specify the figure width as a multiple of
the line width as in the example below using .eps graphics
\begin{verbatim}
   \usepackage[dvips]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.eps}
\end{verbatim}
or % Apr 2009 addition
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
for .pdf graphics.
See section~4.4 in the graphics bundle documentation (\url{http://www.ctan.org/tex-archive/macros/latex/required/graphics/grfguide.ps})

A number of width problems arise when LaTeX cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command.

\subsubsection*{Author Contributions}
If you'd like to, you may include  a section for author contributions as is done
in many journals. This is optional and at the discretion of the authors.

\subsubsection*{Acknowledgments}
Use unnumbered third level headings for the acknowledgments. All
acknowledgments, including those to funding agencies, go at the end of the paper.

==> todos.tex <==
\todo[inline]{
Todos: \\
1. P0 Results: \\
 \;\; - \sout{Abstract: need a summary stat or two} \\
 \;\; - Ablations: a) in appendix: need table of correlations between attn wts and homophily scores. b) put in line markers for what random baseline will be \\ 
 \;\; - \sout{Ablations: need label-propagation results} \\
 \;\; - Scalability: need runtimes and machine details \\
2. P0 Writing: \\
 \;\; - \sout{Interpretability: which dataset? \TM{ogbn-arxiv}} \\
3. P1 Results: \\
 \;\; - Fig 3: needs other 3 datasets (in appendix). Also needs p-values \\
 \;\; - Extra: graph property-prediction + graph rewiring. Ok to have limited examples \\
 \;\; - random/uniform regularization 
 \;\; - Should we worry about graph diffusion distance and cheeger constant stuff? Could be a solid appendix section

}


==> v1_theory.tex <==
\subsection{Graph Attention Networks}

Attention mechanisms have been effectively used across many domains by enabling models to dynamically attend to the specific parts of an input that are most relevant to a prediction task \citep{attention_survey}. In graph settings, attention mechanisms compute the relevance of node-neighbor relations. The neighbor aggregation operator in GNNs then uses this information to weight the contribution of each node-neighbor relation in the prediction task. 

Across the multitude of graph attention mechanisms that have been proposed \citep{gat_survey}, the procedures for computing attention take on a general form \citep{gat}. A graph attention layer takes as input a set of node features $\mathbf{h} = \{\vec{h}_1,...,\vec{h}_N\}$, $\vec{h}_i \in \mathbb{R}^F$, where $N$ is the number of nodes and $F$ is the dimensionality of the node features. From these node features, the graph attention layer in a GAT computes unnormalized attention weights for each edge $(i,j)$
\begin{equation}
    \label{eqn:attn_edges}
    e_{ij} = a(\mathbf{W}\vec{h}_i,\mathbf{W}\vec{h}_j),
\end{equation}
where $\mathbf{W}\in \mathbb{R}^{F' \times F}$ linearly projects the input features into a new feature space and the attention mechanism function $a : \mathbb{R}^{F'} \times \mathbb{R}^{F'} \rightarrow \mathbb{R}$ uses these new node features to compute an attention weight for each edge. These attention weights are typically normalized with respect to the 1-hop neighborhood of each node using the softmax function, yielding normalized attention coefficients $\alpha_{ij}$ that indicate the importance of node $i$'s input features to node $j$. For a node $j$, these normalized attention weights are then used to compute a linear combination of the new features for node $j$'s neighbors, which serves as the output of the graph attention layer for node $j$.
\begin{equation}
    \label{eqn:attn_aggr}
    \vec{h}_j' =  \sum_{i\in N_j}\alpha_{ij}\mathbf{W}\vec{h}_i
\end{equation} 
% 
To employ multi-headed attention with $K$ heads, each of the $K$ attention mechanisms first independently calculates its respective normalized attention weights $\alpha_{i,j}^{(k)}$ using its own attention mechanism function $a^{(k)}( \cdot )$ and linear projection weights $\mathbf{W}^{(k)}$. These attention weights are used to compute attention head-specific node outputs $\vec{h}_j'^{(k)}$, which are then averaged across the $K$ attention heads.
\begin{equation}
    \label{eqn:attn_heads}
    \vec{h}_j' = \frac{1}{K}\sum_{k=1}^{K}\vec{h}_j'^{(k)}
\end{equation}

In this paper, we focus on three widely used graph attention architectures: the original graph attention network (GAT) \citep{gat}, a modified version of this original network (GATv2) \citep{gatv2}, and the Graph Transformer network \cite{transformerconv}. These graph attention architecture variants are distinguished by the manner in which they compute the unnormalized attention weights $e_{ij}$ (Table \ref{table:gat_variants}). Here, $||$ denotes concatenation. For GAT and GATv2, the concatenated node features are passed through a single-layer feedforward neural network featuring a weight vector $\mathbf{a} \in \mathbb{R}^{2F'}$ and the LeakyReLU nonlinearity. 

\begin{table}[h!]
\centering
\caption{Attention weight calculation across graph attention architecture variants}
\label{table:gat_variants}
\renewcommand{\arraystretch}{2.5}
\begin{tabular}{ | c | c |} 
    \hline
    GAT \citep{gat} & \(\displaystyle e_{ij} = \text{LeakyReLU}\big(\vec{\mathbf{a}}^T [ \mathbf{W}\vec{h}_i || \mathbf{W}\vec{h}_j \big)]\big) \)  \\
    \hline
    GATv2 \citep{gatv2} & \(\displaystyle e_{ij} = \vec{\mathbf{a}}^T\text{LeakyReLU}\big( \mathbf{W} \vec{h}_i || \mathbf{W} \vec{h}_j \big) \) \\ 
    \hline
    Graph Transformer \citep{transformerconv} & \(\displaystyle e_{ij} = \frac{(\mathbf{W}\vec{h}_i)^T(\mathbf{W}\vec{h}_j)}{\sqrt{F'}} \) \\ 
    \hline
\end{tabular}
\end{table}

% In the original graph attention network (GAT) framework, the unnormalized attention weights are computed as follows \citep{gat}. Here, $||$ denotes concatenation and the concatenated node features are passed through a single-layer feedforward neural network featuring a weight vector $\mathbf{a} \in \mathbb{R}^{2F'}$ and the LeakyRELU nonlinearity. 
% \begin{equation}
%     \label{eqn:gat_attn}
%     e_{ij} = \text{LeakyReLU}\big(\vec{\mathbf{a}}^T [ \mathbf{W}\vec{h}_i || \mathbf{W}\vec{h}_j \big)]\big)
% \end{equation}
% GATv2 was proposed to improve upon the expressiveness of the original graph attention mechanism by applying the linear projection to concatenated input node features instead of individual node features \citep{gatv2}.
% \begin{equation}
%     \label{eqn:gatv2_attn}
%     e_{ij} = \vec{\mathbf{a}}^T\text{LeakyReLU}\big( \mathbf{W} \vec{h}_i || \mathbf{W} \vec{h}_j \big)
% \end{equation}
% Lastly, the Graph Transformer network extends the Transformer architecture used in natural language processing \citep{transformer} to graphs and computes the attention weights as follows, where as above $F'$ is the dimensionality of the new feature space \citep{transformerconv}. 
% \begin{equation}
%     \label{eqn:transformer_attn}
%     e_{ij} = \frac{(\mathbf{W}\vec{h}_i)^T(\mathbf{W}\vec{h}_j)}{\sqrt{F'}}
% \end{equation}

\subsection{Causal Attention Regularization Scheme}

We propose a general-purpose regularization framework for graph attention networks that enhances a given learning task by including an attention learning scheme based on active graph interventions. In this framework, we leverage the intuition that relevant node-neighbor relations for a particular task should not only be assigned high attention weights but also be important to the predictive accuracy of the model. When removed from the graph, these relevant edges should cause the predictions that rely on them to dramatically worsen. 

\subsubsection{Causal Attention Objective}
We formalize this intuition by devising a weakly supervised prediction task that aims to align the attention weight for an edge with the causal effect of removing that edge. The objective function for this task is as follows. 
\\
\begin{equation}
    \label{eqn:causal_reg}
    \mathcal{L}^{c} = \frac{1}{R} \sum^{R}_{r=1} \frac{1}{\left| S^{\left( r \right )} \right|}\sum_{\left(n, i, j \right) \in S^{\left( r \right ) }} \ell^{c} \left( \alpha_{ij}^{(n)}, c_{ij}^{(n)} \right)
\end{equation}
% \begin{equation}
%     \label{eqn:causal_reg}
%     \mathcal{L}^{c} = \frac{1}{N} \sum^{N}_{n=1} \frac{1}{\left| S^{\left( n \right )} \right|} \sum_{\left( i, j \right) \in S^{\left( n \right ) }} \ell^{c} \left( \alpha_{ij}^{(n)}, c_{ij}^{(n)} \right)
% \end{equation}

% Here, $n$ represents a single entity for which we aim to make a prediction. For a node prediction task, $n$ corresponds to a node, while in a graph prediction task, $n$ corresponds to a graph. $N$ represents the number of such entities in the training set. $\alpha_{ij}^{(n)}$ is the attention weight associated with edge $(i,j)$ for entity $n$. For models with multiple attention heads, $\alpha_{ij}^{(n)}$ is the mean attention weight for edge $(i,j)$ for entity $n$ across the attention heads. 

% $S^{(n)}$ denotes a set of edges $(i,j)$ associated with entity $n$ that will be individually removed from the training data to compute the causal effect $c_{ij}^{(n)}$. Importantly, we select only one edge per entity to remove in computing $c_{ij}^{(n)}$, so that the direct causal effect of each intervention can be calculated independently of other interventions. $\ell^c(\cdot,\cdot)$ is the loss function used to compare the attention weights and the causal effects, which we refer to as the causal regularization loss. 

Here, $n$ represents a single entity for which we aim to make a prediction. For a node prediction task, $n$ corresponds to a node, while in a graph prediction task, $n$ corresponds to a graph. We perform $R$ rounds of edge interventions per mini-batch, sampling a set of edges in each round such that the prediction for each entity in the mini-batch will strictly be affected by at most one edge intervention in that round. For example, in a node classification task for a model with one GNN layer, one round of edge interventions for a mini-batch entails removing only a single incoming edge for each node being classified in the mini-batch. Because a model with one GNN layer only aggregates information over a 1-hop neighborhood, the removal of each edge will only affect the model's prediction for that edge's target node. Similarly, in the graph property prediction case, only one edge will be removed from each graph per round. $S^{(r)}$ denotes a set of tuples $(n,i,j)$, each of which corresponds to a selected edge $(i,j)$ for an entity $n$ in round $r$. 

This edge intervention selection procedure is crucial, as it enables the direct causal effect of each selected intervention $c_{ij}^{(n)}$ on an entity $n$ to be calculated independently of other interventions. Furthermore, by selecting only one intervention per entity within each round, we can parallelize the computation of these direct causal effects across all entities per round, enabling the causal effect calculations to be highly scalable. Each causal effect $c_{ij}^{(n)}$ is compared to the attention weight $\alpha_{ij}^{(n)}$ of its corresponding edge via the loss function $\ell^c(\cdot,\cdot)$. For models with multiple attention heads, $\alpha_{ij}^{(n)}$ is the mean attention weight for edge $(i,j)$ for entity $n$ across the attention heads.

We quantify the causal effect $c_{ij}$ of removing edge $(i,j)$ on the prediction for entity $n$ as follows. 
\begin{equation}
    \label{eqn:causal_effect}
    c_{ij}^{(n)} = \sigma \bigg( \frac{\ell \bigl( \hat{y}_{\backslash ij}^{(n)}, y^{(n)} \bigr)-\ell \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)} {\ell \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)} \bigg)
\end{equation}
% talk about importance of using prediction loss to compute causal effect instead of just change in predictions???
$\ell^p(\cdot,\cdot)$ corresponds to the loss function for the given prediction task, $\hat{y}^{(n)}$ is the prediction for entity $n$, $\hat{y}_{\backslash ij}^{(n)}$ is the prediction for entity $n$ upon removal of edge $(i,j)$, and $y^{(n)}$ is the ground truth value for entity $n$. We also include $\sigma(\cdot)$ as a link function that maps its input to the support of the distribution of attention weights. 

We include the above learning task as an additional task to be optimized during training so as to regularize the attention mechanism in accordance with the learned causal effects from edge interventions. Thus, our full objective function $\mathcal{L}$ includes the loss associated with the prediction $\mathcal{L}^p$, the loss associated with causal attention task $\mathcal{L}^{c}$, and a causal regularization strength hyperparameter $\lambda$ that mediates the contribution of the causal attention task to the objective.
\begin{equation}
    \label{eqn:full_objective}
    \mathcal{L} = \mathcal{L}^{p} + \lambda \mathcal{L}^{c}
\end{equation}

==> v2_theory.tex <==
\subsection{Graph Attention Networks}

Attention mechanisms have been effectively used in many domains by enabling models to dynamically attend to the specific parts of an input that are relevant to a prediction task \citep{attention_survey}. In graph settings, attention mechanisms compute the relevance of edges in the graph for a prediction task. A neighbor aggregation operator then uses this information to weight the contribution of each edge \citep{gat_survey,gated_graph_sequence,self_attn_graph_pooling}. 

The approach for computing attention is similar in many graph attention mechanisms. A graph attention layer takes as input a set of node features $\mathbf{h} = \{\vec{h}_1,...,\vec{h}_N\}$, $\vec{h}_i \in \mathbb{R}^F$, where $N$ is the number of nodes. The graph attention layer uses these node features to compute attention coefficients for each edge: $\alpha_{ij} = a(\mathbf{W}\vec{h}_i,\mathbf{W}\vec{h}_j)$, 
% \begin{equation}
%     \label{eqn:attn_edges}
%     e_{ij} = a(\mathbf{W}\vec{h}_i,\mathbf{W}\vec{h}_j),
% \end{equation}
where $a : \mathbb{R}^{F'} \times \mathbb{R}^{F'} \rightarrow (0,1)$ is the attention mechanism function, and the attention coefficient $\alpha_{ij}$ for an edge indicates the importance of node $i$'s input features to node $j$.
% $\mathbf{W}\in \mathbb{R}^{F' \times F}$ projects the input features into a new feature space. The attention mechanism function $a : \mathbb{R}^{F'} \times \mathbb{R}^{F'} \rightarrow [0,1]$ uses these new node features to compute an attention coefficient $\alpha_{ij}$ for each edge that indicates the importance of node $i$'s input features to node $j$. 
% These attention coefficients are typically normalized with respect to the 1-hop neighborhood of each node using the softmax function, yielding normalized attention coefficients $\alpha_{ij}$ that indicate the importance of node $i$'s input features to node $j$.
For a node $j$, these attention coefficients are then used to compute a linear combination of its neighbors' features: $\vec{h}_j' =  \sum_{i\in N(j)}\alpha_{ij}\mathbf{W}\vec{h}_i, ~ ~ \mathit{s.t.} ~ \sum_{i\in N(j)} \alpha_{ij} = 1$.
For multi-headed attention, each of the $K$ heads first independently calculates its own attention coefficients $\alpha_{i,j}^{(k)}$ with its head-specific attention mechanism $a^{(k)}(\cdot,\cdot)$, after which the head-specific outputs are averaged. 
% \begin{equation}
%     \label{eqn:attn_aggr}
%     \vec{h}_j' =  \sum_{i\in N(j)}\alpha_{ij}\mathbf{W}\vec{h}_i,
%     ~ ~ \mathit{s.t.} ~ 
%     \sum_{i\in N(j)} \alpha_{ij} = 1
% \end{equation} 
% 

%RS: commenting out to save some space and make room for causal in the intro
%
%se attention coefficients are used to compute attention-head specific node outputs $\vec{h}_j'^{(k)}$, which are then averaged across the $K$ attention heads.
%
% \begin{equation}
%     \label{eqn:attn_heads}
%     \vec{h}_j' = \frac{1}{K}\sum_{k=1}^{K}\vec{h}_j'^{(k)}
% \end{equation}

In this paper, we focus on three widely used graph attention architectures: the original graph attention network (GAT) \citep{gat}, a modified version of this original network (GATv2) \citep{gatv2}, and the Graph Transformer network \citep{transformerconv}. %These graph attention architecture variants are distinguished by the manner in which they compute the unnormalized attention coefficients $e_{ij}$ (Table \ref{table:gat_variants}). 
The three architectures and their equations for computing attention  are presented in \textbf{Appendix} \ref{appen:gat_variants}. 

% In the original graph attention network (GAT) framework, the unnormalized attention coefficients are computed as follows \citep{gat}. Here, $||$ denotes concatenation and the concatenated node features are passed through a single-layer feedforward neural network featuring a weight vector $\mathbf{a} \in \mathbb{R}^{2F'}$ and the LeakyRELU nonlinearity. 
% \begin{equation}
%     \label{eqn:gat_attn}
%     e_{ij} = \text{LeakyReLU}\big(\vec{\mathbf{a}}^T [ \mathbf{W}\vec{h}_i || \mathbf{W}\vec{h}_j \big)]\big)
% \end{equation}
% GATv2 was proposed to improve upon the expressiveness of the original graph attention mechanism by applying the linear projection to concatenated input node features instead of individual node features \citep{gatv2}.
% \begin{equation}
%     \label{eqn:gatv2_attn}
%     e_{ij} = \vec{\mathbf{a}}^T\text{LeakyReLU}\big( \mathbf{W} \vec{h}_i || \mathbf{W} \vec{h}_j \big)
% \end{equation}
% Lastly, the Graph Transformer network extends the Transformer architecture used in natural language processing \citep{transformer} to graphs and computes the attention coefficients as follows, where as above $F'$ is the dimensionality of the new feature space \citep{transformerconv}. 
% \begin{equation}
%     \label{eqn:transformer_attn}
%     e_{ij} = \frac{(\mathbf{W}\vec{h}_i)^T(\mathbf{W}\vec{h}_j)}{\sqrt{F'}}
% \end{equation}

\begin{figure}
    \centering
    %\includegraphics[width=0.95 \linewidth ]{iclr2023/causal_attn_fig1_rs-v4.pdf}
    \includegraphics[width=0.9 \linewidth ]{car_regularization_overview.pdf}
    \caption{Schematic of \methodname: Graph attention networks learn the relative importance of each node-neighbor for a given prediction task. However, their inferred attention coefficients can be miscalibrated due to noise, spurious correlations, or confounders (e.g., node size here). Our causal approach directly intervenes on a sampled subset of edges and supervises an auxiliary task that aligns an edge's causal importance to the task with its attention coefficient.}
    \label{fig:figure_1}
\end{figure}

\subsection{Causal Attention Regularization Scheme}

\methodname is motivated by the invariant prediction (IP) formulation of causal inference \citep{RePEc:bla:jorssb:v:78:y:2016:i:5:p:947-1012}. The central insight of this formulation is that, given sub-models that each contain a different set of predictor variables, the underlying causal model of a system is comprised of the set of all sub-models for which the target-variable marginals are equivalent. This approach is capable of providing statistically rigorous estimates for both the causal effect strength of predictor variables as well as confidence intervals. We leverage the residual formulation of IP, which assumes that we can generate many sub-models with different sets of predictor variables $S^e$ corresponding to many different experiments. We can compute the predictions, $Y^e$ for every sub-model as well as the residuals $\mathcal{R} = Y - Y^e$. IP requires that we perform a hypothesis test on the means of the residuals. The generic method for invariant prediction is to test each hypothetical set of features against the null-hypothesis, $H_{0,S}(\mathcal{E})$, such that there exists $g: \mathbb{R}^{|S|} \times \mathbb{R} \rightarrow \mathbb{R}$ and $\epsilon^e$ that $Y^e = g(\mathcal{G}^e_S, \mathcal{X}^e_S, \epsilon^e)$, $\epsilon^e \sim F_\epsilon$ and $\epsilon^e \indep S^e$ for all $e \in \mathcal{E}$. This is satisfied if the conditionals $Y^e|S^e$ and $Y^f | S^f$ are identical for all experiments $e, f \in \mathcal{E}$. IP then provides a method to construct an estimator of the true causal model by taking the intersection of all models for which the null hypothesis was rejected. 

% Classification tasks on graphs can be understood as estimating $p( C | \mathcal{G}, \mathcal{X} ) = p(C | S) $, where $\mathcal{G}$ is the graph structure, $\mathcal{X}$ is the set of features associated with the graph $\mathcal{G}$, and $S$ is the set of predictor variables. For node classification, the node label is the target variable of interest, and the model is composed of the adjacency matrix and the method by which probabilities are computed. 

To construct a GNN capable of causal inference, we require a technique to generate different sub-models and experiments with different conditional dependence structures. Each sub-model will have the same GNN structure but a slightly different graph structure generated via edge-removal. Given a set of experiments $\{ \mathcal{E} \}$, with target variables $Y^e$ and predictor variables $S^e$, we say that the subset of latent variables, $S^*$, is causal for the prediction of target variable $Y$ if for all $e \in \mathcal{E}$, $S^e$ has an arbitrary distribution and $Y^e = g(S^e, \epsilon^e)$ where $g$ is our statistical model, and $\epsilon^e \sim F_{\epsilon}$ is the error distribution.

The core insight of \methodname is that the graph structure itself is a set of predictor variables in addition to the set of node features.
% that are traditionally explored in causal regularization frameworks. 
This is equivalent to the intuition that relevant edges for a particular task should not only be assigned high attention coefficients but also be important to the predictive accuracy of the model (\textbf{Figure} \ref{fig:figure_1}). When removed from the graph, these relevant edges should cause the predictions that rely on them to substantially worsen. We formalize this intuition by devising an auxiliary supervised prediction task that aims to align the attention coefficient for an edge with the causal effect of removing that edge as per the following loss function:
\begin{equation}
    \label{eqn:causal_reg}
    \mathcal{L}^{c} = \frac{1}{R} \sum^{R}_{r=1} \bigg( \frac{1}{\left| S^{\left( r \right )} \right|}\sum_{\left(n, i, j \right) \in S^{\left( r \right ) }} \ell^{c} \left( \alpha_{ij}^{(n)}, c_{ij}^{(n)} \right) \bigg)
\end{equation}

% We begin by briefly presenting the residual formulation of invariant prediction and then discuss in detail our notion of predictor variable, experiment generation, and experiment test. 
% A key question in causal inference is the identification of identifiable models. Theorem 2 of \citet{RePEc:bla:jorssb:v:78:y:2016:i:5:p:947-1012} indicates that do-interventions such explicit edge deletions generate identifiable causal models in the limit that all predictor variables have been independently intervened upon. While this would be computationally intractable, 

Here, $n$ represents a single entity for which we aim to make a prediction. For a node prediction task, the entity $n$ corresponds to a node, and in a graph prediction task, $n$ corresponds to a graph. In this paper, we assume that all edges are directed and, if necessary, decompose an undirected edge into two directed edges. In each mini-batch, we perform generate $R$ separate sub-models, each of which consists of a set of edge interventions $S^{(r)}$, $r=1,\ldots,R$. Each edge intervention in $S^{(r)}$ is represented by a set of tuples $(n,i,j)$ which denote a selected edge $(i,j)$ for an entity $n$. Note that in a node classification task, $n$ is the same as $j$ (i.e., the node with the incoming edge). More details for the edge intervention procedure and causal effect calculations can be found in the sections below. The causal effect $c_{ij}^{(n)}$ scores the impact of deleting edge $(i,j)$ through a likelihood ratio test. This causal effect is compared to the edge's attention coefficient $\alpha_{ij}^{(n)}$ via the loss function $\ell^c(\cdot,\cdot)$. 
% For models with multiple attention heads, $\alpha_{ij}^{(n)}$ is the mean attention coefficient across heads.

We regularize the attention mechanism in accordance with the learned causal effects from edge interventions. Thus, our full objective function $\mathcal{L}$ includes the loss associated with the prediction $\mathcal{L}^p$, the loss associated with causal attention task $\mathcal{L}^{c}$, and a causal regularization strength hyperparameter $\lambda$ that mediates the contribution of the causal attention task to the objective. 
Rather than explicitly construct our estimator, we rely on regularization as a way to balance the complexity and instability of the model in the following way:

\begin{equation}
    \label{eqn:full_objective}
    \mathcal{L} = \mathcal{L}^{p} + \lambda \mathcal{L}^{c}
\end{equation}
Here, we have $\mathcal{L}^p=\frac{1}{N}\sum_{n=1}^{N}\ell^p(\hat{y}^{(n)}, y^{(n)})$, where $N$ is the size of the training set, $\ell^p(\cdot,\cdot)$ corresponds to the loss function for the given prediction task, $\hat{y}^{(n)}$ is the prediction for entity $n$, and $y^{(n)}$ is the ground truth value for entity $n$. A detailed algorithm for \methodname is provided in \textbf{Appendix} \ref{appen:algo}. We seek to align the attention coefficient for an edge with the causal effect of removing that edge through the use of the following loss function:


% \paragraph{Causal attention objective}
% We leverage the intuition that relevant node-neighbor relations for a particular task should not only be assigned high attention coefficients but also be important to the predictive accuracy of the model (\textbf{Figure} \ref{fig:figure_1}). When removed from the graph, these relevant edges should cause the predictions that rely on them to substantially worsen. We formalize this intuition by devising an auxiliary supervised prediction task that aims to align the attention coefficient for an edge with the causal effect of removing that edge as per the following loss function:
% \begin{equation}
%     \label{eqn:causal_reg}
%     \mathcal{L}^{c} = \frac{1}{R} \sum^{R}_{r=1} \bigg( \frac{1}{\left| S^{\left( r \right )} \right|}\sum_{\left(n, i, j \right) \in S^{\left( r \right ) }} \ell^{c} \left( \alpha_{ij}^{(n)}, c_{ij}^{(n)} \right) \bigg)
% \end{equation}
% \begin{equation}
%     \label{eqn:causal_reg}
%     \mathcal{L}^{c} = \frac{1}{N} \sum^{N}_{n=1} \frac{1}{\left| S^{\left( n \right )} \right|} \sum_{\left( i, j \right) \in S^{\left( n \right ) }} \ell^{c} \left( \alpha_{ij}^{(n)}, c_{ij}^{(n)} \right)
% \end{equation}

% Here, $n$ represents a single entity for which we aim to make a prediction. For a node prediction task, $n$ corresponds to a node, while in a graph prediction task, $n$ corresponds to a graph. $N$ represents the number of such entities in the training set. $\alpha_{ij}^{(n)}$ is the attention coefficient associated with edge $(i,j)$ for entity $n$. For models with multiple attention heads, $\alpha_{ij}^{(n)}$ is the mean attention coefficient for edge $(i,j)$ for entity $n$ across the attention heads. 

% $S^{(n)}$ denotes a set of edges $(i,j)$ associated with entity $n$ that will be individually removed from the training data to compute the causal effect $c_{ij}^{(n)}$. Importantly, we select only one edge per entity to remove in computing $c_{ij}^{(n)}$, so that the direct causal effect of each intervention can be calculated independently of other interventions. $\ell^c(\cdot,\cdot)$ is the loss function used to compare the attention coefficients and the causal effects, which we refer to as the causal regularization loss. 


% Here, $n$ represents a single entity for which we aim to make a prediction. For a node prediction task, the entity $n$ corresponds to a node, and in a graph prediction task, $n$ corresponds to a graph. In this paper, we assume that all edges are directed and, if necessary, decompose an undirected edge into two directed edges. In each mini-batch, we perform $R$ separate rounds of causal effect calculations, each of which consists of a set of edge interventions $S^{(r)}$, $r=1,\ldots,R$. More details for the edge intervention procedure and causal effect calculations can be found in the sections below. 

% Each edge intervention in $S^{(r)}$ is represented by a set of tuples $(n,i,j)$ which denote a selected edge $(i,j)$ for an entity $n$. Note that in a node classification task, $n$ is the same as $j$ (i.e., the node with the incoming edge). The causal effect $c_{ij}^{(n)}$ scores the impact of deleting edge $(i,j)$ on predictive performance. This causal effect is compared to the edge's attention coefficient $\alpha_{ij}^{(n)}$ via the loss function $\ell^c(\cdot,\cdot)$. For models with multiple attention heads, $\alpha_{ij}^{(n)}$ is the mean attention coefficient across heads.

% We regularize the attention mechanism in accordance with the learned causal effects from edge interventions. Thus, our full objective function $\mathcal{L}$ includes the loss associated with the prediction $\mathcal{L}^p$, the loss associated with causal attention task $\mathcal{L}^{c}$, and a causal regularization strength hyperparameter $\lambda$ that mediates the contribution of the causal attention task to the objective. 

% \begin{equation}
%     \label{eqn:full_objective}
%     \mathcal{L} = \mathcal{L}^{p} + \lambda \mathcal{L}^{c}
% \end{equation}
% Here, we have $\mathcal{L}^p=\frac{1}{N}\sum_{n=1}^{N}\ell^p(\hat{y}^{(n)}, y^{(n)})$, where $N$ is the size of the training set, $\ell^p(\cdot,\cdot)$ corresponds to the loss function for the given prediction task, $\hat{y}^{(n)}$ is the prediction for entity $n$, and $y^{(n)}$ is the ground truth value for entity $n$. A detailed algorithm for \methodname is provided in \textbf{Appendix} \ref{appen:algo}.

\paragraph{Edge intervention procedure}
% Classification tasks on graphs can be understood as estimating $p( C | \mathcal{G}, \mathcal{X} ) = p(C | S) $, where $\mathcal{G}$ is the graph structure, $\mathcal{X}$ is the set of features associated with the graph $\mathcal{G}$, and $S$ is the set of predictor variables. For node classification, the node label is the target variable of interest, and the model is composed of the adjacency matrix and the method by which probabilities are computed. To construct a GNN capable of causal inference, we require a technique to generate different sub-models and experiments with different conditional dependence structures. Each sub-model will have the same GNN structure but a slightly different graph structure generated via edge-removal. Given a set of experiments $\{ \mathcal{E} \}$, with target variables $Y^e$ and predictor variables $S^e$, we say that the subset of latent variables, $S^*$, is causal for the prediction of target variable $Y$ if for all $e \in \mathcal{E}$, $S^e$ has an arbitrary distribution and $Y^e = g(S^e, \epsilon^e)$ where $g$ is our statistical model, and $\epsilon^e \sim F_{\epsilon}$ is the error distribution.

We sample a set of edges in each round $r$ such that the prediction for each entity will strictly be affected by at most one edge intervention in that round to ensure effect independence. For example, in a node classification task for a model with one GNN layer, a round of edge interventions entails removing only a single incoming edge for each node being classified. In the graph property prediction case, only one edge will be removed from each graph per round. Because a model with one GNN layer only aggregates information over a 1-hop neighborhood, the removal of each edge will only affect the model's prediction for that edge's target node. To select a set of edges in the $L$-layer GNN case, edges are sampled from the 1-hop neighborhood of each node being classified, and sampled edges that lie in more than one target nodes' $L$-hop neighborhood are removed from consideration as intervention candidates. %; this limits the computational expense of interventions. 

This edge intervention selection procedure is crucial, as it enables the causal effect of each selected intervention $c_{ij}^{(n)}$ on an entity $n$ to be calculated independently of other interventions on a graph. Moreover, by selecting only one intervention per entity within each round, we can parallelize the computation of these causal effects across all entities per round instead of iteratively evaluating just one intervention for the entire graph per entity, significantly aiding scalability. 
 
\paragraph{Calculating task-specific causal effects}
\label{subsec:methods:causaleffect}
We quantify the causal effect of an intervention at edge $(i,j)$ on entity $n$ through the use of an approximate likelihood-ratio test

% as the relative change in the prediction loss for entity $n$ upon removal of that edge.
% \begin{equation}
%     \label{eqn:causal_effect}
%     c_{ij}^{(n)} = \sigma \bigg( \bigg( \frac{\ell^p \bigl( \hat{y}_{\backslash ij}^{(n)}, y^{(n)} \bigr)} {\ell^p \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)} \bigg)^{d(n)}  -1 \bigg)
% \end{equation}

\begin{equation}
    \label{eqn:causal_effect}
    c_{ij}^{(n)} = \sigma \bigg( \bigg( \rho^{(n)}_{ij} \bigg)^{d(n)} - 1 \bigg)\;\;\;\text{where}\;\; \rho^{(n)}_{ij} = \frac{\ell^p \bigl( \hat{y}_{\backslash ij}^{(n)}, y^{(n)} \bigr)} {\ell^p \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)}
\end{equation}

% \begin{equation}
%     \label{eqn:causal_effect}
%     c_{ij}^{(n)} = \sigma \bigg( \frac{\ell^p \bigl( \hat{y}_{\backslash ij}^{(n)}, y^{(n)} \bigr)-\ell^p \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)} {\ell^p \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)} \bigg)
% \end{equation}
Here, $\hat{y}_{\backslash ij}^{(n)}$ is the prediction for entity $n$ upon removal of edge $(i,j)$. $d(n)$ represents the node degree for node classification, while it represents the number of edges in a graph for graph classification. Interventions will likely have smaller effects on higher degree nodes due to the increased likelihood of there being multiple edges that are relevant and beneficial for predictions for such nodes. In graph classification, graphs with many edges are likely to be less affected by interventions as well. Exponentiating the relative intervention effect $\rho^{(n)}_{ij}$ by $d(n)$ is intended to adjust for these biases. We have experimented both with and without raising $\rho$ to the factor of $d$, but have found empirically better results with. We do not have a rigorous explanation as to why, although we suspect the correlated nature of edges implies some amount of shrinkage is necessary. 

% $\ell^p \bigl( \hat{y}_{\backslash ij}^{(n)}, y^{(n)} \bigr) / \ell^p \bigl( \hat{y}^{(n)}, y^{(n)} \bigr)$ so as to account for the number of edges contributing to the prediction for entity $n$. For example, in node classification tasks, predictions for a high-degree node will involve aggregating information over many neighbors, so the effect of a single edge intervention is adjusted via this $d(n)$ term to account for this specific node's high-degree context. 
The link function $\sigma : \mathbb{R} \rightarrow (0,1)$ maps its input to the support of the distribution of attention coefficients. The predictions $\hat{y}^{(n)}$ and $\hat{y}_{\backslash ij}^{(n)}$ are generated from the graph attention network being trained with \methodname. We emphasize that $\hat{y}^{(n)}$ and $\hat{y}_{\backslash ij}^{(n)}$ are both computed during the same training run, rather than in two separate runs. 

% \RS{@AW: the two y's are computed in a single run, right? pls clarify that as a line here?}
% \AW{added another sentence. is this what you mean?}
% %Furthermore, by using the prediction loss in these calculations, \methodname guides attention learning in a manner that is aware of the causal effects on the specific prediction task at hand. 

\paragraph{Scalability}
\methodname increases the computational cost of training in two ways: (i) additional evaluations of the loss function due to the causal effect calculations, and (ii) searches to ensure independent interventions. \methodname performs $\mathcal{O}(RN)$ interventions, where $R$ is the number of interventions per entity and $N$ is the number of entities in the training set. Because our edge intervention procedure ensures that the sampled interventions per round are independent, the causal effects of these interventions can be computed in parallel. In addition, if edge interventions were sampled uniformly across the graph, ensuring the independence each intervention would require a $L$-layer deep BFS that has time complexity $\mathcal{O}(b^L)$, resulting in a worst case time complexity of $\mathcal{O}(R N b^L)$, where $L$ is the depth of the GNN, and $b$ is the mean in-degree. We note that, in practice, GNNs usually have $L \leq 2$ layers since greater depth increases the computational cost and the risk of oversmoothing~\citep{gcn_oversmoothing,measuring_oversmoothing,topping2022understanding}. The contribution of this intervention overlap search step would, therefore, be minimal for most GNNs. We are also able to mitigate much of the computational cost by parallelizing these searches. Further speedups can achieved by identifying non-overlapping interventions as a preprocessing step. In summary, we have found \methodname to have a modest effect on the scalability of graph attention methods, with training runtimes that are only increased by 1.5-2 fold (\textbf{Appendix} \ref{appen:runtime_memory}).

%We have found \methodname to be highly scalable, with training runtimes that are only 1.5-2x of non-regularized attention training (Appendix \ref{appen:runtime_memory}).

% \TM{ Number of interventions scales as $O(C * |V|)$. Each intervention scales as $O(b^2l)$ due to the BFS to ensure non-overlapping interventions, where b is the branching factor and l is the number of layers. In the long run, we're unconcerned about the identification of non-overlapping interventions can be done as a preprocessing step, similar to the generation of graph samples in graph sage.}

